The Poisson linearization problem for $\mathfrak{sl}_2(\mathbb{C})$. Part II: The Nash-Moser method

This is the second of two papers, in which we prove a version of Conn's linearization theorem for the Lie algebra $\mathfrak{sl}_2(\mathbb{C})\simeq \mathfrak{so}(3,1)$. Namely, we show that any Poisson structure whose linear approximation at a zero is isomorphic to the Poisson structure associated to $\mathfrak{sl}_2(\mathbb{C})$ is linearizable. In the first part, we calculated the Poisson cohomology associated to $\mathfrak{sl}_2(\mathbb{C})$, and we constructed bounded homotopy operators for the Poisson complex of multivector fields that are flat at the origin. In this second part, we obtain the linearization result, which works for a more general class of Lie algebras. For the proof, we develop a Nash-Moser method for functions that are flat at a point.

==> Analysis.tex <==

\section{Homotopy operators for the foliated complex}\label{subsection: homotopy operators}

In this section we prove Lemma \ref{lemma: infinite time pullback} and Proposition \ref{lemma: homotopies}. In Subsection \ref{section: definition}, we construct the homotopy operators as the infinite flow of a specific vector field, and then we reduce Lemma \ref{lemma: infinite time pullback} and Proposition \ref{lemma: homotopies} to their more concrete versions: Lemma \ref{convergence of the flow} and Lemma \ref{well-defined}. We prove these results in Subsection \ref{section: convergence of the flow} by using a detailed analysis of the flow of the vector field, which is provided in Subsection \ref{subsection_analysis_flow}.


\subsection{Construction of the homotopy operators}\label{section: definition}
In order to construct the homotopy operators from Proposition \ref{lemma: homotopies}, we build a foliated homotopy between the identity map and the retraction $r_{\Sk}$. We will do this using the flow of the vector field $W\in \mathfrak{X}^1(\mathfrak{sl}_2(\C))$ given by:
  \begin{align}\label{W}
   W_A=&\frac{1}{4}[A,[A,A^*]].
  \end{align}
  Here the bracket denotes the standard Lie bracket on $\mathfrak{sl}_2(\C)$ and we think of $W$ as a real vector field.
\begin{lemma}\label{lemma: properties vector field}
 The vector field $W$ has the following properties:
 \begin{enumerate}[(1)]
     \item $W$ vanishes precisely on $\Sk$.
     \item $W$ is tangent to the foliation: $\Lie_W f=0$.
     \item $W$ is $SU(2)$-invariant.
     %\item $\Lie_W(\theta)=\dif \theta(W)=0$,
     \item $\Lie_W(R^2 )\leq 0$, with equality only along $\Sk$.
\end{enumerate}
\end{lemma}
\begin{proof}
\begin{enumerate}[(1)]
    \item For the norm of $W$ we get:
    \begin{equation*}
        \begin{array}{rcl}
        |W_A|^2& = & \frac{1}{16}\tr([A,[A,A^*]][[A,A^*],A^*]\\
        & \stackrel{\eqref{eq:invariant polynomials a}}{=} & \frac{1}{16}\tr(4(f\cdot A^*+AA^*A)(\overline{f}\cdot A+A^*AA^*))\\
        &\stackrel{\eqref{eq:invariant polynomials a}}{=} & \frac{1}{4}\tr(\nf^2(A^*A-2AA^*)+(AA^*)^3)\\
        &=&\frac{1}{4}\tr(AA^*((AA^*)^2-\nf^2))\\
        &\stackrel{\eqref{eq:invariant polynomials aah}}{=}&\frac{1}{4}\tr(AA^*)(\tr(AA^*)^2-4\nf^2)\\
        &=&\frac{1}{8}R^2 (R^4-4\nf^2)
        \end{array}
    \end{equation*}
    which is zero iff $A\in \Sk$ due to Lemma \ref{lemma: characterization skeleton}.
    \item A straightforward calculation for $A\in \spl \setminus S_0$ gives:
    \begin{equation*}
        \begin{array}{ccl}
             \Lie_W f &=& \frac{\dif}{\dif t}f(A+tW_A)|_{t=0}  \\
             & =&\frac{\dif}{\dif t}\det(A+tW_A)|_{t=0}\\
            &=&\det(A)\tr(A^{-1}W_A)\\ &=&\frac{1}{4}\det(A)\tr([A,A^*]-A^{-1}[A,A^*]A)\\
             &=&0
        \end{array}
    \end{equation*}
    Since $\spl \setminus S_0$ is dense, (2) holds everywhere on $\spl$.
    \item Straightforward.
    \item We check this again by a direct calculation:
    \begin{equation*}
        \begin{array}{ccl}
             \Lie_W (R^2)&=& \frac{\dif}{\dif t}\tr((A+tW_A)(A^*+tW_A^*))|_{t=0}\\
             &=&\frac{1}{4}\tr([A,[A,A^*]]A^*+A[[A,A^*],A^*])\\
             &=&\frac{1}{4}\tr(4(\nf^2\mathds{1}-(AA^*)^2))\\
             &\stackrel{\eqref{eq:invariant polynomials aah}}{=}&4\nf^2 -R^4\\
             &\stackrel{\eqref{eq:norm-fiber inequality}}{\leq} &0
        \end{array}
    \end{equation*}
    with equality iff $A\in \Sk$ again due to Lemma \ref{lemma: characterization skeleton}.\qedhere
\end{enumerate}
\end{proof}

The last property in Lemma \ref{lemma: properties vector field} implies that the flow lines starting at a point inside the closed ball $\overline{B}_r(0)$ are trapped inside that ball; hence the flow is defined for all positive time, and will be denoted by:
  \begin{equation*}
  \begin{array}{cccc}
   \phi:&\R_{\geq 0}\times\  \mathfrak{sl}_2(\C) &\to&\mathfrak{sl}_2(\C)\\
   &(t,A)&\mapsto&\phi_t(A).
  \end{array}
  \end{equation*}
The above properties of $W$ imply that:
\begin{itemize}
\item $\phi_t$ fixes $\Sk$;
\item $\phi_t^*(f)=f$;
\item $\phi_t$ is $SU(2)$-equivariant.
%\item $\phi_t^*(\dif \theta)=\dif \theta$.
\end{itemize}
In particular, $\phi_t^*$ preserves the complex $(\CC^{\bullet},\dif)$. Also $i_W$ preserves $\CC^{\bullet}$: since $\Lie_W f=0$, we have that $\Lie_{W}f_1=i_W\dif f_1=0$ and $\Lie_W f_2=i_W\dif f_2=0$. 

Next, Cartan's magic formula implies the homotopy relation
\begin{equation}\label{eq: at time t}
\phi_t^*(\alpha)-\alpha=\dif \circ h_t(\alpha)+h_t\circ \dif(\alpha),
\end{equation}
for all $\alpha\in \Omega^{\bullet}_0(\spl)$, where
\[h_t:\Omega^{\bullet}_0(\spl)\to \Omega^{\bullet-1}_0(\spl), \ \ h_t(\alpha)=\int_0^{t}i_W\phi_s^*(\alpha)\dif s.\]
By the discussion above, note that also $h_t$ preserves $\CC^{\bullet}$.

In order to prove Proposition \ref{lemma: homotopies} we will take the limit as $t\to\infty$ in \eqref{eq: at time t}. In the following subsection we will give explicit formulas for $\phi_t$, which imply the point-wise limit: 
\begin{align}\label{infinity now}
\lim_{t\to\infty}\phi_t(A)=r_{\Sk}(A), \ \ \ \forall\  A\in \mathfrak{sl}_2(\C).
\end{align}
The following results are much more involved, and their proofs will occupy the rest of this section:
\begin{lemma}\label{convergence of the flow}
On $\mathfrak{sl}_2(\C)\backslash S_0$, we have that \[\lim_{t\to\infty}\phi_t=r_{\Sk}\] 
with respect to the compact-open $C^{\infty}$-topology.
\end{lemma}

\begin{lemma}\label{well-defined}
For any $\alpha\in \Omega_{0}^{\bullet}(\mathfrak{sl}_2(\C))$, the following limit exists:
   \begin{align}\label{limit h}
    h_{\Sk}(\alpha):=\lim_{t \to \infty}{h_{t}(\alpha)}\in \Omega_{0}^{\bullet-1}(\mathfrak{sl}_2(\C)),
   \end{align}
with respect to the compact-open $C^{\infty}$-topology. Moreover, $h_{\Sk}$ satisfies property $SLB$ for $(0,5,35)$.
\end{lemma}

Recall that the existence of a limit with respect to the compact-open $C^{\infty}$-topology means that all partial derivatives converge uniformly on compact subsets; more details are given in 
Subsection \ref{subsubsection_limits}. 

The results above suffice to complete our proofs:

\begin{proof}[Proofs of Lemma \ref{lemma: infinite time pullback} and Proposition \ref{lemma: homotopies}]
Since the limit \eqref{limit h} is uniform on compact subsets with respect to all $C^k$-topologies, $h_{\Sk}$ satisfies
   \begin{align*}
    \dif h_{\Sk}(\alpha)&=\lim_{t \to \infty}{\dif h_{t}(\alpha)}.
   \end{align*}
From \eqref{eq: at time t}, we obtain that for any $\alpha\in \Omega_0^{\bullet}(\mathfrak{sl}_2(\C))$
\[\lim_{t\to\infty}\phi_t^*(\alpha)=\alpha+\dif h_{\Sk}(\alpha)+h_{\Sk}(\dif \alpha)\]
holds for the compact-open $C^{\infty}$-topology. On the other hand, on $\mathfrak{sl}_2(\C)\backslash S_0$, $\lim_{t\to\infty}\phi_t=r_{\Sk}$, and since this limit is also with respect to the compact-open $C^{\infty}$-topology, we have that 
\[\lim_{t\to\infty}\phi_t^*(\alpha)|_{\mathfrak{sl}_2(\C)\backslash S_0}=r_{\Sk}^*(\alpha)|_{\mathfrak{sl}_2(\C)\backslash S_0}.\]
Therefore, $r_{\Sk}^*(\alpha)|_{\mathfrak{sl}_2(\C)\backslash S_0}$ extends to a smooth form on $\mathfrak{sl}_2(\C)$, which we denote by $p_{\Sk}(\alpha)$. This implies Lemma \ref{lemma: infinite time pullback} and the homotopy equation:
\[p_{\Sk}(\alpha)-\alpha=\dif h_{\Sk}(\alpha)+h_{\Sk}(\dif \alpha).\]
Finally, since $h_t$ commutes with $e_{\varphi}$, and this condition is closed, we have that $h_{\Sk}(\CC^{\bullet})\subset \CC^{\bullet-1}$. Thus, the above relation holds on $\CC^{\bullet}$, and so we obtain also Proposition \ref{lemma: homotopies}.
\end{proof}

% Finally, let us remark also the following properties of these operators.
% \begin{lemma}
% We have that 
% \[h_{\Sk}^2=0,\quad h_{\Sk}\circ p_{\Sk}=0,\quad p_{\Sk}\circ h_{\Sk}=0.\]
% \end{lemma}
% \begin{proof}
% Let $\alpha\in \Omega^{\bullet}_{0}(\spl)$. Then the following hold:
% \[i_{W}h_t(\alpha)=0\ \Rightarrow\ i_Wh_{\Sk}(\alpha)=0\
%  \Rightarrow\ i_W\phi_t^*(h_{\Sk}(\alpha))=0\ \Rightarrow\ h_{\Sk}^2(\alpha)=0.
% \]
% Next, taking $\lim_{s\to \infty}$ in $\phi_s\circ \phi_t=\phi_{s+t}$, we obtain $r_{\Sk}\circ \phi_t=r_{\Sk}$, and so $\dif r_{\Sk} (W)=0$. This implies
% \[i_{W}p_{\Sk}(\alpha)=0\ \Rightarrow\ h_t(p_{\Sk}(\alpha))=0\
%  \Rightarrow\ h_{\Sk}\circ p_{\Sk}(\alpha)=0.
% \]
% The last equation follows from this and because $\phi_t^*$ and  $h_s$ commute.
% \end{proof}

\subsection{The analysis of the flow}\label{subsection_analysis_flow}

In this subsection we analyse the flow $\phi_t$ of the vector field $W$ from \eqref{W}. 

\subsubsection{An explicit formula for the flow}\label{subsection:explicit flow}

The result will be expressed in terms of the function: 
\begin{align*}
          & g:\R_{\ge 0}\times \mathfrak{sl}_2(\C) \to  
          \herm(\C) \\
          & g_t(A):=\left(\mathds{1}+\frac{\tanh(\nf t)}{\nf}AA^*\right)^{\frac{1}{2}}
\end{align*}
and $g_t(A)$ is defined for $f(A)=0$ by continuity as $\left(\mathds{1}+t AA^*\right)^{\frac{1}{2}}$. Here we use the square root of a positive definite Hermitian matrix, as in Subsection \ref{subsubsec_retraction}. Note also that $g$ is a smooth function; this follows because $\tanh(u)/u$ is an even function, and therefore it is a smooth function of $u^2$. Finally, note that, for $f(A)\neq 0$, $\lim_{t\to \infty}g_t(A)=g_{\infty}(A)$. 

We give now an explicit formula for the flow and for the evolution along the flow lines of the norm and of the measure of ``a-normality":
 \begin{lemma}\label{le:flow}
    The flow of $W$ starting at $A\in \mathfrak{sl}_2(\C)$ is given by:
    \begin{equation}\label{eq:A_t}
    A_t:=\phi_t(A)= g_t(A)^{-1}A g_t(A),     
    \end{equation}
    for $t\geq 0$, and moreover, $A_t$ satisfies: 
    \begin{align}
        R_t^2&:=\tr(A_tA_t^*)=2\nf\frac{2\nf\tanh(2\nf t)+ R^2}{2\nf+R^2\tanh(2\nf t)}\label{eq:R_t^2}\\
        K_t&:=[A_t,A_t^*]=
        \frac{2\nf}{2\nf\cosh(2\nf t)+R^2\sinh(2\nf t)}[A,A^*]\label{eq: commutator flow}
    \end{align}
 \end{lemma}

\begin{proof}
First we prove \eqref{eq:R_t^2}. In the proof of Lemma \ref{lemma: properties vector field} (4), we have seen that $\mathcal{L}_W(R^2)=4|f|^2-R^4$. Therefore, $x_t:=R_t^2$ satisfies the following ODE:
\begin{equation}\label{eq:ODE}
x'_t=a^2-x_t^2,
\end{equation}
where $a=2|f|$. The solution of this ODE starting at $x_0=x$ is:
\begin{equation}\label{sol_ODE}
x_t=\frac{a\tanh(a t)+ x}{1+\tanh(a t)\frac{x}{a}}=\frac{\dif }{\dif t}\ln\Big(\cosh(at)+\sinh(at)\frac{x}{a}\Big).
\end{equation}
The second expression will be used later, and the first yields \eqref{eq:R_t^2}.

To prove equation \eqref{eq:A_t}, we first calculate the positive semi-definite Hermitian matrices $S_t:= A_tA_t^*\ge 0$. Using the definition of $W$ \eqref{W} and the characteristic equations \eqref{eq:invariant polynomials a}, we obtain the following ODE for $S_t$:
\begin{align*}
S'_t&=\frac{1}{4}\big(
[A_t,[A_t,A_t^*]]A_t^*+A_t[[A_t,A_t^*],A_t^*]\big)\\
&=\frac{1}{4}\big(2
(A_t)^2(A_t^*)^2-4(A_tA_t^*)^2+A_t(A_t^*)^2A_t+A_t^*(A_t)^2A_t^*\big)\\
&=\nf^2 \mathds{1}-S_t^2.
\end{align*}
This is an ODE of the same form as \eqref{eq:ODE}, but instead of being in $\R$ it is in the commutative algebra spanned by $\mathds{1}$ and $AA^*$, and one can easily see that the solution is of the same form as \eqref{sol_ODE}:
\[S_t =\frac{ \nf \tanh(\nf t)\mathds{1}+AA^*}{ \mathds{1}+\frac{\tanh(\nf t)}{\nf}AA^*} =\frac{\dif }{\dif t}\ln\Big(\cosh(\nf t)\mathds{1}+\frac{\sinh(\nf t)}{\nf}AA^*\Big).\]
In writing this formulas we use that any smooth function $\xi:\R_{>0}\to \R$ ``extends" to a smooth function on $\xi:\herm(\mathbb{C})\to \mathrm{Herm}(\mathbb{C})$, which follows from ``basic functional calculus''. For a diagonal matrix, the extension acts by applying $\xi$ to each diagonal entry, and in general, one uses that the extension is invariant under conjugation by unitary matrices.

Next, we note that the defining ODE for $A_t$ can be written in using $S_t$:
\begin{align*}
A'_t&=\frac{1}{4}[A_t,[A_t,A_t^*]]\\
&=\frac{1}{4}\big(
(A_t)^2A_t^*-2A_tA_t^*A_t+A_t^*(A_t)^2\big)\\
&=\frac{1}{2}[A_t,S_t], 
\end{align*}
where we used the characteristic equation \eqref{eq:invariant polynomials a}. Now, define 
 \[X_t:=\frac{1}{2}\int_0^t{S_s \dif s}=\frac{1}{2}\ln\Big(\cosh(\nf t)\mathds{1}+\frac{\sinh(\nf t)}{\nf}AA^*\Big).\]
The matrices $X_t ,X'_t $ belong to the commutative subalgebra of $\mathfrak{gl}_2(\C)$ generated by $AA^*$, and therefore they commute, which implies that: 
\[\frac{\dif}{\dif t}e^{X_t}=X'_t e^{X_t}=e^{X_t}X'_t.\]
Therefore: 
\[\frac{\dif}{\dif t}e^{X_t}A_te^{-X_t}=e^{X_t}([X'_t,A_t]+A'_t)e^{-X_t}=e^{X_t}(\frac{1}{2}[S_t,A_t]+A'_t)e^{-X_t}=0,\]
and so we obtain a closed formula:
\[A_t=e^{-X_t}Ae^{X_t}.\]
The formula \eqref{eq:A_t} from the statement follows because: 
\[e^{X_t}=\Big(\cosh(\nf t)\mathds{1}+\frac{\sinh(\nf t)}{\nf}AA^*\Big)^{\frac{1}{2}}=
\sqrt{\cosh(\nf t)} g_t(A).
\]

Finally, in order to prove \eqref{eq: commutator flow}, we calculate the derivative of the commutator $K_t$ using the definition of $W$ \eqref{W}:
\begin{align*}
K'_t&=\frac{1}{4}\big(
[[A_t,[A_t,A_t^*]],A_t^*]+[A_t,[[A_t,A_t^*],A_t^*]]\big)\\
&=\frac{1}{2}\big(
(A_t)^2(A_t^*)^2-2(A_tA_t^*)^2+2(A_t^*A_t)^2-(A_t^*A_t)^2\big)\\
&=-R_t^2K_t,
\end{align*}
where we have used the characteristic equations \eqref{eq:invariant polynomials a} and \eqref{eq:invariant polynomials aah}. This ODE has as solution: 
\[K_t=e^{-\int_{0}^tR^2_s\dif s}K_0.\]
Using the second form of \eqref{sol_ODE}, this expression becomes \eqref{eq: commutator flow}.
\end{proof}



\subsubsection{Estimates for the flow and its derivative}

To write the estimates, it will be convenient to introduce the following smooth function:
\begin{equation}\label{varsigma}
\epsilon_t:=\frac{1}{\cosh(2|f|t)+\frac{\sinh(2\nf t)}{2\nf}R^2},  
\end{equation}
which appeared in the formula \eqref{eq: commutator flow}, i.e.\ $K_t=\epsilon_t [A,A^*]$.

The following notation will be very useful. For $u\in \frac{1}{2}\N_{0}$ and $v\in \N_{0}$, let \[\mu_{u,v}:=\sum_{j=0}^{p}t^{u-\frac{j}{2}}R^{v-j}, \ \ p:=\mathrm{min}(2u,v).\]

The following inequalities is immediate: 
\begin{equation}\label{submult}
\mu_{u,v}\, \mu_{u',v'}\leq C \mu_{u+u', v+v'}
\end{equation}
for some constants $C=C(u,u',v,v')$. In particular:
\begin{equation*}
R^{v'}\mu_{u,v}=\mu_{0,v'}\mu_{u,v}\leq \mu_{u, v+v'}.
\end{equation*}
Also, for $w\in \frac{1}{2}\N_0$, note that
\begin{equation}\label{submult1}
 \mu_{u,v}\leq \mu_{u+w, v+2w}.
\end{equation}
We will use these inequalities later on.

In this section, for convenience, we rename the coordinates $(x_i,y_i)$ on $\spl$ from Subsection \ref{section: formal poisson} as $(x_i,x_{i+3})$. Then we obtain partial derivative operators $D^a$, for $a\in \N_0^6$, acting on functions in $C^{\infty}(\spl)$ (see Appendix \ref{subsection: derivatives}). 

As before, we denote $A_t:=\phi_t(A)$. 

\begin{proposition}\label{lemma:bounds on the flow}
For any $a\in \N_0^6$ with $n= \lvert a\rvert$ there is $C=C(a)$ such that:
 \begin{align*}
 \lvert D^a(A_t)\rvert\, &\le\,
 C\,\mu_{2n+\frac{1}{2},3n+2},\\
 \lvert D^a (A'_{t})\rvert\, &\le\, C\, \epsilon_t\, \mu_{2n+\frac{1}{2},3n+4}.
 %&\le 
  %   C t^{\frac{n-1}{2}}(1+tR^2)^{\frac{3n+2}{2}},\\
% \lvert D^a(A_t)\rvert &\le \sigma_{2n,3n+1}\sqrt{1+tR^2},\\
% \lvert D^a(A_t)\rvert &\le  CR^{1-n}
%     \sum_{\frac{n-1}{2}\leq l\leq n}\Big(\frac{tR^2}{1+t|f|}\Big)^{l}    \\
%\lvert D^a (A'_{t})\rvert &\le C\epsilon_t\, t^{\frac{n-3}{2}}(1+tR^2)^{\frac{3n+4}{2}}.
%\lvert D^a (W_{t})\rvert &\le C\varsigma^{-1}\mu_{2n,3n+3}\sqrt{1+tR^2}.
% \lvert D^a (W_{t})\rvert &\le C\frac{1}{\varsigma}\sum_{\frac{n-3}{2}\leq l\leq 2n-1} t^l R^{2l-n+3}.
\end{align*}
\end{proposition}

\subsubsection{Proof of Proposition \ref{lemma:bounds on the flow}}

The proof is split into several steps, which occupy the rest of this section. First, we introduce some auxiliary quantities.

% We give estimates for the flow $A_t:=\phi_t(A)$ and for the vector field $W$ along the flow lines, more precisely, for the function:
% \[A\mapsto W_t(A)=\frac{1}{4}[A_t,[A_t,A_t^*]].\]

% In our estimates, we will use certain polynomial expressions, which we introduce here. For $k\in \N_0$ and $l\in \Z$ define the polynomial $\sigma_{k,l}$ as the sum of all monomials $t^jR^d$ with  
% \[d-2j=l \ \  \textrm{and}\ \ 0\leq j\leq k,\]
% or, in a closed formula: 
% %\[\sigma_{k,l}=\sum_{\frac{|l|-l}{4}\leq j\leq k} t^jR^{2j+l}, \ \ k\in \N, \ l\in \mathbb{Z},\]
% %\[\sigma_{k,l}=\sum_{\mathrm{max}(0,l/2)\leq j\leq k} t^jR^{2j+l}, \ \ k\in \N, \ l\in \mathbb{Z},\]
% \[\sigma_{k,l}=R^l\sum_{m\leq j\leq k} t^jR^{2j}, \ \ m:=\mathrm{max}\big(0,-l/2 \big),\]
% and we set $\sigma_{k,l}=0$ if $m> k$ and $\sigma_{0,0}=1$.

% By comparing terms, the following is immediate: 
% \begin{equation}\label{submult}
% \sigma_{k,l}\, \sigma_{k',l'}\leq C \sigma_{k+k', l+l'},
% \end{equation}
% for some constant $C=C(k,k',l,l')$. In particular:
% \begin{equation*}
% R^d\sigma_{k,l}=\sigma_{0,d}\sigma_{k,l}\leq \sigma_{k, l+d}.
% \end{equation*}
% We will use these inequalities later on. 



Any smooth even function $a(x)$ on $\R$ can be written as $a(x)=b(x^2)$, for a smooth function $b$ on $\R_{\geq 0}$. Using this fact, we introduce 3 functions $\theta_1,\theta_2$ and $\theta_3$ on $\R_{\geq 0}$ defined by:
\begin{equation}\label{theta_tanh}
\theta_1(x^2)=\frac{\tanh(x)}{x},\qquad
\theta_2(x^2)=\cosh(x),\qquad 
\theta_3(x^2)=\frac{\sinh(x)}{x}.  
\end{equation}

The derivatives of these functions satisfy: 
\begin{lemma}\label{lemma:estimate theta}
For $n\geq 0$, there is $C=C(n)$, such that for all $x\geq 0$:
\begin{align*}
|\theta_1^{(n)}(x^2)|&\leq C\frac{1}{(1+x)^{2n+1}},\\
|\theta_2^{(n)}(x^2)|&\leq C\frac{\cosh(x)}{(1+x)^{n}},\\
|\theta_3^{(n)}(x^2)|&\leq C\frac{\cosh(x)}{(1+x)^{n+1}}.
\end{align*}
\end{lemma}
\begin{proof}
It suffices to show the first inequality for $x\geq 1$, and this is equivalent to showing that the following function is bounded:  
\[|x^{2n+1}\theta_1^{(n)}(x^2)|.\]
We prove this by induction. For $n=0$, this follows using $|\tanh(x)|\leq 1$. 
Taking $n\geq 1$ derivatives in the defining equation of $\theta_1$ from \eqref{theta_tanh}, and multiplying by $x^n$, one obtains an expression of the form:
\[x^{2n+1}\theta_1^{(n)}(x^2)=\sum_{1\leq i\leq \frac{n+1}{2}}c_{n,i}x^{2(n-i)+1}\theta_1^{(n-i)}(x^2)+\frac{x^n}{2^n}\tanh^{(n)}(x).\]
By induction, the elements of the sum are bounded. Next, using that \[\tanh'(x)=1-\tanh(x)^2 \quad \textrm{and} \quad \tanh^{(2)}(x)=-2\tanh'(x)\tanh(x),\] we can write $\tanh^{(n)}(x)=\tanh'(x)P_n(\tanh(x))$, where $P_n$ is a polynomial. Clearly, $P_n(\tanh(x))$ and also $x^n\tanh'(x)=\frac{x^n}{\cosh{(x)}}$ are bounded functions, which concludes the proof of the first inequality.

The second inequality is easier: taking $n$ derivatives in the defining equation of $\theta_2$ from \eqref{theta_tanh}, we obtain
\[x^{n}\theta_2^{(n)}(x^2)=\sum_{n/2\leq i<n}c_{n,i}x^{2i-n}\theta_2^{(i)}(x^2)+\frac{1}{2^n}\cosh^{(n)}(x).\]
Using induction, the terms on the right are bounded by $\cosh(x)$, which is enough to conclude the proof of the second inequality. 

The third follows in the same way as the second.
\end{proof}



First, we estimate the derivatives of $\nf^2$:
\begin{lemma}\label{lemma:norm f estimate}
There exists $0<C$ such that for any $a\in \N_0^6$ with $n=\lvert a \rvert$:
\[ \lvert D^a (\nf^2)\rvert  \le C
    \begin{cases}
     \nf\cdot R &\text{ if } n= 1\\
     R^{4-n}&\text{ if }  2\le n \le 4\\
    0 &\text{ else.}
    \end{cases}\]
\end{lemma}
\begin{proof}
The cases $n\neq 1$ follow because $f$ is a homogeneous polynomial of degree 2. The case $n=1$, follows by applying the Leibniz rule in the decomposition $|f|^2=f\overline{f}$.
\end{proof}


Next, we estimate the size of $g_t$:

\begin{lemma}\label{lemma:gt norm}
There is a constant $C$ such that for any $A\in \spl$, we have: 
\[ \lvert g_t(A)\rvert\leq C\mu_{\frac{1}{2},1} \quad \textrm{and}\quad \lvert g_t^{-1}(A)\rvert \leq C.\]
% \[ \lvert g_t(A)\rvert\leq C\Big(1+\frac{tR^2}{1+t\nf}\Big)^{\frac{1}{2}} \quad \textrm{and}\quad \lvert g_t^{-1}(A)\rvert \leq C.\]
% \[ \lvert g_t(A)^{\pm 1}\rvert\leq \sqrt{2+\frac{\tanh(\nf t)}{\nf}R^2}{\color{green}\leq C\sqrt{1+\frac{tR^2}{1+t\nf}}}
% .\]
%, \quad  \lvert g_t(A)^{-1}\rvert\leq =\sqrt{2+\frac{\tanh(\nf t)}{\nf}R^2} .\]
\end{lemma}
\begin{proof}
By the characteristic equation \eqref{eq:invariant polynomials aah} the eigenvalues of $AA^*$ satisfy:
\[\lambda_{-}+\lambda_{+}=R^2,\quad \lambda_{-}\lambda_{+}=|f|^2.\]
The eigenvalues of $g_t(A)^2$ are 
\[1+\frac{\tanh(\nf t)}{\nf}\lambda_{\pm},\]
therefore, using also Lemma \ref{lemma:estimate theta}, we obtain:
\begin{align*}
|g_t(A)|&=\sqrt{\tr(g_t(A)^2)}=\Big(2+\frac{\tanh(\nf t)}{\nf}R^2\Big)^{\frac{1}{2}}\\
&\leq  C\Big(1+\frac{tR^2}{1+t\nf}\Big)^{\frac{1}{2}}\leq C\sqrt{1+tR^2}.
\end{align*}
The first inequality follows now from the following:
\[\sqrt{1+tR^2}\leq 1+t^{\frac{1}{2}}R=\mu_{\frac{1}{2},1}.\]
Similarly, we have that: 
\begin{align*}
\tr(g_t(A)^{-2})&=\frac{1}{1+\frac{\tanh(\nf t)}{\nf}\lambda_{-}}+\frac{1}{1+\frac{\tanh(\nf t)}{\nf}\lambda_+}\\
&=\frac{2+\frac{\tanh(\nf t)}{\nf}R^2}{1+\frac{\tanh(\nf t)}{\nf}R^2+\tanh(\nf t)^2}\\
&\leq 2
\end{align*}
which implies the second inequality.
\end{proof}


We calculate the size of the derivatives of $g_t^2$:
\begin{lemma}\label{lemma:gt estimate}
For any $a\in \N_0^6$ with $0<n=\lvert a\rvert$ there is a constant $C=C(a)$ such that:
% \[\lvert D^a(g_t^2(A))\rvert \le C R^{-n} \sum_{n/2\leq l\leq n}\Big(\frac{tR^2}{1+t|f|}\Big)^{l}.\]
\[\lvert D^a(g_t^2(A))\rvert \le C \mu_{n+1,n+2}.\]
% \[R^{-n}\big(\sum_{ \frac{n}{2}\le p \le n }{(\nf t)^{2p-n}(R^2 t)^{n}\kappa_{p}(\nf t)}+ \sum_{0\le p \le \frac{n}{2} }{(R^2 t)^{2p} \kappa_{p}(\nf t)}\big)+\]
% \[ R^{-n}(1+R^2t) \big(\sum_{ \frac{n}{2}\le p \le n }{(\nf t)^{2p-n}(R^2 t)^{n}\kappa_{p+1}(\nf t)}+ \sum_{0\le p \le \frac{n}{2} }{(R^2 t)^{2p} \kappa_{p+1}(\nf t)}\big).\]
\end{lemma}
\begin{proof}
Using the general chain rule (see Appendix \ref{subsection: derivatives}) and Lemma \ref{lemma:estimate theta}, we first calculate:
\[|D^a(t\theta_1(t^2|f|^2))|\leq C\sum_{k=1}^n\Big(\frac{t}{1+t|f|}\Big)^{2k+1}{\sum}' \prod_{j=1}^{k} D^{a^{j}}(\nf^2),\]
where $\sum '$ sums over all non-trivial $a^j$ with $a=\sum_{j=1}^{k}{a^j}$. Clearly, only the terms with $1\le \vert a^j\rvert \le 4$ are non-zero. Denote by $k_p$ the number of $a^j$'s with $\vert a^j\rvert=p$. Then
using Lemma \ref{lemma:norm f estimate}, we obtain:
\[ |\prod_{j=1}^{k} D^{a^{j}}(\nf^2)|\le C |f|^{k_1}R^{k_1}R^{4k_2-2k_2}R^{4k_3-3k_3}R^{4k_4-4k_4}=C|f|^{k_1}R^{4k-n-2k_1},\]
where we have also used that $k=\sum k_p$ and $n=\sum p k_p$. These decompositions immediately imply that $l:=2k-k_1$ satisfies $m:=\mathrm{max}(k,n/2)\leq l\leq M:=\mathrm{min}(n,2k)$. Therefore, we obtain:
\begin{align*}
|D^a(t\theta_1(t^2|f|^2))|&\leq C\sum_{k=1}^n\sum_{m\leq l\leq M}\Big(\frac{t}{1+t|f|}\Big)^{2k+1}|f|^{2k-l}R^{2l-n}\\
&= C\sum_{k=1}^n\sum_{m\leq l\leq M}\Big(\frac{t|f|}{1+t|f|}\Big)^{2k-l}
\Big(\frac{t}{1+t|f|}\Big)^{l+1}
R^{2l-n}\\
%&\leq CR^{-n-2}\sum_{n/2\leq l\leq n}\Big(\frac{tR^2}{1+t|f|}\Big)^{l+1}\\
&\leq C\sum_{\frac{n}{2}\leq l\leq n}t^{l+1}R^{2l-n}\\
&\leq C\mu_{n+1,n}.
\end{align*}

Next, we apply the Leibniz rule in $g_t^2(A)= \mathds{1} +t\theta(t^2|f|^2) AA^*$, and obtain:
\begin{align*}
|D^a(g_t^2(A))|&\leq\sum_{b+c=a}|D^b(t\theta_1(t^2|f|^2))||D^{c}(AA^*)|\\
&\leq C\sum_{q=0}^2\mu_{n-q+1,n-q}\,\mu_{0,2-q}\\
&\leq C\sum_{q=0}^2\mu_{n-q+1,n+2-2q}\\
&\leq C\mu_{n+1,n+2}
\end{align*}
where for the first terms we have use the inequalities from above, and, because $AA^*$ is a homogeneous polynomial of degree two, that the second term is non-zero only for $q=|c|\leq 2$, and in these cases \[|D^{c}(AA^*)|\leq CR^{2-q}=C\mu_{0,2-q},\]
and finally, the inequalities for the polynomials $\mu_{k,m}$ \eqref{submult} and \eqref{submult1}. 
\end{proof}



\begin{lemma}\label{corollary:g deriv estimate}
For any $a\in \N_0^6$ with $n=\lvert a\rvert>0$ there is a constant $C=C(a)$ such that:
\begin{align*}
    \lvert D^a(g_t^{\pm 1}(A))\rvert \le &\, C \mu_{2n,3n}.
\end{align*}
\end{lemma}
\begin{proof}
Note that by the chain rule (see Appendix \ref{subsection: derivatives}) we have:
\[ D^a(g_t(A))=\sum_{1\leq k\leq n}D^k(x^{\pm \frac{1}{2}})(g_t^2(A)){\sum}' \prod_{j=1}^{k} D^{a^{j}}(g_t^2(A))\]
where $\sum '$ sums over all non-trivial $a^j$ with $a=\sum_{j=1}^{k}{a^j}$. The first part can be estimated using Lemma \ref{lemma:gt norm} by a constant: 
\begin{align*}
    \lvert D^k(x^{\pm \frac{1}{2}})(g_t^2(A))\rvert \leq &\ C\lvert g_t^{-2k\pm 1}(A)\rvert \leq C. \end{align*}
For the second part we set $n_j:=\lvert a^j\rvert $ and use Lemma \ref{lemma:gt estimate} and \eqref{submult} to get:
\begin{align*}
    \lvert\prod_{j=1}^{k}D^{a^{j}}(g_t^2(A))\rvert\le &\, C \prod_{j=1}^{k}\mu_{n_j+1,n_j+2}\\
    \le &\, C \mu_{n+k,n+2k}\\
    \le &\, C \mu_{2n,3n}.
\end{align*} 
Combining these, we obtain the conclusion. 
\end{proof}


\begin{proof}[Proof of the first part of Proposition \ref{lemma:bounds on the flow}]
We use the Leibniz rule to obtain
\begin{align*}
    D^a (A_t)=& \ \sum_{a^1+a^2+a^3=a}D^{a^1}(g_t^{-1}(A))D^{a^2}(A) D^{a^3}(g_t(A)).
\end{align*}
Denote by $n_j:=|a^j|$. Clearly, $n_2=0$ or $n_2=1$. To each term, we apply either Lemma \ref{lemma:gt norm} or \ref{corollary:g deriv estimate}. By Lemma \ref{lemma:gt norm}, the inequality from Lemma \ref{corollary:g deriv estimate} for $g_t^{-1}(A)$ holds also for $n_1=0$, and therefore we only need to consider separately the case when $n_3=0$ and $n_3>0$. In the first case, we obtain: 
\begin{align*}
|D^{a^1}(g_t^{-1}(A))||D^{a^2}(A)| |g_t(A)|&\leq C(\mu_{2n,3n}R+\mu_{2n-2,3n-3})\mu_{\frac{1}{2},1}\\
&\leq C \mu_{2n+\frac{1}{2},3n+2}.
\end{align*}
For the case with $n_3>0$, we also obtain:
\begin{align*}
|D^{a^1}(g_t^{-1}(A))||D^{a^2}(A)| |D^{a^3}(g_t(A))|
\leq & C(\mu_{2n_1,3n_1}R\mu_{2(n-n_1),3(n-n_1)}\\
&+ \mu_{2n_1,3n_1}\mu_{2(n-n_1-1),3(n-n_1-1)})\\
\leq& C(\mu_{2n,3n}R+
\mu_{2n-2,3n-3})\\
\leq& C\mu_{2n,3n+1}\\
\leq &C \mu_{2n+\frac{1}{2},3n+2}.\qedhere
 \end{align*}
% Thus, we obtain that 
% \begin{equation}\label{finer_ineq}
% |D^a (A_t)|\leq C \mu_{2n,3n+1}\sqrt{1+tR^2}.
% \end{equation}
% Now, if $n$ is even, then
% \begin{align*}
% \mu_{2n,3n+1}\sqrt{1+tR^2}&=t^{\frac{n}{2}}R(1+tR^2+\ldots+t^{\frac{3n}{2}}R^{3n})\sqrt{1+tR^2}\\
% &\leq t^{\frac{n-1}{2}}(1+tR^2)^{\frac{3n}{2}+1},
% \end{align*}
% where we have used that $t^{1/2}R\leq \sqrt{1+tR^2}$. If $n$ is odd:
% \begin{align*}
% \mu_{2n,3n+1}\sqrt{1+tR^2}&=t^{\frac{n-1}{2}}(1+tR^2+\ldots+t^{\frac{3n+1}{2}}R^{3n+1})\sqrt{1+tR^2}\\
% &\leq t^{\frac{n-1}{2}}(1+tR^2)^{\frac{3n}{2}+1}.
% \end{align*}
% This concludes the proof. 
\end{proof}

Next, we estimate the derivatives of the commutator:

\begin{lemma}\label{lemma:bounds on the commutator}
For any $a\in \N_0^6$ with $n=\lvert a\rvert $ there is a constant $C=C(a)$ such that:
%\[ \lvert D^a(K_t)\rvert\le C \frac{1}{\varsigma} \sum_{\frac{n-2}{2}\leq l\leq n }t^{l} R^{2l+2-n}\]
\[ \lvert D^a(K_t)\rvert\le C \epsilon_t\, \mu_{2n,3n+2}.\]
\end{lemma}
\begin{proof}
First we estimate $\varsigma_t:=\epsilon_t^{-1}$. For this, we write:
\[\varsigma_t=\theta_2(4\nf^2t^2 )+tR^2\theta_3(4\nf^2t^2),\]
and estimate the two components. Applying Lemma \ref{lemma:estimate theta} and an argument similar to the proof of Lemma \ref{lemma:gt estimate}, we obtain that: 
\begin{align*}
|D^a(\theta_2(4\nf^2 t^2))|&\leq C \sum_{k=1}^n|\theta_2^{(k)}(4\nf^2 t^2)|t^{2k}{\sum}'\prod_{j=1}^k |D^{a^j}(|f|^2)|\\
&\leq C \cosh(2|f|t) \sum_{k=1 }^n
\sum_{m\leq l\leq M}
\Big(\frac{t^2}{1+\nf t}\Big)^k|f|^{2k-l}R^{2l-n}\\
&= C \cosh(2|f|t) \sum_{k=1 }^n
\sum_{m\leq l\leq M}
\Big(\frac{t|f|}{1+\nf t}\Big)^{2k-l}\frac{t^lR^{2l-n}}{(1+|f|t)^{l-k}}\\
&\leq C \cosh(2|f|t) 
\sum_{n/2\leq l\leq n}
t^lR^{2l-n}\\
&\leq   C \cosh(2|f|t)\mu_{n,n},
\end{align*}
where $m=\mathrm{max}(k, n/2)$ and $M:=\mathrm{min}(n,2k)$ and $n=|a|$. 

By a similar argument, we have that:
\begin{align*}
|D^a(t\theta_3(4\nf^2 t^2))|&\leq C \sum_{k=1}^n|\theta_3^{(k)}(4\nf^2 t^2)|t^{2k+1}{\sum}'\prod_{j=1}^k |D^{a^j}(|f|^2)|\\
%&\leq C \cosh(2|f|t) \sum_{k=1 }^n
%\sum_{m\leq l\leq M}
%\Big(\frac{1}{1+\nf t}\Big)^{k+1}t^{2k+1}|f|^{2k-l}R^{2l-n}\\
&\leq C \cosh(2|f|t) \sum_{k=1 }^n
\sum_{m\leq l\leq M}
\Big(\frac{t|f|}{1+\nf t}\Big)^{2k-l}\frac{t^{l+1}R^{2l-n}}{(1+|f|t)^{l+1-k}}\\
&\leq C \cosh(2|f|t) 
\sum_{n/2\leq l\leq n}
t^{l+1}R^{2l-n}\\
&\leq  C \cosh(2|f|t)\mu_{n+1,n}.
\end{align*}
Therefore, applying the Leibniz rule, we obtain:
\begin{align*}
|D^a(tR^2\theta_3(4\nf^2t^2))|&\leq C\sum_{a^1+a^2=a}|D^{a^1}(R^2)||D^{a^2}(t\theta_3(4\nf^2t^2))|\\
&\leq C\cosh(2|f|t)
\sum_{q=0}^2R^{2-q}\mu_{n+1-q,n-q}\\
&\leq C\cosh(2|f|t)
\sum_{q=0}^2\mu_{n+1-q,n+2-2q}\\
&\leq C\cosh(2|f|t)\mu_{n+1,n+2}.
\end{align*}

Combining the estimates obtained so far, and using \eqref{submult1}, we obtain:
\[|D^a(\varsigma_t)|\leq C \cosh(2|f|t) \mu_{n+1,n+2}.
\]


Using this inequality, the chain rule,
that and $\cosh(2\nf t)\leq \varsigma_t$, we get: 
\begin{align*}
    \lvert D^{a}(\epsilon_t)\rvert \le&  C  \sum_{1\leq k\leq n}\varsigma_t^{-k-1} {\sum}' \prod_{j=1}^{k} |D^{a^{j}}(\varsigma)|\\
     \le & C\epsilon_t  \sum_{1\leq k\leq n} {\sum}'\prod_{j=1}^k\mu_{n_j+1,n_j+2}\\
     \le & C\epsilon_t  \sum_{1\leq k\leq n}  \mu_{n+k,n+2k}\\
     \le & C  \epsilon_t \mu_{2n,3n}
     \end{align*} 
where ${\sum}'$ is over all non-trivial decompositions $a=\sum_{j=1}^{k}a^{j}$, and $n_j=|a^j|$.

Recall from \eqref{eq: commutator flow} that $K_t=\varsigma^{-1}[A,A^*]$. By applying the Leibniz rule in this equality, and using the inequality above, we obtain the conclusion:
\begin{align*}
|D^a(K_t)|&\leq \sum_{a=a^1+a^2}|D^{a^1}(\epsilon_t) ||D^{a^2}([A,A^*])|\\
&\leq C \epsilon_t \sum_{q=0}^2\mu_{2n-2q,3n-3q}R^{2-q}\\
&\leq C\epsilon_t \sum_{q=0}^2\mu_{2n-2q,3n-4q+2}\\
&\leq C\epsilon_t \mu_{2n,3n+2}.\qedhere
\end{align*}
\end{proof}


\begin{proof}[Proof of the second part of Proposition \ref{lemma:bounds on the flow}]
In $A_t'=\frac{1}{4}[A_t,K_t]$ we use the Leibniz rule, then the first part of Proposition \ref{lemma:bounds on the flow}, then Lemma \ref{lemma:bounds on the commutator}, and we obtain the inequality from the statement:
\begin{align*}
 |D^a (A'_{t})|&\leq C \sum_{a^1+a^2=a}|D^{a^1}(A_t)||D^{a^2}(K_t)|\nonumber \\
 &\leq C\epsilon_t\sum_{n_1+n_2=n}\, \mu_{2n_1+\frac{1}{2},3n_1+2}
 \mu_{2n_2,3n_2+2}\nonumber \\
 &\leq C\, \epsilon_t\, \mu_{2n+\frac{1}{2},3n+4}.\qedhere
\end{align*}
\end{proof}



\subsection{Proofs of Lemma \ref{convergence of the flow}
and Lemma \ref{well-defined}}\label{section: convergence of the flow}


In the proof below we apply the criterion for the existence of limits of smooth families of functions from Appendix \ref{subsubsection_limits}. 



\subsubsection{Proof of Lemma \ref{convergence of the flow}}
The set $\spl\backslash S_0=\{|f|>0\}$ is covered by the compact sets:
\[K(r,\delta):=\{R\leq r\}\cap \{|f|\geq \delta \}\subset \spl,\ \ \delta, r>0.\]
By the criterion in Appendix \ref{subsubsection_limits}, we need to bound the partial derivatives of $A'_t$ uniformly on $K(r,\delta)$ by an integrable function. By Lemma \ref{lemma:bounds on the flow}
\[\lvert D^a (A'_{t})\rvert \le C\epsilon_t\,\mu_{2n+\frac{1}{2},3n+4}\le C
(1+r)^{3n+4}e^{-2\delta t}t^{2n+\frac{1}{2}},\]
for $t\geq 1$, where we used that 
\[\epsilon_t\leq \cosh^{-1}(2|f|t)\leq e^{-2|f|t}\leq e^{-2\delta t}.\]
Since the right hand side is an integrable function, the conclusion follows.


\subsubsection{A crucial inequality}

The following inequality will play a crucial role in the proof of Lemma \ref{well-defined}:

\begin{lemma}\label{lemma: finite integrals}
For any $q\geq 1$ there is a constant $C=C(q)$ such that:
\[\epsilon_t\, R_t^{2q}\leq C \frac{R^{2q}}{(1+tR^2)^{q}},\]
for all $t\geq 0$ and all $A\in \spl$.
\end{lemma}

\begin{proof}
The inequality is equivalent to 
\begin{align}\label{eq:inequality rewrite}
    \Big(\frac{1}{\cosh(2|f|t)+\frac{\sinh(2\nf t)}{2\nf}R^2}\Big)^{\frac{1}{q}}\Big(\frac{R_t}{R}\Big)^2\leq  \frac{C}{1+R^{2}t}.
\end{align}
Denote $x:=2 \nf t$ and $y:=R^2t$. Then by Lemma \ref{le:flow}, we have:  
\[    \Big(\frac{R_t}{R}\Big)^2= 
\frac{\cosh(x)+\frac{x}{y}\sinh(x)}{\cosh(x)+\frac{y}{x}\sinh(x)}.\]
Using \eqref{eq:norm-fiber inequality}, i.e.\ that $x\leq y$, we have that:
\[    \Big(\frac{R_t}{R}\Big)^2\leq 
\frac{\cosh(x)+\sinh(x)}{\cosh(x)+\frac{y}{x}\sinh(x)}=
\frac{e^x}{\cosh(x)+\frac{y}{x}\sinh(x)}.\]
Therefore, \eqref{eq:inequality rewrite} follows if we prove:
\[ 
\frac{e^x}{\big(\cosh(x)+\frac{y}{x}\sinh(x)\big)^{1+\frac{1}{q}}}\leq \frac{C}{1+y}\]
for $0\leq x\leq y$. Clearly, it suffices to show this for $y\geq 1$, and on this domain this follows if we show that the function 
\[l(x,y):=\frac{ye^x}{\big(\cosh(x)+\frac{y}{x}\sinh(x)\big)^{1+\frac{1}{q}}}\]
is bounded on $0\leq x\leq y$. We have that:
\[\partial_yl(x,y)=\frac{e^x(\cosh(x)-y\frac1q\frac{\sinh(x)}{x})
}{\big(\cosh(x)+\frac{y}{x}\sinh(x)\big)^{2+\frac{1}{q}}}.\]
Therefore, for a fixed $x$, the $l(x,y)$ attains its maximum in 
\[y_x:=\frac{qx}{\tanh(x)}\geq x.\]
We have that 
\[l(x,y_x)=\frac{q}{(1+q)^{1+\frac{1}{q}}}\frac{xe^x}{\sinh(x)\cosh(x)^{\frac{1}{q}}}.\]
Since $l(x,y)\leq l(x,y_x)$, and  
\[\lim_{x\to 0}l(x,y_x)=l(0,q)=\frac{q}{(1+q)^{1+\frac{1}{q}}}, \quad \lim_{x\to \infty}l(x,y_x)=0,\]
is follows that $l(x,y)$ is bounded, which completes the proof.
\end{proof}

\subsubsection{Estimates for the pullback}

Next, we estimate the pullback under $\phi_t$ of flat forms.
We will prove all estimates on the closed ball $\overline{B}_r\subset \spl$ of radius $r>0$ centered at the origin. We will use the norms $\fnorm{\cdot}_{n,k,r}$ on flat forms $\Omega^i_0(\overline{B}_r)$ defined in \eqref{eq: flat norms}.


\begin{lemma}\label{pullback estimates}
For every $a\in \N^6_0$ with $n=|a|$, any $j,l\in \N_0$ there is a constant $C$ such that for any flat form $\alpha\in \Omega^{d}_0(\overline{B_r})$ and any $t\geq 0$:
\begin{align*}
|D^a(\phi_t^*(\alpha))|&\leq C R_t^{j+l}\mu_{\frac{5}{2}(n+d),5(n+d)}\fnorm{\alpha}_{n+l,j,r}.
\end{align*}
\end{lemma}
\begin{proof}
\underline{Step 1}: We first prove the estimate for $n=d=0$, i.e., for $g\in C^{\infty}_0(\overline{B_r})$ and for $a=0\in \N_0^6$. For $l=0$, the estimate follows
\[|\phi_t^*(g)|=R_t^{j}\frac{|\phi_t^*(g)|}{R_t^{j}}
\le R_t^{j}\fnorm{g}_{0,j,r}.
\]
For $l\geq 1$, we use Taylor's formula with integral remainder to write
\[g(A)=\sum_{|b|=l}A^{b}\int_{0}^1l(1-s)^{l-1}(D^{b} g)(sA)\dif s,\]
where we used that $g$ is flat at the origin, and we denoted $A^{b}=\prod_{i=1}^6 x_i^{b_i}$ in the coordinates introduced in Subsection \ref{subsection: derivatives}. Therefore we obtain:
\begin{align}\label{eq: integral remainder}
    \phi_t^*(g)(A)=\sum_{|b|=l}A_t^{b}\int_{0}^1l(1-s)^{l-1}(D^{b} g)(sA_t)\dif s.
\end{align}
We clearly have that
\[|A_t^{b}|\leq R_t^{l}.\]
For any $j\in \N_0$, we have that
\[|(D^{b} g)(sA_t)|\leq (sR_t)^{j}\fnorm{g}_{l,j,r}.\]
Using these inequalities in \eqref{eq: integral remainder}, we obtain the estimate in this case:
\begin{equation}\label{eq:Step1}
|\phi_t^*(g)|\leq CR_t^{l+j}\fnorm{g}_{l,j,r}.
\end{equation}

\noindent\underline{Step 2}: we prove now the estimate for a flat function $g$ and $a\in \N^6_0$ with $1\le n=|a|$. We use the chain rule (see Appendix \ref{subsection: derivatives}) to write:
\[D^a(g\circ \phi_t)=\sum_{1\leq |b|\leq n}D^b(g)(A_t)\ {\sum}'\prod_{i=1}^{6}\prod_{j=1}^{b_i}D^{a^{ij}}(x_{i,t}),
\]
where $b=(b_i)_{i=1}^6$ and $\sum'$ is the sum over all non-trivial decompositions: 
\[a=\sum_{i=1}^6\sum_{j=1}^{b_i}a^{ij}.\]
We apply \eqref{eq:Step1} with $l\leftarrow n-|b|+l$ to estimate the first term: 
\begin{align*}
    |D^b(g)(A_t)|&\leq  C R_t^{n-|b|+l+j}\fnorm{g}_{n+l,j,r}.
\end{align*}
We estimate the second term using Proposition \ref{lemma:bounds on the flow}
\begin{align*}
\big|\prod_{i=1}^6\prod_{j=1}^{b_i}D^{a^{ij}}(x_{i,t})\big|&\leq C \prod_{i=1}^6\prod_{j=1}^{b_i}
\mu_{2|a^{ij}|+\frac{1}{2},3|a^{i,j}|+2}\\
&\leq C\mu_{2n+\frac{1}{2}|b|,3n+2|b|}.
\end{align*}
The second case follows by using these two estimates, and the inequalities: 
\begin{align*}
R_t^{n-|b|}&\leq R^{n-|b|}=\mu_{0,n-|b|}\\
\mu_{0,n-|b|}\mu_{2n+\frac{1}{2}|b|,3n+2|b|}&\leq C\mu_{2n+\frac{1}{2}|b|,4n+|b|}\leq C\mu_{\frac{5}{2}n,5n}.
\end{align*}

\noindent\underline{Step 3}: let $\alpha\in \Omega^d_0(\overline{B}_r)$, $d\geq 1$, and $a\in \N^6_0$. Note that the coefficients of $\phi_t^*(\alpha)$ are sums of elements of the form 
\[g\circ \phi_t\cdot M(\phi_t),\] 
where $g\in C^{\infty}_0(\overline{B}_r)$ is a coefficient of $\alpha$ and $M(\phi_t)$ denotes the determinant of a minor of rank $d$ of the Jacobian matrix of $\phi_t$. By the Leibniz rule:
\[D^a(g\circ \phi_t\cdot M(\phi_t))=\sum_{b+c=a}D^b(g\circ \phi_t)D^c(M(\phi_t)).\]
For the first term, we apply Step 2 with $n\leftarrow |b|$ and $l\leftarrow |c|+l$:
\begin{align*}
|D^b(g\circ \phi_t)|&\leq C R_t^{|c|+l+j} \mu_{\frac{5|b|}{2},5|b|}\fnorm{\alpha}_{n+l,j,r}\\
&\leq C R_t^{l+j} \mu_{\frac{5|b|}{2},5|b|+|c|}\fnorm{\alpha}_{n+l,j,r}.
\end{align*}
Note that $M(\phi_t)$ is a homogeneous polynomial of degree $d$ in the first order partial derivatives of the components $x_{i,t}$ of $\phi_t$. By Proposition \ref{lemma:bounds on the flow} each partial derivative satisfies: 
\[\Big|D^{c}\Big(\frac{\partial x_{i,t}}{\partial x_j}\Big)\Big|\leq C \mu_{2|c|+\frac{5}{2},3|c|+5}.\]
Therefore, by applying the Leibniz rule and \eqref{submult}, we obtain:
\[|D^c M(\phi_t)|\leq C \mu_{2|c|+\frac{5}{2}d,3|c|+5d}.\]
The estimate follows by combing these two estimates and using that: 
\[
\mu_{\frac{5|b|}{2},5|b|+|c|}
\mu_{2|c|+\frac{5}{2}d,3|c|+5d}\leq 
\mu_{2n+\frac{|b|+5d}{2},4n+|b|+5d}\leq \mu_{\frac{5}{2}(n+d),5(n+d)}.\qedhere\]
\end{proof}

\subsubsection{Proof of Lemma \ref{well-defined}}

Let $\alpha\in \Omega^d_0(\spl)$. As explained in Subsection \ref{subsubsection_limits}, for each $r>0$, we need to bound the partial derivatives of $h'_t(\alpha)$ uniformly on the balls $\overline{B}_r$ by an integrable function.

Let $a\in \N^6_0$, with $n=|a|$. First, we show that for any $j\geq 2$ there is a constant $C=C(n,j)$ such that:
\begin{equation}\label{important_equation}
|D^a(h'_t(\alpha))|\leq C\, R^{3+j}(1+tR^2)^{\frac{5(n+d)+1-j}{2}}\fnorm{\alpha}_{n,j,r}.
\end{equation}

For this recall that
\[h'_t(\alpha)=i_{W}\phi_t^*(\alpha)=\phi_t^*(i_W\alpha)=\sum_{i=1}^6x'_{i,t}\,\phi_t^*(\alpha_i),\]
where $\alpha_i=i_{\partial_{x_i}}\alpha$ and $x'_{i,t}$ are denote the entries of the matrix $A'_t$. 

First we apply the Leibniz rule:
\[D^a(x_{i,t}'\,\phi_t^*(\alpha_i))=\sum_{b+c=a}D^b(x_{i,t}') D^c(\phi_t^*(\alpha_i)).\]
By using Proposition \ref{lemma:bounds on the flow}, we obtain:
\[|D^b(x'_{i,t})|\leq 
C\, \epsilon_t\, \mu_{2|b|+\frac{1}{2}, 3|b|+4}.\]
By applying Lemma \ref{pullback estimates} with $n\leftarrow n-|b|=|c|$ and $l\leftarrow |b|$, we obtain:
\begin{align*}
|D^c(\phi_t^*(\alpha_i))|
&\leq C R_t^{|b|+j}\mu_{\frac{5}{2}(|c|+d),5(|c|+d)}\fnorm{\alpha}_{n,j,r}\\
&\leq C R_t^{j}\mu_{\frac{5}{2}(|c|+d),5(|c|+d)+|b|}\fnorm{\alpha}_{n,j,r}.
\end{align*}
When we combine these inequalities, we first note that:
\begin{align*}
\mu_{2|b|+\frac{1}{2}, 3|b|+4}\mu_{\frac{5}{2}(|c|+d),5(|c|+d)+|b|}&\leq 
C\mu_{2n+\frac{1}{2}(|c|+5d+1),4n+|c|+5d+4}\\
&\leq
\mu_{\frac{1}{2}(5(n+d)+1),5(n+d)+4}.
\end{align*}
Thus, we obtain:
\begin{equation}
|D^a(h'_t(\alpha))|\leq C\,\epsilon_t\, R_t^j\mu_{\frac{1}{2}p,p+3}\fnorm{\alpha}_{n,j,r},
\end{equation}
where $p=5(n+d)+1$. Next, note that: 
\[\mu_{\frac{p}{2},p+3}=\sum_{j=0}^pt^{\frac{p-j}{2}}R^{p-j+3}\leq R^3(1+t^{\frac{1}{2}}R)^{p}\leq C R^3(1+tR^2)^{\frac{p}{2}}, \]
where we have use that $(1+t^{\frac{1}{2}}R)\leq \sqrt{2}(1+tR^2)^{\frac{1}{2}}$. Using this and Lemma \ref{lemma: finite integrals} with $q=\frac{j}{2}\geq 1$, we obtain \eqref{important_equation}.

For $j=5(n+d+1)$, \eqref{important_equation} gives:
\begin{align*}
|D^a(h'_t(\alpha))|\leq C\, \frac{R^{j+3}}{(1+tR^2)^2}\fnorm{\alpha}_{n,j,r}\leq C\, r^{j-1}t^{-2}\fnorm{\alpha}_{n,j,r}.
\end{align*}
The right-hand side is integrable over $t\in [1,\infty)$. Therefore by Appendix \ref{subsubsection_limits}, $h_t(\alpha)$ converges as $t\to\infty$ in all $C^n$-norms on $\overline{B}_r$ to a smooth form $h_{\Sk}(\alpha)$. This form is flat at the origin, because flatness is $C^{\infty}$-closed. 

Next, for $j=5(n+d+1)+k$, \eqref{important_equation} gives:
\begin{align*}
|D^a(h'_t(\alpha))|&\leq C\, \frac{R^{5(n+d+1)+3+k}}{(1+tR^2)^{2+\frac{k}{2}}}\fnorm{\alpha}_{n,5(n+d+1)+k,r}\\
&\leq C\,r^{5(n+d+1)+1} \frac{R^{2+k}}{(1+tR^2)^{2}}\fnorm{\alpha}_{n,5(n+d+1)+k,r}.
\end{align*}
Since $\int_0^{\infty}\frac{R^{2}\dif t}{(1+tR^2)^{2}}=1$, we obtain:
\begin{align*}
|D^a(h_t(\alpha))|&=
\Big|\int_0^t D^a(h'_s(\alpha))\dif s\Big|\\
&\leq C\, r^{5(n+d+1)+1}R^k\fnorm{\alpha}_{n,5(n+d+1)+k,r}.
\end{align*}
And so:
\begin{align*}
\frac{|D^a(h_t(\alpha))|}{R^k}&\leq C\, r^{5(n+d+1)+1}\fnorm{\alpha}_{n,5(n+d+1)+k,r}.
\end{align*}
This implies that:
\begin{align*}
\fnorm{h_t(\alpha)}_{n,k,r}
\leq C\, (1+r)^{5(n+d+1)+1}\fnorm{\alpha}_{n,5(n+d+1)+k,r}.
\end{align*}
Taking $\lim_{t\to\infty}$ on the left implies that $h_{\Sk}$ satisfies property SLB for $(0,5,35)$.

==> Flat_foli.tex <==
\section{Flat foliated cohomology of $\spl$}\label{section flat foli}

%it in Proposition \ref{proposition:flat foliated ch} 

In this section we define the flat foliated cohomology of the singular foliation $\F$ on $\spl$. For the calculation of this cohomology, we first apply an averaging argument for the compact subgroup $SU(2)\subset SL(2,\C)$. The more involved part of the calculation uses a so-called \emph{cohomological skeleton} for the foliation $\F$, i.e., a subvariety that contains the cohomological information of the closed leaves. A retraction to the cohomological skeleton is further used to build homotopy operators for the flat foliated complex. This is based on Lemma \ref{lemma: infinite time pullback} and Proposition \ref{lemma: homotopies}, whose proofs we delay to Section \ref{subsection: homotopy operators}. 

The flat foliated cohomology and the homotopy operators will be the building blocks for the computation of flat Poisson cohomology and the existence of ``good'' homotopy operators for the flat Poisson complex. These will play a crucial role in the proof of the linearization theorem. 

\subsection{The statement and explanations of the results}\label{section: foliated ch}

The singular foliation $\F$ of $(\spl,\pi)$ restricts on $\spl\backslash\{0\}$ to a regular, corank two, unimodular foliation. In this subsection we first recall the foliated de Rham complex of a regular foliation. Then we adapt this notion to introduce the flat foliated complex of $\F$ on $\spl$, which gives rise to flat foliated cohomology. We also state the main results of Section \ref{section flat foli}: we describe the flat foliated cohomology groups and claim the existence of homotopy operators. The proofs of these results will occupy the rest of Section \ref{section flat foli} and Section \ref{subsection: homotopy operators}.



\subsubsection{Foliated cohomology}
We first look at a regular foliation $\mathcal{F}$ on a manifold $M$, and we denote the \textbf{complex of foliated forms} by 
\[(\Omega^{\bullet}(\mathcal{F}), \dif_{\mathcal{F}})\ \ \ \text{
where }\ \ \Omega^{\bullet}(\mathcal{F}):=\Gamma(\wedge^{\bullet} T^*\mathcal{F}).\]
This complex consists of smooth families of differential forms along the leaves of $\mathcal{F}$, and $\dif_{\mathcal{F}}$ is the leafwise de Rham differential. The resulting cohomology is called the \textbf{foliated cohomology} of $\F$, denoted $H^{\bullet}(\F)$. The normal bundle to $\F$, denoted by $\nu:=TM/T\F$, carries the \textbf{Bott connection}
\[\nabla:\Gamma(T\F)\times \Gamma(\nu)\to \Gamma(\nu),\ \ \ \  \nabla_X(\overline{V}):=\overline{[X,V]},\]
which, via the usual formula for the exterior derivative, induces a differential on $\nu$-valued forms $(\Omega^{\bullet}(\F,\nu),\dif_{\nabla})$. This yields the cohomology of $\F$ with values in $\nu$, denoted $H^{\bullet}(\F,\nu)$. Similarly, the dual connection on $\nu^*$ gives rise to a connection on the exterior powers $\wedge^{q}\nu^*$, and we obtain the complexes $(\Omega^{\bullet}(\F,\wedge^{q}\nu^*),\dif_{\nabla})$, with cohomology groups $H^{\bullet}(\F,\wedge^{q}\nu^*)$.

In particular, for $q=\mathrm{codim}(\F)$, we have a canonical isomorphism
\[(\Omega^{\bullet}(\F,\wedge^q\nu^*),\dif_{\nabla})\simeq (\CC^{\bullet},\dif),\]
where $(\CC^{\bullet},\dif)$ is the subcomplex of $(\Omega^{\bullet+q}(M),\dif)$, defined by:
\[ \CC^{p}:=\big\{\alpha\in\Omega^{p+q}(M)\, |\, \forall\, v_1,\ldots,v_p\in T_x\F\, :\,  i_{v_1}\ldots i_{v_p}\alpha\in \wedge^q\nu_x^*\big\}.\]
Assume that $\F$ is coorientable and let $\varphi\in \Gamma(\wedge^q\nu^*)\subset \Omega^q(M)$ be a defining $q$-form for $\F$, i.e., $\varphi$ is nowhere zero and $T\F=\ker (\varphi)$. Then the subcomplex $\CC^{\bullet}$ admits the alternative description:
% \[(\Omega^{\bullet}(\F,\wedge^q\nu^*),\dif_{\nabla})\simeq (\CC^{\bullet},\dif)=(e_{\varphi}(\Omega^{\bullet}(M)),\dif) \subset (\Omega^{\bullet+q}(M),\dif),\]
\[(\CC^{\bullet},\dif)=(e_{\varphi}(\Omega^{\bullet}(M)),\dif) \subset (\Omega^{\bullet+q}(M),\dif),\]
where $e_{\varphi}(-)=\varphi\wedge (-)$ denotes the exterior product with $\varphi$.

The foliation $\F$ is called \textbf{unimodular} if there exists a defining $q$-form $\varphi$ which is closed: $\dif \varphi=0$. Such a form is parallel for the dual of the Bott connection, and it induces an isomorphism of complexes: 
\begin{align}\label{eq: cochain isomorphism}
    (\Omega^{\bullet}(\F),\dif_{\F})\diffto (\Omega^{\bullet}(\F,\wedge^q \nu^*),\dif_{\nabla}), \ \ \eta\mapsto \varphi \otimes  \eta.
\end{align}
Therefore, in this case, the subcomplex $\CC^{\bullet}$ can be used to calculate the foliated cohomology of $\F$.

\subsubsection{Flat foliated cohomology of $\spl$}
Note that on $\spl\setminus\{0\}$ the regular foliation $\F|_{\spl\setminus\{0\}}$ is unimodular with defining $2$-form
\[\varphi:=\dif f_1\wedge \dif f_2,\quad \textrm{where}\quad f=f_1+i f_2.\]
We denote by $\Omega_0^{\bullet}(\spl)$ the set of differential forms that are flat at the origin, i.e., all partial derivatives of the coefficients vanish at the origin. Motivated by the discussion in the previous subsection, we introduce: 
\begin{definition}\label{definition: flat foliated ch}
We call the cohomology of the complex 
\begin{equation}\label{ffcomplex}
(\CC^{\bullet}:=e_{\varphi}(\Omega^{\bullet}_0(\spl)),\dif)
\end{equation}
the \textbf{flat foliated cohomology} of $\spl$, and we denote it by $H^{\bullet}_0(\F)$.
\end{definition}
The rest of the section is devoted to the calculation of the groups $H^{\bullet}_0(\F)$.


\subsubsection{The foliated cohomology away from $S_0$}\label{subsection:away from S_0}

To gain some geometric intuition, let us first discuss the foliated cohomology of $\F$ restricted to the open set $\spl\backslash S_0$. Here, the foliation is given by a the fibers of a locally trivial fibration:
\[ f:\spl \setminus S_0 \to \C^{\times}:= \C\setminus \{0\}.\]

For any such locally trivial fibration $p:E\to B$ with connected fibers, if the cohomology groups of the fibers are finite-dimensional, then they fit into a smooth vector bundle:
\[\mathcal{H}^{\bullet}\to B,\quad \mathcal{H}^{k}_b:=H^{k}(p^{-1}(b)).\]
The global sections of $\mathcal{H}^{\bullet}$ can be identified with the cohomology of the simple foliation $\mathcal{F}(p)$ associated to the submersion $p$:
\[H^{\bullet}(\mathcal{F}(p))\simeq \Gamma(\mathcal{H}^{\bullet}).\]

In our case, the fibers $f^{-1}(z)=S_z$, for $z\in \C^{\times}$, are all diffeomorphic to $T^*S^2$, which is homotopy equivalent to $S^2$. 
Hence, we have that
\[H^{k}(\F|_{\spl\backslash S_0})\simeq \Gamma(\mathcal{H}^k)=0,\quad \textrm{for } k\notin \{0,2\},\] 
and clearly  
\[H^{0}(\F|_{\spl\backslash S_0})\simeq C^{\infty}(\C^{\times}).\]
The situation in degree 2 is a bit more involved, because the rank 1 vector bundle $\mathcal{H}^2\to \C^{\times}$ is non-trivial. The leafwise symplectic structures $\omega_1$ and $\omega_2$, associated to the Poisson structures $\pi_1$ and $\pi_2$ from \eqref{eq: real identification}, induce sections
\[[\omega_1], [\omega_2]\in \Gamma(\mathcal{H}^2).\]
We will see that the vanishing loci of these sections are the positive real half-line and the negative real half-line, respectively:
\begin{align*}
&[\omega_1(z)]=0\in H^2(f^{-1}(z))\iff\quad z\in (0,\infty),\\
&[\omega_2(z)]=0\in H^2(f^{-1}(z))\iff\quad z\in (-\infty,0).
\end{align*}
So, at any point in $\C^{\times}$ at least one of $[\omega_1]$ and $[\omega_2]$ is non-zero, and therefore they span all sections: 
\[\Gamma(\mathcal{H}^2)=\big\{g_1[\omega_1]+g_2[\omega_2]\ |\ g_1,g_2\in C^{\infty}(\C^{\times})\big\}.\]
Because $\mathrm{rank}(\mathcal{H}^2)=1$, the two sections are not independent, and we will prove that they satisfy the relation:
% \begin{align*}%\label{relation:omega's}
%     y[\omega_1] = (|z|-x)[\omega_2],%, \ \ \ \ \ \text{ or equivalently } \ \ \ \ \ y[\omega_2] = (|z|+x)[\omega_1],
% \end{align*}
\begin{align}\label{relation:omega's}
    (|z|-x)[\omega_1] = -y[\omega_2],%, \ \ \ \ \ \text{ or equivalently } \ \ \ \ \ y[\omega_2] = (|z|+x)[\omega_1],
\end{align}
where $z=x+iy$. The second foliated cohomology is given by:
% \[H^{2}(\F|_{\spl\backslash S_0})\simeq 
% \Gamma(\mathcal{H}^2)\simeq \frac{C^{\infty}(\C^{\times})\oplus C^{\infty}(\C^{\times})}{\big\{(g_1,g_2)\ |\ (|z|-x) g_1=-y g_2\big\}}.\]
\[H^{2}(\F|_{\spl\backslash S_0})\simeq 
\Gamma(\mathcal{H}^2)\simeq \frac{C^{\infty}(\C^{\times})\oplus C^{\infty}(\C^{\times})}{\big\{(g_1,g_2)\ |\  yg_1=(|z|-x) g_2\big\}}.\]

\subsubsection{The twisted module}\label{subsection: twisted module}
In the previous subsection, we dealt with the non-trivial line bundle $\mathcal{H}^2\to \C^{\times}$. This bundle does not extend smoothly at the origin. However, to express flat foliated cohomology, we use as inspiration the description of $\Gamma(\mathcal{H}^2)$ above to make sense of its ``space of sections flat at the origin".

The following $C_0^{\infty}(\C)$-module will play a crucial role in this paper: 
\begin{align}\label{eq: definition M}
    \mathcal{M}\subset C^{\infty}_0(\C)\oplus C^{\infty}_0(\C),\quad \mathcal{M}:=\{(g_1,g_2)\, |\, yg_1=-(|z|+x)g_2\}.
\end{align}

For later use, let us give some properties of the module $\mathcal{M}$.


\begin{proposition}\label{proposition: twisted module}
The following hold:
\begin{enumerate}[(1)]
    \item We have an isomorphism of $C_0^{\infty}(\C)$-modules 
    $J:\mathcal{M}\diffto \mathcal{K}$, where 
\[\mathcal{K}\subset C^{\infty}_0(\C)\oplus C^{\infty}_0(\C),\quad \mathcal{K}:=\{(g_1,g_2)\, |\, yg_1=(|z|-x)g_2\},\]
given by $J(g_1,g_2)=(-g_2,g_1)$. 
    \item We have the direct sum decomposition:
    \[\mathcal{M}\oplus \mathcal{K}= C^{\infty}_0(\C)\oplus C^{\infty}_0(\C).\]
\end{enumerate}
\end{proposition}
\begin{proof}
For item (1), one uses the relation $(|z|-x)(|z|+x)=y^2$. 

The direct sum decomposition corresponds to the projections:
\begin{align}
p_{\mathcal{M}}:C^{\infty}_0(\C)&\oplus C^{\infty}_0(\C)\to \mathcal{M},\quad 
p_{\mathcal{K}}:C^{\infty}_0(\C)\oplus C^{\infty}_0(\C)\to \mathcal{K},\nonumber\\
p_{\mathcal{M}}(g_1,g_2)&:=\frac{1}{2|z|}\left((|z|+x)g_1-y g_2, -yg_1 + (|z|-x)g_2\right),\label{eq: projection m}\\
p_{\mathcal{K}}(g_1,g_2)&:=\frac{1}{2|z|}\left((|z|-x)g_1+y g_2, yg_1 + (|z|+x)g_2\right).\nonumber \qedhere
\end{align}
\end{proof}


\subsubsection{The description of the flat foliated cohomology}\label{section: result ffch}

In this subsection we describe the groups $H^{\bullet}_0(\F)$. Because of the flatness condition at the origin, which we impose on the forms, the singularity of the foliation will bring no contributions in cohomology. In fact, with some adaptations, the discussion from the previous subsection can be extended to describe the flat foliated cohomology. 

In degree zero, we obtain smooth functions on $\spl$ that are constant along the leaves of $\F$ and flat at $0$. Of course, these are precisely the Casimir functions of $(\spl,\pi)$ (described in Proposition \ref{prop:Casimirs}) that are flat at 0. We have the following isomorphism:
\[C_0^{\infty}(\C)\diffto  H^{0}_{0}(\F)\quad \quad g \mapsto e_{\varphi}(g \circ f).\]

To represent the second cohomology classes, we will need the following:
\begin{lemma}\label{lemma: extension omega}
For $i=1,2$, there exist 2-forms $\tilde{\omega}_i\in \Omega^2(\spl \setminus \{0\})$ that extend the leafwise symplectic forms $\omega_i$
\[\omega_i =\tilde{\omega}_i|_{T\F}\quad \textrm{on}\quad \spl \setminus \{0\},\]
and such that, when multiplied with $R^2=\mathrm{tr}(AA^*)$, become smooth at $0$:
\[ R^2 \cdot \tilde{\omega}_i \in \Omega^2(\spl).\]
\end{lemma}

\begin{proof}
In the coordinates from Subsection \ref{section: formal poisson}, the extensions are defined as:
\begin{align*}
    \tilde{\omega}_1:&=\frac{2}{R^2}\sum_{c.p.}
    \big(
    x_1 (\dif y_2\wedge \dif y_3-\dif x_{2}\wedge\dif x_3) -y_1 (\dif x_2\wedge \dif y_3+ \dif y_2 \wedge\dif x_3)\big)\\
&=\frac{1}{|z|^2}\sum_{c.p.}
    \Re \big(-z_1 \dif \overline{z}_2\wedge\dif \overline{z}_3\big)\\
    \tilde{\omega}_2:&=\frac{2}{R^2}\sum_{c.p.}\big(y_1(\dif y_2\wedge\dif y_3 -\dif x_{2}\wedge\dif x_{3})
    +x_1 (\dif x_{2}\wedge\dif y_3+ \dif y_2\wedge\dif x_{3})\big)\\
&=\frac{1}{|z|^2}\sum_{c.p.}
    \Im \big(-z_1 \dif \overline{z}_2\wedge\dif \overline{z}_3\big)
\end{align*}
where $\sum_{c.p.}$ denotes the sum over all cyclic permutations of the indexes $1,2,3$. A direct calculation shows that they satisfy:
\[\pi_i^{\sharp} \circ \tilde{\omega}_i^{\flat} \circ \pi_i^{\sharp} = \pi_i^{\sharp}.\]
Another way to describe $\tilde{\omega}_i$ is as following: we define the two vector fields $V_1,V_2\in \mathfrak{X}^1(\spl \setminus\{0\})$ by
\begin{align}\label{eq: v}
    V_1:=\frac{1}{R^2}\sum_{i=1}^{3}(x_{i}\partial_{x_i}-y_{i}\partial_{y_i})\quad \text{ and }\quad V_2:= \frac{1}{R^2}\sum_{i=1}^{3}(x_i\partial_{y_i}+y_i\partial_{x_i})
\end{align}

The vector fields $V_1$ and $V_2$ trivialize the normal bundle of $\F$ away from the origin as they satisfy the relations
\begin{align}\label{eq:v transversality}
    \dif f_j(V_i)=\delta_{ij}.
\end{align}
The 2-form $\tilde{\omega}_i$ is the unique extension of $\omega_i $ satisfying
\[ i_{V_j}\tilde{\omega}_i=0 \ \ \ \ \ \text{ for }\ j \in \{1,2\}.\qedhere\]
\end{proof}

The extensions from the lemma have only mild singularities at the origin, in particular, for any flat function $h\in C^{\infty}_0(\spl)$, 
\[h\cdot \tilde{\omega}_i\in \Omega^{2}_0(\spl).\]

% Next, in order to obtain unique representatives for cohomology classes, let us introduce the subalgebra: 
% \[C^{\infty}_{0,\tau}(\C):=\{g\in C^{\infty}_0(\C)\,|\, g(\overline{z})=g(z)\}.\]


The following result describes the flat foliated cohomology of $\F$, and to state it we use the $C^{\infty}_0(\C)$-modules $\mathcal{M}$ and $\mathcal{K}$ from the previous subsection.  
The proof will occupy the rest of Section \ref{section flat foli} and Section \ref{subsection: homotopy operators}.

\begin{proposition}\label{proposition:flat foliated ch}
For $k\notin \{0,2\}$, $H^k_0(\F)\simeq 0$, and 
\begin{itemize}
    \item for $k=0$, we have the isomorphism:
    \begin{equation}\label{eq: zero fol iso}
    \begin{array}{cccc}
         &C_0^{\infty}(\C)&\xrightarrow{\simeq} & H^{0}_{0}(\F)\\
         &g&\mapsto &e_{\varphi}(g \circ f)
    \end{array}
    \end{equation}
    \item for $k=2$, we have a surjective map
    \begin{equation} \label{eq: quotient}
        \begin{array}{cccc}
             &C_0^{\infty}(\C)\oplus C^{\infty}_0(\C)&\to & H^{2}_{0}(\F) \\
             &(g_1,g_2)&\mapsto & [e_{\varphi}(g_1\circ f\cdot \tilde{\omega}_1 +g_2\circ f\cdot \tilde{\omega}_2)]
        \end{array}
    \end{equation}
with kernel $\mathcal{K}$. Hence  \eqref{eq: quotient} restricts to a $C^{\infty}_0(\C)$-linear isomorphism
    \begin{equation}\label{eq:2nd:flat:foliated}
\mathcal{M} \diffto  H^{2}_{0}(\F).
    \end{equation}
    % whose kernel is
%     \[\big\{(g_1,g_2)\ |\  yg_1=(|z|-x)g_2\big\},\quad  \textrm{where}\quad z=x+yi.\]
% Moreover, the map \eqref{eq: quotient} restricts to a linear isomorphism: 
%     \begin{equation}\label{eq:2nd:flat:foliated}
% C_{0,\tau}^{\infty}(\C)\oplus C^{\infty}_{0,\tau}(\C)\simeq  H^{2}_{0}(\F).
%     \end{equation}
\end{itemize}
\end{proposition}

\begin{remark}
Note that the 2-forms
\[e_{\varphi}(g_1\circ f\cdot \tilde{\omega}_1 +g_2\circ f\cdot \tilde{\omega}_2)\in \Omega^{4}_0(\spl)\]
are independent of the chosen extensions. However, the explicit extensions were needed in order to show that these forms are indeed part of our complex.
\end{remark}


\subsubsection{Good homotopy operators}

In the second part of the paper we prove Theorem \ref{theorem: nondegenerate} using the Nash-Moser method. For this, mere descriptions of the cohomology will not suffice. We will need to construct so-called \emph{homotopy operators}, which play the role of partial inverses to the differential. To be of use in the analysis part, these maps need to satisfy a locality condition with respect to closed balls around the origin and certain estimates. We collect these properties in the following: 

\begin{definition}\label{definition: property H}
Let $V$ and $W$ be two vector bundles over an inner product space $H$ (we will only use $H=\spl$ and $H=\C$). Consider vector subspaces of sections
\[\mathscr{V}\subset \Gamma_0(V)\quad \textrm{and}\quad \mathscr{W}\subset \Gamma_0(W),\]
where $\Gamma_0(\cdot)$ denotes the space of sections that are flat at the origin. Let $\iota_r:\overline{B}_r\to H$ denotes the inclusion of the closed ball of radius $r>0$ and denote $\mathscr{V}_r:=\iota_r^*(\mathscr{V})$ and $\mathscr{W}_r:=\iota_r^*(\mathscr{W})$. After choosing trivializations of $V$ and $W$, we have norms  $\fnorm{\cdot}_{n,k,r}$ on
$\mathscr{V}_r$ and $\mathscr{W}_r$, defined for $s\in \mathscr{V}_r$
by
\begin{align}\label{eq: flat norms}
    \fnorm{s}_{n,k,r}:= \sup_{x\in \overline{B}_r}\ \sup_{a\in \N^m_0\, :\, |a|\le n}|x|^{-k}|D^a s(x)| \ \in \ [0,\infty).
\end{align}

We say that a linear operator: 
\[\ell:\mathscr{V}\to \mathscr{W}\]
satisfies \textbf{property SLB} for some $(a,b,c)\in \N_0^3$ (SLB from semi-local and bounded), if it induces linear operators $\ell_r$, for $r>0$, such that the diagrams:
\begin{equation}\label{eq: property H diagram}
    \begin{tikzpicture}[baseline= (a).base]
    \node[scale=.9] (a) at (0,0){
    \begin{tikzcd}
    \mathscr{V}\arrow{r}{\ell}\arrow{d}[swap]{\iota_r^*}& \mathscr{W} \arrow{d}{\iota_r^*}\\
    \mathscr{V}_r\arrow{r}{\ell_{r}}&\mathscr{W}_r
    \end{tikzcd}
    };
\end{tikzpicture}
\end{equation}
commute, and such that the following estimates hold
\begin{align}\label{eq: property H estimate}
    \fnorm{\ell_{r}(\alpha)}_{n,k,r}\le C\, \fnorm{\alpha}_{n+a,k+bn+c,r},\quad \forall\, \alpha\in \mathscr{V}_r,
\end{align}
for all $n,k\in \N_0$, where $C=C(r,n,k)$ depends continuously on $r$. 
\end{definition}


\begin{example} Note that any linear partial differential operator $\ell$ of degree $d$ satisfies the SLB property of $(d,0,0)$. 
\end{example}


\begin{remark}
Throughout the paper we will encounter many operators which satisfy the SLB property and we will keep track of the triples $(a,b,c)\in \N^3_0$ which appear. However, the reader may ignore their precise values, the only important thing for our proof is that the SLB property holds for some $(a,b,c)$.  
\end{remark}


\begin{remark}
The seminorms $\fnorm{\cdot}_{n,k,r}$ defined in \eqref{eq: flat norms} are equivalent to the seminorms $|\cdot|_{n,k,r}$ defined in \eqref{eq: flat norms 2} (see Subsection \ref{subsec: equivalent seminorms}).
\end{remark}

This type of operators are closed under composition. 
\begin{lemma}\label{lemma: slb property}
Let $U, V$ and $W$ be three vector bundles over an inner product space $H$ and consider two linear operators:
\begin{align*}
    \ell_1 : \mathscr{U}\subset \Gamma_0(U)\to \mathscr{V}\subset \Gamma_0(V) \quad \textrm{and}\quad \ell_2:\mathscr{V}\subset \Gamma_0(V)\to \mathscr{W}\subset \Gamma_0(W).
\end{align*}
If $\ell_i$ satisfies property SLB for $(a_i,b_i,c_i)$, $i=1,2$, then the operator $\ell_2\circ \ell_1$ satisfies property SLB for $(a_1+a_2,b_1+b_2, a_2b_1 +c_1+c_2)$.
\end{lemma}%}

To calculate the flat foliated cohomology, we will reduce the complex from \eqref{ffcomplex} to quasi-isomorphic subcomplexes. It will be useful to package this procedure into the following standard notion (see, e.g., \cite{LS87}):

\begin{definition}\label{definition: dr}
A \textbf{deformation retraction} of a complex $(C^{\bullet},d)$ consists of a \textbf{cochain projection}, i.e., a cochain map
\begin{align*}
    p:(C^{\bullet},d) \to (C^{\bullet},d) \quad \textrm{such that}\quad p\circ p=p,
\end{align*}
together with \textbf{cochain homotopies} between $p$ and $\mathrm{id}_{C}$, i.e., linear maps
\begin{align*}
    h:C^{\bullet+1}\to C^{\bullet} \quad \textrm{such that}\quad p-\mathrm{id}_{C}= h\circ d+d\circ h.
\end{align*}
\end{definition}

The conditions in the definition imply that the maps:
\[(C^{\bullet},d)\stackrel{p}{\to}(p(C^{\bullet}),d)\quad \textrm{and}\quad (p(C^{\bullet}),d)\stackrel{\mathrm{incl}}{\hookrightarrow}(C^{\bullet},d)\]
are inverses to each other in cohomology, thus we have an isomorphism:  
\[H^{\bullet}(C)\simeq H^{\bullet}(p(C)).\]

The following is the quantitative version of Proposition \ref{proposition:flat foliated ch} as it gives homotopy operators for the complex $(\CC^{\bullet},\dif)$ computing the flat foliated cohomology from \eqref{ffcomplex}. The proof will be given later. 

\begin{proposition}\label{proposition: property H fol}
There exists a deformation retraction $(p_{\F},h_{\F})$ for the complex $(\CC^{\bullet},\dif)$ such that: 
\begin{enumerate}[(1)]
    \item $\dif\circ p_{\F}=0$;
    \item $h_{\F}$ satisfies property SLB for $(0,5,35)$.
\end{enumerate} 
\end{proposition}

The first condition says that the differential vanishes on $p_{\F}(\CC^{\bullet})$. Thus, from the discussion above, every cohomology class has a unique representative in $p_{\F}(\CC^{\bullet})$, and so we have an isomorphism:
\[p_{\F}(\CC^{\bullet})\simeq H^{\bullet}_{0}(\F).\]

The second condition together with the homotopy relation imply that also $p_{\F}$ satisfies property SLB, but for $(1,5,40)$. In particular all these operators can be restricted to closed balls centered at the origin. 

\subsection{Averaging the $SU(2)$-action}\label{section: su2 average}

The operators from Proposition \ref{proposition: property H fol} will be constructed in two steps. In this subsection, we perform the first step: we average with respect to the action of $SU(2)\subset SL(2,\C)$. Consider the operator 
\[p_{SU(2)}:\Omega^{\bullet}(\spl)\to \Omega^{\bullet}(\spl),\]
\[\alpha\mapsto \int_{SU(2)}\Ad_{U}^*(\alpha)\mu(U),\]
where we integrate with respect to the normalized Haar measure $\mu$ on $SU(2)$. We show that $p_{SU(2)}$ induces a deformation retraction of the subcomplex computing flat foliated cohomology. %\ref{section: invariant cohomology}.

\begin{proposition}\label{proposition: invariance skeleton}
There are operators $h_{SU(2)}$ such that $(p_{SU(2)},h_{SU(2)})$ is a deformation retraction of $(\Omega^{\bullet}(\spl),\dif)$. Moreover, this pair restricts to a deformation retraction of $(\CC^{\bullet},\dif)$, and both restricted maps satisfy property SLB for $(0,0,0)$.
\end{proposition}
\begin{remark}
The proof follows a general method for constructing homotopy operators for actions of compact and connected groups on complexes, which we have learned from \cite{VV14}. We have discussed this method in some greater generality in \cite{thesis_Florian}, here we apply it explicitly to the case of $SU(2)$.
\end{remark}

\begin{proof}
It follows easily that 
%Clearly, $p_{SU(2)} \dif=\dif p_{SU(2)}$ and $p_{SU(2)}^2=p_{SU(2)}$. So 
$p_{SU(2)}$ is a cochain projection of the complex $(\Omega^{\bullet}(\spl),\dif)$ whose image is the $SU(2)$-invariant subcomplex. 

Next, consider the pullback of the Haar measure (which we regard as a volume form, after choosing an orientation) to $\mathfrak{su}(2)$ via the exponential:
\[ \lambda:=\exp^*(\mu)\in \Omega^3(\mathfrak{su}(2)).\]

One easily checks (see e.g.\ \cite[Section 1.5]{DK}) that the exponential map of $SU(2)$ restricts to a diffeomorphism: 
    \[\exp:\mathcal{I}\diffto SU(2)\backslash\{-\mathds{1}\},\]
    where $\mathcal{I}\subset \mathfrak{su}(2)$
denotes the open ball of radius $\sqrt{2}\pi$ with respect to the norm $|X|=\sqrt{\mathrm{tr}(XX^*)}$ and on the boundary it satisfies \[\exp (\partial\mathcal{I})=\{-\mathds{1}\}.\]
This allows us to write:
\[p_{SU(2)}(\alpha)=\int_{SU(2)}\Ad_{U}^*(\alpha)\mu(U) 
=\int_{\overline{\mathcal{I}}}\Ad_{\exp(X)}^*(\alpha)\lambda(X).
\]
Denote by $\mathrm{ad}_X\in \mathfrak{X}^1(\spl)$ the vector field whose flow is $\Ad_{\exp(tX)}$, i.e.\
\[\mathrm{ad}_X(A):=[X,A].\]
Then, using Cartan's formula, we have that:
\[\frac{\dif}{\dif t}\Ad_{\exp(tX)}^*(\alpha)=\dif \Ad_{\exp(tX)}^* i_{\mathrm{ad}_X}(\alpha)+
\Ad_{\exp(tX)}^* i_{\mathrm{ad}_X}\dif (\alpha).
\]
This implies that:
\begin{align*}
p_{SU(2)}(\alpha)-\alpha
=&\int_{\overline{\mathcal{I}}}\big(\Ad_{\exp(X)}^*(\alpha)-\alpha\big)\lambda(X)\\
=&\int_{\overline{\mathcal{I}}}\int_0^1
\frac{\dif}{\dif t}\Ad_{\exp(tX)}^*(\alpha)\, \dif t\lambda(X)\\
=&\dif 
\int_{\overline{\mathcal{I}}}\int_0^1 \Ad_{\exp(tX)}^* i_{\mathrm{ad}_X}(\alpha)\dif t\lambda(X)\\
&+\int_{\overline{\mathcal{I}}}\int_0^1 \Ad_{\exp(tX)}^* i_{\mathrm{ad}_X}(\dif \alpha)\dif t\lambda(X).
\end{align*}
Thus, if we define:
\[h_{SU(2)}(\beta):=\int_{\overline{\mathcal{I}}}\int_0^1 \Ad_{\exp(tX)}^* i_{\mathrm{ad}_X}(\beta)\dif t\lambda(X),
\]
then we obtain the homotopy relation:
\[p_{SU(2)}(\alpha)-\alpha=\dif h_{SU(2)}(\alpha)+h_{SU(2)}(\dif \alpha).\]

Next, let us note that both $p_{SU(2)}$ and $h_{SU(2)}$ preserve
\[\CC^{\bullet}=e_{\varphi}(\Omega^{\bullet}_0(\spl))\subset \Omega^{\bullet+2}(\spl).\]
This follows because $\varphi=\dif f_1\wedge\dif f_2$ is $SU(2)$-invariant, and also satisfies $i_{\mathrm{ad}_X}\varphi=0$, and because the action fixes the origin. 

Next, since the $SU(2)$-action preserves the metric on $\spl$, it follows that both operators induce operators above closed balls around the origin, i.e.\ the first condition of property SLB holds. The inequalities from the second condition follow by using the explicit form of the norms.
\end{proof}


% \begin{lemma}
% We have that 
% \[h_{SU(2)}^2=0,\quad h_{SU(2)}\circ p_{SU(2)}=0,\quad p_{SU(2)}\circ h_{SU(2)}=0.\]
% \end{lemma}

\subsection{The ``cohomological skeleton'' $\mathfrak{S}$} \label{section: skeleton}

The main ingredient to calculate the flat foliated cohomology is what we call the ``cohomological skeleton'' $\mathfrak{S}$ associated with the foliation $\F$. One may think of $\Sk$ as an object that contains the cohomological information of the closed leaves of $\F$. In our case, we will see that this is satisfied by the set of normal matrices, and so we define the \textbf{cohomological skeleton} as 
\begin{align*}
\Sk :=\{ A\in \spl |[A,A^*]=0\}.
\end{align*}

This subsection is divided as follows. We first give an alternative descriptions of $\Sk$, then we give an explicit continuous projection map $r_{\Sk}$ from $\mathfrak{sl}_2(\C)$ onto $\Sk$ and study its properties, then we show that the smooth locus of $\Sk$ is an embedded submanifold and we find a desingularization for $\Sk$. 

\subsubsection{Characterizations of $\Sk$}

To give other descriptions of $\Sk$, we first recall some basic linear algebra. Since any $A\in \spl$  satisfies its own characteristic equation, we have
\begin{equation}\label{eq:invariant polynomials a}
    \begin{array}{rcc}
          A^2 = -f\mathds{1}, \  & &\  (A^*)^2=-\overline{f}\mathds{1}, 
    \end{array}
\end{equation}
The standard norm squared on $\mathfrak{sl}_2(\C)$ is given by
\begin{align}\label{eq:norm}
  R^2=R(A) ^2&:= |A|^2= \tr(A A^*). %more convenient without the half for everything later in estimates
\end{align}
For $A\in \spl$, the characteristic equation of $AA^*$ is: 
\begin{align}\label{eq:invariant polynomials aah}
    (AA^*)^2- R^2 AA^*+\nf^2\mathds{1}=0.
\end{align}
Since $AA^*$ has real eigenvalues, the discriminant of this equation is positive, which implies the following very useful inequality:
\begin{equation}\label{eq:norm-fiber inequality}
   2\nf\leq R^2.
\end{equation}
% \begin{align*}
%     \nf =\det(AA^*)^{\frac{1}{2}}\le &\ \frac{1}{2}\tr(AA^*)=\frac{1} {2}R^2
% \end{align*}
% Solving the characteristic equation, we find the eigenvalues of $AA^*$ to be: 
% \begin{equation}\label{eigen_S}
% \frac{R^2\pm \sqrt{R^4-4|f|^2}}{2}.
% \end{equation}

Normal matrices can be described as follows.
\begin{lemma}\label{lemma: characterization skeleton}
For $A\in \spl$ the following are equivalent:
\begin{enumerate}[(1)]
    \item $A\in \Sk$
    \item $A$ is unitarily diagonizable
    \item $R^2=2|f|$
    \item $AA^*=\nf \mathds{1}$.
\end{enumerate}
\end{lemma}
\begin{proof}
The equivalence (1)$\iff$ (2) is the content of the spectral theorem.

Next, by Schur's decomposition theorem, any $A\in \spl$ is unitary equivalent to an upper triangular matrix $\Lambda$:
\[ A=U\Lambda U^{*}, \quad U\in SU(2), \quad   \Lambda =\begin{pmatrix}
     \lambda_{11} & \lambda_{12} \\
     0&-\lambda_{11}
     \end{pmatrix}\]
Using this, we obtain the following expression for $|f|$:
\begin{align*}
    \nf  =\det(AA^*)^{\frac{1}{2}} = \det(\Lambda \Lambda^*)^{\frac{1}{2}}=|\lambda_{11}|^2
\end{align*}
and for the norm of $A$ we find: 
\begin{align*}
    R^2 =|A|^2=\tr(AA^*)=\tr(\Lambda \Lambda^*) = 2|\lambda_{11}|^2+ |\lambda_{12}|^2.
\end{align*}
Thus, $R^2=2|f|$ if and only if $\lambda_{12}=0$, i.e., $\Lambda$ is diagonal. This proves the implication (3) $\implies$ (2). The other implications: 
\[ (2)\ \  \implies  \ \ (4)\ \  \implies  \ \ (3) \]
are immediate. 
\end{proof}


\subsubsection{The retraction to the cohomological skeleton}\label{subsubsec_retraction}
The goal of this subsection is to define a continuous retraction $r_{\Sk}$ from $\spl$ onto $\Sk$ and study its properties. In Section \ref{subsection: homotopy operators} we will realize $r_{\Sk}$ as the infinite flow of a vector field.

First, we introduce the smooth function:
\begin{equation*}
    \begin{array}{cccc}
         g_{\infty} :&\spl \setminus S_0&\to &\herm(\C) \\
         & A&\mapsto&\left(\mathds{1}+\frac{1}{\nf}AA^*\right)^{\frac{1}{2}}
    \end{array}
\end{equation*}
where $\herm(\C)$ denotes the set of positive definite Hermitian $2\times 2$-matrices. In defining this map, we used the diffeomorphism: 
\[\sqrt{\cdot}: \herm(\C)\to \herm(\C).\]
Note that elements in $\herm(\C)$ are invertible. Define the retraction: 
\begin{align}\label{retract}
r_{\Sk}&:\spl \to \Sk\subset \spl\nonumber \\
r_{\Sk} (A)&:=
   \begin{cases}
    g_{\infty}(A)^{-1}Ag_{\infty}(A)&\text{ if } f(A)\ne 0\\
    0&\text{ if } f(A)= 0
\end{cases}
\end{align}

\begin{lemma}\label{lemma:properties of p}
The map $r_{\Sk}$ is a projection onto $\Sk$:
\[r_{\Sk}(\spl)=\Sk \quad \textrm{and}\quad r_{\Sk}|_{\Sk}=\mathrm{id}_{\Sk},\]
and has the following properties: 
it is continuous on $\spl$ and smooth on $\spl\setminus S_0$, it is $SU(2)$-equivariant and it preserves the fibers of $f$.
\end{lemma}
\begin{proof}
We first check that the image of $r_{\Sk}$ lies indeed inside of $\Sk$. Note that by \eqref{eq:invariant polynomials a} we have the identity
\begin{align*}
    A \ g_{\infty}(A)^{2}A^*  =&\ AA^*+\nf \mathds{1}  = \nf \,  g_{\infty}(A)^{2},
\end{align*}
and therefore:
\begin{equation}\label{eq: retraction well-defined}
    r_{\Sk}(A)r_{\Sk}(A)^* = \ g_{\infty}(A)^{-1}A \ g_{\infty}(A)^{2}A^* g_{\infty}(A)^{-1}= \nf\, \mathds{1}.
\end{equation}
We easily obtain that $r_{\Sk}$ preserves $f$
% \[f(r_{\Sk}(A))=-\det (r_{\Sk}(A))= -\det (A) =f(A),\]
\[f(r_{\Sk}(A))=\det (r_{\Sk}(A))= \det (A) =f(A),\]
and therefore Lemma \ref{lemma: characterization skeleton} (4) and \eqref{eq: retraction well-defined} imply that $r_{\Sk}(A)\in \Sk$. 

Next, for $A\in \Sk\backslash S_0$, again by Lemma \ref{lemma: characterization skeleton} (4), we have that $g_{\infty}(A)=\sqrt{2}\mathds{1}$, and so $r_{\Sk}(A)=A$. Since $\Sk\cap S_0=\{0\}$,
we conclude that $r_{\Sk}|_{\Sk}=\id_{\Sk}$.



Using again \eqref{eq: retraction well-defined} we obtain
\[ \lvert r_{\Sk}(A)\rvert^2 =2\nf,\]
which proves continuity of $r_{\Sk}$ at points in $S_0\subset \spl$. Continuity and smoothness on the set $\spl\setminus S_0$ follow from the formula of $r_{\Sk}$ on this set. That $r_{\Sk}$ is $SU(2)$-equivarients follows immediately. 
\end{proof}


\subsubsection{The cochain projection associated to $r_{\Sk}$}

Even though $r_{\Sk}$ is not smooth along $S_0$, we will show in Section \ref{subsection: homotopy operators} that it induces a pullback map on flat forms:
\begin{lemma}\label{lemma: infinite time pullback}
For every $\alpha \in \Omega_{0}^{\bullet}(\spl)$, the form $r_{\Sk}^*(\alpha)|_{\spl\backslash S_0}$ extends to a smooth form on $\spl$, which is flat at $0$:
\[p_{\Sk}(\alpha)\in \Omega^{\bullet}_0(\spl).\]
\end{lemma}

By Lemma \ref{lemma:properties of p}, $r_{\Sk}^2=r_{\Sk}$, and therefore $p_{\Sk}$ is a cochain projection:
\[p_{\Sk}:(\Omega^{\bullet}_0(\spl),\dif)\to (\Omega^{\bullet}_0(\spl),\dif).\] 
The same lemma also implies that $p_{\Sk}$ commutes with $e_{\varphi}$ (it suffices to check this away from $S_0$), therefore $p_{\Sk}$ restricts to a cochain projection of $(\CC^{\bullet},\dif)$. 

The proof of the following proposition will occupy most of Section \ref{subsection: homotopy operators}:

\begin{proposition}\label{lemma: homotopies}
There are operators $h_{\Sk}$ such that $(p_{\Sk},h_{\Sk})$ is a deformation retraction of $(\Omega^{\bullet}_0(\spl),\dif)$. Moreover, this pair restricts to a deformation retraction of $(\CC^{\bullet},\dif)$, and $h_{\Sk}$ satisfies property SLB for $(0,5,35)$.
\end{proposition}

By combining the operators from Propositions \ref{proposition: invariance skeleton} and \ref{lemma: homotopies} we obtain the deformation retraction from Proposition \ref{proposition: property H fol} (for such compositions, see e.g.\ \cite[Lemma 2.4]{LS87})

\begin{corollary}\label{corollary:chain:proj} 
The pair $(p_{\F},h_{\F})$ defined by 
\[p_{\F}:=p_{SU(2)}\circ p_{\Sk} \quad \text{and}\quad h_{\F}:=p_{SU(2)}\circ h_{\Sk}+h_{SU(2)}\]
is a deformation retraction for the complex $(\CC^{\bullet},\dif)$, and $h_{\F}$ satisfies property SLB for $(0,5,35)$.
\end{corollary}
\begin{proof}
By Lemma \ref{lemma:properties of p}, $r_{\Sk}$ is $SU(2)$-equivariant, and this implies that $p_{\Sk}$ and $p_{SU(2)}$ commute. Hence $p_{\F}$ is a cochain projection. The homotopy relation follows easily: 
\begin{align*}
p_{\F}-\mathrm{id}=&p_{SU(2)}(p_{\Sk}-\mathrm{id})+p_{SU(2)}-\mathrm{id}\\
=&p_{SU(2)}(\dif h_{\Sk}+h_{\Sk}\dif )+\dif h_{SU(2)}+ h_{SU(2)}\dif \\
=&\dif (p_{SU(2)} h_{\Sk}+ h_{SU(2)})+(p_{SU(2)}h_{\Sk}+h_{SU(2)})\dif\\
=&\dif h_{\F }+ h_{\F}\dif.
\end{align*}
Property SLB for the original operators implies it for $h_{\F}$. 
\end{proof}

In the following subsections, we will see that $\dif\circ p_{\F}=0$, which will conclude the proof of Proposition \ref{proposition: property H fol}.



\subsubsection{A desingularization of $\Sk$}\label{section: descing skeleton}

The skeleton $\Sk$ is a smooth submanifold away from $0$. In this subsection, we construct a desingularization for $\Sk$. 

First note that, by Lemma \ref{lemma: characterization skeleton} (2), $\Sk$ is precisely the image of the map: 
% \begin{equation*}\label{eq:surjective map}
%     \begin{array}{cccc}
%          \widehat{\rho}:&SU(2)\times \C &\to &\spl  \\
%          &(U,\lambda)&\mapsto& U \begin{pmatrix}
%          \lambda&0\\
%          0&-\lambda
%          \end{pmatrix}U^*
%     \end{array}
% \end{equation*}
\begin{equation*}\label{eq:surjective map}
    \begin{array}{cccc}
         \widehat{\rho}:&SU(2)\times \C &\to &\spl  \\
         &(U,\lambda)&\mapsto& U \begin{pmatrix}
         i\lambda&0\\
         0&-i\lambda
         \end{pmatrix}U^*
    \end{array}
\end{equation*}
This map is invariant under the right action on $SU(2)$ of the subgroup 
\[\Big\{
\begin{pmatrix}
          z&0\\
          0&\overline{z}
         \end{pmatrix}\, |\, z\in S^1
\Big\}.\]
Therefore, the map descends to a map on the quotient:
\[\rho: S^2\times \C \to \spl,\]
where we identify $SU(2)/S^1\simeq S^2$ via the Hopf fibration:
% \begin{equation}\label{eq:Hopf}
%          \begin{pmatrix}
%          a&b\\
%          -\overline{b}&\overline{a}
%          \end{pmatrix} \mapsto (2ab,\lvert a\rvert^2 -\lvert b\rvert^2),
% \end{equation}
\begin{equation}\label{eq:Hopf}
         \begin{pmatrix}
         a&b\\
         -\overline{b}&\overline{a}
         \end{pmatrix} \mapsto (\lvert a\rvert^2 -\lvert b\rvert^2,\Im(-2ab),\Re(-2ab)),
\end{equation}
where we regard $S^2\subset \R^3$. For later use, let us note that, if we use coordinates $w=(w_1,w_2,w_3)\in S^2\subset \R^3$, then $\rho$ is given by
\begin{equation}\label{eq:cohomology map}
    \rho(w,\lambda)=\begin{pmatrix}
         i\lambda \cdot w_1 &\lambda \cdot (-w_2+iw_3)\\
         \lambda \cdot (w_2+iw_3)&-i\lambda \cdot w_1
         \end{pmatrix}
\end{equation}
% \begin{equation}\label{eq:cohomology map}
%     \rho(y,\lambda)=\begin{pmatrix}
%          \lambda \cdot y_3 &-\lambda \cdot (y_1 +i y_2)\\
%          -\lambda \cdot (y_1 -i y_2)&-\lambda \cdot y_3
%          \end{pmatrix}
% \end{equation}

\begin{lemma}\label{lemma:identification of skeleton}
The map $\rho$ has the following properties:
\begin{enumerate}[(1)]
\item $\rho$ is $SU(2)$-equivariant for the natural left action on $S^2\simeq SU(2)/S^1$ and the action on $\spl$ by conjugation;
\item $f\circ \rho(w,\lambda)=\lambda^2$, and so the preimages of the leaves of $\F$ are given by 
\[\rho^{-1}(S_z)=S^2\times\big\{\pm\sqrt{z}\big\},\]
where $\pm\sqrt{z}$ are the two square roots of $z\in \C$;
%\item $\mathrm{im}(\rho)=\Sk$;
\item $\rho$ descends to a smooth map 
\[\underline{\rho}:S^2\times_{\Z_2}\C\to \spl,\]
where $\Z_2$ acts on $S^2\times \C\subset \R^5$ by multiplication with $-1$; 
\item the regular part of the skeleton $\Sk^{\textrm{reg}}:=\Sk\backslash\{0\}$ is an embedded submanifold of $\spl$ and 
$\underline{\rho}$ restricts to a diffeomorphism:
\begin{equation}\label{eq:desingularization}
\underline{\rho}:S^2\times_{\Z_2}\C^{\times}\diffto \Sk^{\text{reg}}.
    \end{equation}
\end{enumerate}
\end{lemma}

\begin{remark}
We think of the map $\underline{\rho}:S^2\times_{\Z_2}\C\to \Sk$ as a \textbf{desingularization} of the skeleton. However, for calculations it will be more convenient to use the map $\rho$.
\end{remark}

\begin{proof}
Items (1), (2) and (3) are immediate. An easy way to show that $\Sk^{\textrm{reg}}$ is an embedded submanifold is to note that, because $\Sk=\mathrm{im}(\widehat{\rho})$, it follows that $\Sk^{\mathrm{reg}}$ is the preimage under the submersion:
\[\mathrm{pr}:\spl\backslash\{0\}\to \mathbb{CP}(\spl)\]
of a (compact!) orbit of the induced $SU(2)$-action. % through the element
%\[\mathrm{pr}\begin{pmatrix}
%1 &0 \\
%0& -1
%\end{pmatrix}\in \mathbb{CP}(\spl).\]

% To show that $\Sk^{\textrm{reg}}$ is an embedded submanifold, we show that it is locally given by the fibers of a submersion. For this, note that for $A=(a_{ij})_{1\le i,j\le 2}\in \spl$ we have
% \begin{align*}
%     [A,A^*]=&\ \begin{pmatrix}
%     |a_{12}|^2-|a_{21}|^2&2(a_{11}\overline{a}_{21}-\overline{a}_{11}a_{12})\\
%     2(\overline{a}_{11}a_{21}-a_{11}\overline{a}_{12})&|a_{21}|^2-|a_{12}|^2
%     \end{pmatrix}
% \end{align*}
% Consider the following map: 
% \begin{equation*}
%     \begin{array}{cccc}
%          h:&\spl &\to &\C \\
%          &A&\mapsto & a_{11}\overline{a}_{21}-a_{12}\overline{a}_{11} 
%     \end{array}
% \end{equation*}
% Note that the restriction of $h$ to the open subset $\mathcal{O}:= \{a_{11}\ne 0\}$ is a submersion, and note also that:
% \[\mathcal{O}\cap h^{-1}(0)=\mathcal{O}\cap\Sk^{\textrm{reg}}.\]
% Therefore, $\mathcal{O}\cap \Sk^{\textrm{reg}}$ is an embedded submanifold. Next, for an element 
% $A\in \Sk^{\textrm{reg}} \setminus \mathcal{O}$, we can always find an element $U\in SU(2)$ such that 
% \[ \Ad_U (A)=UAU^*\in \mathcal{O}.\]
% Since conjugation by $U$ leaves $\Sk^{\textrm{reg}}$ invariant, $\Sk^{\textrm{reg}}$ is given around $A$ as the fiber of the submersion $m\circ \Ad_U: \Ad_{U^*}(\mathcal{O})\to \C$. Thus, we obtain that $\Sk^{\textrm{reg}}$ is an embedded submanifold.


For the last part, we first show that \eqref{eq:desingularization} is a bijection. Surjectivity follows because the image of $\widehat{\rho}$ is $\Sk$. To show injectivity, we need to understand when two elements $(U,\lambda),(\tilde{U},\tilde{\lambda})\in SU(2)\times \C $ have the same image under $\widehat{\rho}$. First, by comparing the determinants, we have that $\lambda=\pm \tilde{\lambda}$. For $\lambda =\tilde{\lambda}\ne 0$, note that the centralizer of the matrix \[\begin{pmatrix}
\lambda &0 \\
0& -\lambda
\end{pmatrix}\]
in $SU(2)$ the subgroup
\[S^1\simeq \Big\{ V(\mu):= \begin{pmatrix}
\mu&0\\
0&\overline{\mu}
\end{pmatrix}
| \ \mu \in S^1\Big \}.\]
In the case $\lambda =-\tilde{\lambda}\ne 0$ we use that 
\[ \begin{pmatrix}
\lambda &0 \\
0& -\lambda
\end{pmatrix}= \gamma \begin{pmatrix}
-\lambda &0 \\
0& \lambda
\end{pmatrix}\gamma^*, \quad \text{where}\quad  \gamma :=\begin{pmatrix}
0&1\\
-1&0
\end{pmatrix}\]
Using these, we obtain for $\lambda\neq 0$:
\[ \widehat{\rho}(U,\lambda)=\widehat{\rho}(\tilde{U},\tilde{\lambda}) \ \  \Longleftrightarrow \ \   \exists\, \mu \in S^1 , i\in \{0,1\}\, : \,  (\tilde{U},\tilde{\lambda} )=(UV(\mu)\gamma^i ,(-1)^i\lambda).\]
By first taking the quotient modulo $S^1$, and identifying $SU(2)/S^1\simeq S^2$ via \eqref{eq:Hopf}, we obtain that $\widehat{\rho}$ descends to $\rho$. Next, using the relation 
\[ V(\mu)\gamma = \gamma V(-\overline{\mu}).\]
we obtain that the right action of $\gamma$ on $SU(2)$ induces a well-defined $\Z_2$-action on $SU(2)/S^1$, which under the map \eqref{eq:Hopf} becomes multiplication by $-1$ on $S^2$. Hence, we obtain for $\lambda\neq 0$ that:
\[\rho(w,\lambda)=\rho(\tilde{w},\tilde{\lambda}) \ \  \Longleftrightarrow \ \  (\tilde{w},\tilde{\lambda} )=(\pm w ,\pm \lambda).\]
This implies that \eqref{eq:desingularization} is injective. 

Next, it is easy to see that the restriction of $\rho$ to $S^2\times \C^{\times}$ is an immersion. This implies that the map from \eqref{eq:desingularization} is an injective immersion whose image is $\Sk^{\mathrm{reg}}$. But since $\Sk^{\mathrm{reg}}$ is an embedded submanifold, it follows that \eqref{eq:desingularization} is a diffeomorphism.
\end{proof}

\subsubsection{Using the desingularization to calculate cohomology}\label{subsection:desing}

By Corollary \ref{corollary:chain:proj}, the flat foliated cohomology $H^{\bullet}_0(\F)$ can be computed using the subcomplex $p_{\F}(\CC^{\bullet})\subset \CC^{\bullet}$. In this subsection, we will describe this subcomplex by using the desingularization map $\rho$. As a consequence we obtain the description of the flat foliated cohomology from Proposition \ref{proposition:flat foliated ch} and also conclude the proof of Proposition \ref{proposition: property H fol}. 


To describe the result, we first discuss the behavior of flat functions on $\C$ under pullback along the map:
\[\sigma:\C\to \C, \quad \sigma(\lambda)=-\lambda.\]%,\quad\quad  \tau:\C\to \C,\quad \tau(\lambda)=\overline{\lambda}.\]
Consider the eigenspaces: 
%of the pullback along these maps:% To describe the result, we first discuss flat functions on $\C$ invariant under multiplication by $-1$, denoted $\sigma:\C\to \C$, and under the conjugation map, denoted $\tau:\C\to \C$. Consider the eigenspaces of the pullback along these maps:
\[C^{\infty}_{0,\pm \sigma}(\C):=\{g\in C^{\infty}_0(\C)\,|\, g=\pm \sigma^*(g)\},\]
%\[C^{\infty}_{0,\pm\tau}(\C):=\{g\in C^{\infty}_0(\C)\,|\, g=\pm \tau^*(g)\}.\]

The following properties of these spaces will be proven in Appendix \ref{eigenspaces}:
\begin{lemma}\label{lemma:pullbacks and invariant functions}
\begin{enumerate}[(1)]
    \item The following map is an isomorphism of rings: 
    \[C^{\infty}_0(\C)\diffto C^{\infty}_{0,\sigma}(\C)\]
    \[g\mapsto g\circ \mathrm{sq}, \quad \textrm{where}\quad \mathrm{sq}(\lambda):=\lambda^2.\]
    \item The following map is surjective:
    \begin{equation*}
        \begin{array}{cccc}
             & C^{\infty}_0(\C)\oplus C^{\infty}_0(\C) &\to &C^{\infty}_{0,-\sigma}(\C)\\
             &(g_1,g_2)&\mapsto &-\lambda_1\cdot g_1\circ \mathrm{sq}+\lambda_2\cdot g_2\circ \mathrm{sq},
        \end{array}
    \end{equation*} 
where $\lambda_1+i\lambda_2=\lambda$, and its kernel is given by $\mathcal{K}$.
\item The map from (2) restricts to a linear isomorphism:
\[\mathcal{M} \diffto C^{\infty}_{0,-\sigma}(\C).\]
\end{enumerate}
\end{lemma}

\vspace{-5pt}
Next, we introduce the complex:
\[(\DD^{\bullet},\dif)\subset 
(\Omega^{\bullet+2}(S^2\times \C),\dif)
\]
given by
\begin{equation}\label{eq: foliated complex skeleton}
\DD^{k} = \left\{\begin{array}{lr}
        C^{\infty}_{0,\sigma}(\C)\, \rho^*(\varphi), & \text{for } k=0\\
       \quad\quad \quad 0, & \text{for } k=1\\
        C^{\infty}_{0,-\sigma}(\C)\, \rho^*(\varphi)\wedge \omega_{S^2}, & \text{for } k=2
        \end{array}\right.
\end{equation}
where we regard functions on $\C$ as functions on $S^2\times\C$ via the pullback along the second projection and $\omega_{S^2}$ is the standard area form on $S^2$
\begin{align}\label{eq: standard form s2}
    \omega_{S^2}= \sum_{c.p.}w_1 \dif w_2\wedge \dif w_3
\end{align}
Clearly, $\DD^{\bullet}$ consists only of closed forms. Note that, by Lemma \ref{lemma:identification of skeleton} (2),
\begin{equation}\label{eq:pull back of varphi}
    \rho^*(\varphi)=4(\lambda_1^2+\lambda_2^2)\dif \lambda_1\wedge \dif \lambda_2.
\end{equation}



We have the following:

\begin{proposition}\label{proposition: chain isomorphism}
The map $\rho^*$ restricts to a cochain isomorphism:
\[\rho^*:(p_{\F}(\CC^{\bullet}),\dif)\diffto (\mathscr{D}^{\bullet},\dif=0).\]
\end{proposition}

\begin{proof}
We split the proof into several steps:
\smallskip

\noindent\underline{Step 1}: Injectivity. Let $\alpha\in p_{\F}(\CC^{\bullet})$ such that $\rho^*(\alpha)=0$. Recall that, by Lemma \ref{lemma:identification of skeleton}, $\rho:S^2\times \C^{\times}\to \Sk^{\textrm{reg}}$ is a 2-to-1 covering map, and therefore $i^*(\alpha)=0$, where $i:\Sk^{\textrm{reg}}\hookrightarrow\spl$ denotes the inclusion. Since $r_{\Sk}(\spl\backslash S_0)=\Sk^{\textrm{reg}}$, it follows that $r_{\Sk}^*(\alpha)|_{\spl\backslash S_0}=0$, and so $p_{\Sk}(\alpha)=0$. Since $\alpha\in p_{\F}(\CC^{\bullet})$, we have that:
\[\alpha=p_{\F}(\alpha)=p_{SU(2)}\circ p_{\Sk}(\alpha)=0.\]
This proves injectivity.
\smallskip

\noindent\underline{Step 2}: $\mathrm{Im}(\rho^*)\subset \mathscr{B}^{\bullet}$, where we denote 
\begin{align*}
    \mathscr{B}^{\bullet}:=e_{\rho^*(\varphi)}(\Omega^{\bullet}_0(S^2\times \C))^{SU(2)\times \Z_2}\subset \Omega^{\bullet+2}(S^2\times \C),
\end{align*} 
and the subscript $_0$ stands for forms flat at $S^2\times\{0\}$. Note that, since the action of $SU(2)\times \Z_2$ on $S^2\times\C$ preserves the submanifold $S^2\times \{0\}$, the subcomplex in \eqref{eq: foliated complex skeleton} is well-defined. Note that also $\rho^*(\varphi)$ is $\Z_2$-invariant. 

Step 2 is a consequence of the following facts: elements in $p_{\F}(\CC^{\bullet})$ are $SU(2)$-invariant, all elements in the image of $\rho^*$ are $\Z_2$-invariant, elements in $p_{\F}(\CC^{\bullet})$ are flat at the origin and $\rho(S^2\times \{0\})=0$.

\smallskip

\noindent\underline{Step 3}: $\DD^{\bullet}=\mathscr{B}^{\bullet}$. Clearly, $\DD^{\bullet}\subset \mathscr{B}^{\bullet}$. For the converse, note that 
\[\Omega^k(S^2)^{SU(2)} = \left\{\begin{array}{lr}
        \R, & \text{for } k=0\\
    0, & \text{for } k=1\\
        \R\, \omega_{S^2}, & \text{for } k=2
        \end{array}\right.\]
Next, note that if we evaluate any $\alpha \in \mathscr{B}^{k}$ along $S^2\times \{\lambda\}$, we obtain: 
\[ \alpha|_{S^2\times \{\lambda\}} = \rho^*(\varphi)_{\lambda}\wedge \beta,\]
with $\beta\in \Omega^k(S^2)^{SU(2)}$. This implies that $\mathscr{B}^1=0$. For $k=0$ we immediately obtain $\alpha=h\, \rho^*(\varphi)$, with $h\in C^{\infty}_{0,\sigma}(\C)$. For $k=2$, we obtain that $\alpha=h\, \rho^*(\varphi)\wedge \omega_{S^2}$. Since $\gamma^*(\omega_{S^2})=-\omega_{S^2}$, where $\gamma(w)=-w$, it follows that $h\in C^{\infty}_{0,-\sigma}(\C)$.

\smallskip

\noindent\underline{Step 4}: $\DD^{\bullet}\subset \mathrm{Im}(\rho^*)$. In degree 0, by Lemma \ref{lemma:pullbacks and invariant functions}, every element in $\DD^0$
can be written as $e_{\rho^*(\varphi)}(g\circ \mathrm{sq})$, for some $g\in C^{\infty}_0(\C)$. By Lemma \ref{lemma:identification of skeleton} (2):
\begin{equation*}%\label{eq:pullback rho casimirs}
\rho^*(e_{\varphi}(g\circ f))=e_{\rho^*(\varphi)}(g\circ \mathrm{sq}).
\end{equation*}
Next, since $f$ is $SU(2)$-invariant and $r_{\Sk}$ preserves $f$, we have that 
\[p_{\F}(e_{\varphi}(g\circ f))=e_{\varphi}(g\circ f),\]
which proves the statement in degree 0.

For degree 2, we recall first the explicit form of $\rho$ from \eqref{eq:cohomology map}
\begin{align}\label{eq:cohomology map explicit}
\rho(w_1,w_2,w_3,\lambda)=(z_1,z_2,z_3), \quad z_j = \lambda\cdot w_j %\quad \Longleftrightarrow \quad (x_j,y_j)=(\lambda_1 \cdot w_j ,\lambda_2 \cdot w_j),
\end{align}
where we use the coordinates $z_j=x_j+iy_j$ on $\spl$ from Section \ref{section: formal poisson}. Using these in the explicit formula for $\tilde{\omega}_{i}$ from Lemma \ref{lemma: extension omega}, we have: 
\begin{align*}
\rho^*(\tilde{\omega}_1+i\tilde{\omega}_2)&=\rho^*\Big(-\frac{1}{|z|^2}\sum_{c.p.}
    z_1 \dif \overline{z}_2\wedge\dif \overline{z}_3\Big)\\
    &=-\frac{1}{|\lambda|^2}\sum_{c.p.}
    w_1 \lambda (\overline{\lambda} \dif w_2 +w_2\dif\overline{\lambda})\wedge
    (\overline{\lambda} \dif w_3 +w_3\dif\overline{\lambda})\\
&=-\sum_{c.p.} \overline{\lambda}\, w_1 \dif w_2\wedge \dif w_3+ w_1(w_3\dif w_2-w_2\dif w_3)\wedge\dif \overline{\lambda}\\
&=-\overline{\lambda}\,\omega_{S^2}.
\end{align*}
Hence, we obtain:
\begin{equation}\label{eq:pullback forms}
    \begin{array}{rcl}
         \rho^*(\tilde{\omega}_1)&=&-\lambda_1\, \omega_{S^2}\\ \rho^*(\tilde{\omega}_2)&=&\lambda_2\, \omega_{S^2}.
    \end{array}
\end{equation}

Consider an element 
\[\alpha=e_{\rho^*(\varphi)}(h\cdot \omega_{S^2})\in\DD^2,\quad \textrm{with}\quad h\in C^{\infty}_{0,-\sigma}(\C).\] 
By Lemma \ref{lemma:pullbacks and invariant functions}, there are two flat functions $g_1,g_2\in C^{\infty}_0(\C)$ such that 
% \[h=\lambda_2\cdot g_1\circ \mathrm{sq}+\lambda_1\cdot g_2\circ \mathrm{sq}.\]
\[h=-\lambda_1\cdot g_1\circ \mathrm{sq}+\lambda_2\cdot g_2\circ \mathrm{sq}.\]
Define the form
% \[\eta:=e_{\varphi}\big(g_1\circ f\cdot \tilde{\omega}_1+g_2\circ f \cdot\tilde{\omega}_2\big)\in \CC^2.\]
\[\eta:=e_{\varphi}\big(g_1\circ f\cdot \tilde{\omega}_1+g_2\circ f \cdot\tilde{\omega}_2\big)\in \CC^2.\]
By Lemma \ref{lemma:identification of skeleton} (2) and \eqref{eq:pullback forms}, we have that:
\[\rho^*(\eta)=\alpha.\]
The proof will be concluded once we show that:
\begin{equation}\label{eq:final:to:prove}
\rho^*(p_{\F}(\eta))=\alpha.
\end{equation}
First, since $\eta$ is closed, we have that:
\[p_{\F}(\eta)-\eta=\dif h_{\F}(\eta),\]
and so 
\begin{equation}\label{eq:homotopy on eta}
\rho^*(p_{\F}(\eta))-\alpha= \dif \rho^*(h_{\F}(\eta)).    
\end{equation}
Next, since $\rho^*(p_{\F}(\eta))\in \mathscr{D}^2$, there exists $\tilde{h}\in C^{\infty}_{0,-\sigma}(\C)$ such that 
\[\rho^*(p_{\F}(\eta))=e_{\rho^*(\varphi)}(\tilde{h}\cdot \omega_{S_2}\big).\]
Next, since $h_{\F}(\eta)\in \CC^1$, we can write 
\[\rho^*(h_{\F}(\eta))=e_{\rho^*(\varphi)}(\theta),\]
for some $\theta\in \Omega^1(S^2\times \C)$. Thus equation \eqref{eq:homotopy on eta} can be written as:
\[e_{\rho^*(\varphi)}\big((\tilde{h}-h)\cdot\omega_{S^2}-\dif \theta \big)=0.\]
Next, using the form of $\rho^*(\varphi)$ from \eqref{eq:pull back of varphi}, we contract the last equation with $\partial_{\lambda_1}$ and $\partial_{\lambda_2}$, then divide it by $4|\lambda|^2$, and we pull it back via the embedding $i_{\lambda}:S^2\hookrightarrow S^2\times\C$, $w\mapsto (w,\lambda)$; we obtain: 
\[(\tilde{h}(\lambda)-h(\lambda))\cdot\omega_{S^2}=\dif i_{\lambda}^*(\theta).\]
Passing to cohomology, this implies that $\tilde{h}=h$, and so \eqref{eq:final:to:prove} holds. 
\end{proof}

We can prove now the two statements about flat foliated cohomology:
\begin{proof}[Proof of Proposition \ref{proposition: property H fol}]
By Proposition \ref{proposition: chain isomorphism}, $\dif=0$ on $p_{\F}(\CC^{\bullet})$. The rest of the statement was already proven in Corollary \ref{corollary:chain:proj}.
\end{proof}

\begin{proof}[Proof of Proposition \ref{proposition:flat foliated ch}]
Because $p_{\F}$ is a deformation retraction of $(\CC^{\bullet},\dif)$ and because $\dif\circ p_{\F}=0$, we have that every flat foliated cohomology class has a unique representative in $p_{\F}(\CC^{\bullet})$; thus, by Proposition \ref{proposition: chain isomorphism}, we have the isomorphisms: 
\[H^{k}_0(\F)\simeq p_{\F}(\CC^{k})\simeq \DD^{k}.\]

This implies that $H^{k}_0(\F)=0$, for $k\notin\{0,2\}$. 

The case $k=0$ follows from the proof of Proposition \ref{proposition: chain isomorphism}, where we have seen that the set
\[\{e_{\varphi}(g\circ f)\, |\, g\in C^{\infty}_0(\C)\}\]
is fixed under $p_{\F}$ and that $\rho^*$ maps this set isomorphically to $\DD^{0}$. Of course, this case follows also from Proposition \ref{prop:Casimirs}, because $H^0_0(\F)$ consists of Casimir functions of $(\spl,\pi)$ that are flat at the origin (times $\varphi$). 

Finally, let $k=2$. For $g_1,g_2\in C^{\infty}_0(\C)$, denote by 
\[\eta(g_1,g_2):=e_{\varphi}(g_1\circ f\cdot \tilde{\omega}_1+g_2\circ f\cdot\tilde{\omega}_2)\in \CC^2.\]
Consider the map: 
\[\alpha: C^{\infty}_0(\C)\oplus C^{\infty}_0(\C)\to \DD^2,\]
\[(g_1,g_2)\mapsto \rho^*\circ p_{\F}(\eta(g_1,g_2)).\]
By the proof of Proposition \ref{proposition: chain isomorphism}, $\alpha$ is given by
\[\alpha(g_1,g_2)=(-\lambda_1\cdot g_1\circ \mathrm{sq}+\lambda_2\cdot g_2\circ \mathrm{sq})\rho^*(\varphi)\wedge\omega_{S^2}.\]
By part (2) of Lemma \ref{lemma:pullbacks and invariant functions}:
\[\ker(\alpha)=\mathcal{K},\]
and by part (3), $\alpha$ restricts to an isomorphism between the spaces:
\[ \alpha|_{\mathcal{M}}:\mathcal{M}\diffto \DD^2.\]
% By part (2) of Lemma \ref{lemma:pullbacks and invariant functions}, we can rewrite the kernel of $\alpha$ as: 
% \[\ker(\alpha)=\{(g_1,g_2)\, | \, yg_1=(|z|-x)g_2\},\]
% and by part (3), $\alpha$ restricts to an isomorphism between the spaces:
% \[ C^{\infty}_{0,\tau}(\C)\oplus C^{\infty}_{0,\tau}(\C)\diffto \DD^2.\]
By combining the following:
\begin{itemize}
    \item[-]$\rho^*:p_{\F}(\CC^2)\diffto \DD^2$ is an isomorphism;
    \item[-] every class in $H^2_0(\F)$ has a unique representative in $p_{\F}(\CC^2)$;
    \item[-] $\eta(g_1,g_2)$ and $p_{\F}(\eta(g_1,g_2))$ are in the same cohomology class;
\end{itemize}    
the statement follows.
\end{proof}

==> FolCH_1_sl2r.tex <==
\section{Flat Poisson cohomology of $\spl$}\label{section: flat PC}

In this section we compute the flat Poisson cohomology groups of $(\spl,\pi)$ and we build cochain homotopy operators for the flat Poisson complex which satisfy property SLB (see Theorem \ref{main theorem}).

The section is structured as follows. In Subsection \ref{section: Poisson cohomology in terms of foliated cohomology} we build an isomorphism which describes the flat Poisson complex in terms of the flat foliated complex and the transverse variation of the leafwise symplectic form (see Proposition \ref{proposition:PCH as forms}). For this, we use the description of the Poisson complex as the de Rham complex of a Lie algebroid, and the spectral sequence for computing cohomology of regular Lie algebroids. In Subsection \ref{section: perturbation Lemma} we use the Perturbation Lemma and the explicit description of flat foliated cohomology to construct cochain homotopies for the aforementioned complex (see Proposition \ref{proposition: homotopy}). Combining these results, we obtain a description of the flat Poisson cohomology in Theorem \ref{main theorem}. In Subsection \ref{section: algebra} we explain the algebraic structure of Poisson cohomology.

\subsection{Poisson cohomology in terms of foliated cohomology}\label{section: Poisson cohomology in terms of foliated cohomology}


In this subsection we describe the flat Poisson complex of $\spl$ in terms of the flat foliated complex of $\F$. For this, we use the spectral sequence associated to a regular Poisson manifold, which has been introduced in \cite{Vaisman} and \cite{KV1} (see also \cite[Section 2.4]{DZ}). Here, we use the more general setting of Lie algebroids of \cite{mack05}. We can adapt these techniques to our non-regular case by working with sections that are flat at the singularity,


Recall that the linear Poisson structure $\pi$ is regular away from the origin with underlying foliation $\F$. For simplicity, let us denote:
\[\spl^{\times}:=\spl\backslash \{0\}\]
The vector fields $V_1$ and $V_2$ on $\spl^{\times}$, defined in \eqref{eq: v}, form a basis of the normal bundle $\nu$ to $\F$. Since these vector fields are projectable with respect to $f$ (see \eqref{eq:v transversality}), it follows that they preserve the foliation:
\begin{align}\label{eq: flat}
    [V_i,Y]\in \Gamma(T\F|_{\spl^{\times}}), \quad \forall\, Y\in \Gamma(T\F|_{\spl^{\times}}).
\end{align}

We make use of the extension $\tilde{\omega}_1$ of the leafwise symplectic form on $\F$ from Lemma \ref{lemma: extension omega}. This is uniquely determined such that its kernel is spanned by $V_1$ and $V_2$. For $i=1,2$, define:
\begin{align}\label{eq: gammai}
    \gamma_i:=i_{V_i}\dif \tilde{\omega}_1\in \Omega^2(\spl^{\times}).
\end{align}
The restriction $\gamma_i|_{\F}$, for $i=1,2$, is the \emph{variation of the leafwise symplectic form} $\omega_1$ in the direction of $V_i$ (as foliated forms):
\[\gamma_i\big|_{\F}=\frac{\dif}{\dif t}\Big|_{t=0}(\varphi_{V_i}^t)^*\omega_1.\]
In particular, it follows that $\gamma_i|_{\F}\in \Omega^2(\F)$ are closed foliated 2-forms.

Recall that the singularity of $\tilde{\omega}_1$ at the origin is very ``mild", and the same holds for $\gamma_i$. Therefore the product with $\gamma_i$ gives a well-defined map:
\[e_{\gamma_i}:\CC^{p}\to \CC^{p+2},\quad \eta\mapsto \gamma_i\wedge \eta.\]

\begin{proposition}\label{proposition:PCH as forms}
There is an isomorphism of complexes
\[\tilde{a}:(\mathfrak{X}_0^{\bullet}(\spl),\dif_{\pi})\diffto (\bigoplus_{p+q=\bullet}\CC^{p}\otimes \wedge^q\R^2, \dif +\delta),\]
where $\dif$ acts only on the first component $\CC^{\bullet}$ as the exterior derivative and
\begin{align*}
\delta:\CC^{p}\otimes \wedge^q\R^2&\to \CC^{p+2}\otimes \wedge^{q-1}\R^2,\\
\delta(\eta\otimes e_{i})&=(-1)^p\gamma_i\wedge \eta,\quad\quad i=1,2,\\
\delta(\eta\otimes e_{1}\wedge e_2)&=(-1)^p\big(\gamma_1\wedge\eta\otimes e_2- \gamma_2\wedge\eta\otimes e_1\big),
\end{align*}
where $e_{1},e_2$ is the standard basis of $\R^2$. Moreover, the operators $\tilde{a}$, $\tilde{a}^{-1}$ and $\delta$ satisfy property SLB for $(0,0,2)$, $(0,0,4)$ and $(0,0,3)$, respectively. 
\end{proposition}

The rest of this subsection is devoted to the proof of this proposition.

\subsubsection{Cohomology of regular abelian Lie algebroids}


Proposition \ref{proposition:PCH as forms} can be understood as giving an explicit description of the first page of a natural spectral sequence associated to Poisson cohomology, which was introduced for regular Poisson manifolds already in \cite{Vaisman}. The natural framework for this are Lie algebroids (see \cite{mack05}), and, for clarity, we place our discussion in this more general setting. However, we will use these results only for the cotangent Lie algebroid of a regular Poisson manifold. 

As a reference to the theory of Lie algebroids, see \cite{mack05}. Recall that any Lie algebroid $(A,[\cdot,\cdot],\sharp)$ has an associated de Rham complex
\[(\Omega^{\bullet}(A):=\Gamma(\wedge^{\bullet}A^*),\dif_A).\]
Consider a Lie algebroid $(A,[\cdot,\cdot],\sharp)$ over $M$ with the following properties:
\begin{itemize}
    \item $A$ is \textbf{regular}, i.e., the anchor $\sharp$ has constant rank. Then $M$ has a regular foliation $\F$ with $T\F=\im \sharp \subset TM$, the kernel $K:=\ker \sharp$ is a Lie subalgebroid, and we have a short exact sequence of Lie algebroids
    \begin{align}\label{eq: lad ses}
        0 \to K \xrightarrow{j} A \xrightarrow{\sharp} T\F \to 0
    \end{align}
    \item $K$ is an \textbf{abelian} Lie algebroid. Therefore, the bracket on $A$ induce a representation of $T\F$ on $K$.
\end{itemize}

To such a Lie algebroid one associates the \textbf{extension class} \[[\gamma] \in H^2(\F,K),\] 
which measures the failure of the short exact sequence \eqref{eq: lad ses} to split as a sequence of Lie algebroids. Using a vector bundle splitting $\sigma: T\F \to A$ of \eqref{eq: lad ses}, an explicit representative of the extension class is given by:  
\[ \gamma(Y_1,Y_2):= [\sigma(Y_1),\sigma(Y_2)] -\sigma([Y_1,Y_2]) \]
where $Y_1,Y_2\in \Gamma(T\F)$. The class $[\gamma]$ is independent of the choice of the splitting. For such a representative, we have an induced map:
\begin{align}
&\qquad \qquad \qquad i_{\gamma}: \Omega^p(\F,\wedge^qK^*) \to  \Omega^{p+2}(\F,\wedge^{q-1}K^*) \nonumber \\
  i_{\gamma}(\beta)&\,(Y_1 , \dots ,Y_{p+2})(V_1, \dots ,V_{q-1}) :=\label{eq: contraction gamma}\\  &\sum_{i<j}(-1)^{i+j}\beta(Y_1, \dots, \hat{Y}_i,\dots ,\hat{Y}_j,\dots ,Y_{p+2})(\gamma(Y_i,Y_j),V_1,\dots, V_{q-1})\nonumber
\end{align}
where $V_i \in \Gamma(K)$, $Y_j\in \Gamma(T\F)$. We have the following: 

\begin{proposition}\label{proposition: ladcx}
A splitting $\sigma:T\F \to A$ of \eqref{eq: lad ses} induces an isomorphism
\begin{align*}
    (\Omega^{\bullet}(A), \dif_A)\simeq \big(\bigoplus_{p+q=\bullet}\Omega^{p}(\F,\wedge^{q} K^*), \delta_1+\delta_2\big),
\end{align*}
where $\delta_1$ is the standard differential on foliated forms with values in $\wedge^{q}K^*$
\begin{align*}
    \delta_1=\dif_{\F}:\Omega^{p}(\F,\wedge^{q}K^*)\to \Omega^{p+1}(\F,\wedge^{q}K^*)
\end{align*}
and $\delta_2$ is the cup product with the representative of the extension class: 
\begin{align*}
\delta_2=(-1)^{p}i_{\gamma}:\Omega^{p}(\F,\wedge^{q}K^*)\to \Omega^{p+2}(\F,\wedge^{q-1}K^*).
\end{align*}
\end{proposition}

\begin{proof}
We follow \cite[Section 7.4]{mack05} where most of the statement is proven. A splitting $\sigma : T\F \to A$ of \eqref{eq: lad ses} induces surjective maps
\begin{align}\label{eq: surjection ladch}
&\qquad \qquad a^{p,q}:\Omega^{p+q}(A) \to \Omega^{p}(\F,\wedge^q K^*)\\
a^{p,q}(\alpha)&\,(Y_1, \dots ,Y_p) (V_1, \dots V_q):= \alpha(\sigma(Y_1),\dots , \sigma(Y_p),V_1,\dots, V_q)\nonumber
\end{align}
for $V_i \in \Gamma(K)$ and $Y_j\in \Gamma(T\F)$. Let $\kappa = \id-\sigma \circ \sharp:A\to K$ be the induced projection. A right inverse for $a^{p,q}$ is given by: 
\begin{align}\label{eq: ri ladch}
    &\qquad \qquad b^{p,q}: \Omega^{p}(\F,\wedge^q K^*)\to \Omega^{p+q}_p(A)\\
    b^{p,q}(\beta)&\,(X_1, \dots ,X_{p+q}):= \nonumber \\ 
    &\sum_{\tau\in S_{p,q}}\sign(\tau)\beta(\sharp(X_{\tau_{1}}),\dots,\sharp(X_{\tau_{p}}))(\kappa(X_{\tau_{p+1}}),\dots,\kappa(X_{\tau_{p+q}})),\nonumber
\end{align}
where the sum is over all $(p,q)$ shuffles $\tau$. The isomorphism from the statement is $\oplus_{p+q=\bullet}a^{p,q}$, with inverse  $\oplus_{p+q=\bullet}b^{p,q}$.

We calculate the components of the differential under this isomorphism:
\begin{align*}
    \delta_{i}:= a^{p+i,q+1-i}\circ \dif_A \circ b^{p,q}, \quad i\in \N_0.
\end{align*}
For $i=0$ and $i=1$ these are given in \cite[Proposition 7.4.3 \& 7.4.4]{mack05}, namely, $\delta_{0}=0$ because $K$ is assumed to be abelian and the different sign for $\delta_1$ comes from the fact that we multiplied both $a^{p,q}$ and $b^{p,q}$ with a factor of $(-1)^{pq}$. For $\delta_{2}$ we use a proof given for $q=1$ in \cite[Theorem 7.4.11]{mack05} for foliated cohomology. We adapt the computation there to general $q$ and foliated forms as follows. Let $\beta\in \Omega^p(\F,\wedge^qK^*)$. We need to prove that
\begin{align*}
    (a^{p+2,q-1}\circ \dif_A\circ b^{p,q})(\beta)=&\ (-1)^{p}i_{\gamma}(\beta)
\end{align*}
Let $V_i\in \Gamma(K)$ and $Y_j\in \Gamma(T\F)$. For the computation we use the notation
\begin{equation*}
    \begin{array}{rlcrl}
    \mathcal{V} :=& V_1,\dots ,V_{q-1}&\ & 
         \mathcal{Y}:=& Y_1,\dots,Y_{p+2}   \\
         \mathcal{V}_i :=& V_1,\dots,\hat{V}_i,\dots ,V_{q-1}&\ & 
         \mathcal{Y}_i:=& Y_1,\dots,\hat{Y}_i,\dots ,Y_{p+2}   \\
         \mathcal{V}_{ij}:=& V_1,\dots,\hat{V}_i,\dots,\hat{V}_j,\dots ,V_{q-1}
         & &    \mathcal{Y}_{ij}:=&
         Y_1,\dots,\hat{Y}_i,\dots, \hat{Y}_j,\dots ,Y_{p+2}
    \end{array}
\end{equation*}
where the hat stands for omitting the element and by $\sigma(\mathcal{Y}_i)$ we mean $\sigma$ applied to each element, and similarly for $\sigma(\mathcal{Y}_{ij})$. Then we compute that

\begin{align*}
    (a^{p+2,q-1}\circ &\, \dif_A\circ  b^{p,q})(\beta)(\mathcal{Y})(\mathcal{V}) =(\dif_A\circ b^{p,q})(\beta)(\sigma(\mathcal{Y}),\mathcal{V})\\
   =&\sum_{1\le i<j\le p+2}(-1)^{i+j}(b^{p,q}(\beta))([\sigma(Y_i),\sigma(Y_j)],\sigma(\mathcal{Y}_{ij}),\mathcal{V})\\
    &+\sum_{\substack{1\le i\le q-1\\ 1\le j\le p+2}}(-1)^{p+1+i+j}(b^{p,q}(\beta))([\sigma(Y_i),V_j],\sigma(\mathcal{Y}_i),\mathcal{V}_j)\\
    &+\sum_{1\le i<j\le q-1}(-1)^{i+j}(b^{p,q}(\beta))([V_i,V_j],\sigma(\mathcal{Y}),\mathcal{V}_{ij})
    \\
    &+\sum_{1\le i\le p+2}(-1)^{i+1}\Lie_{Y_i}((b^{p,q}(\beta))(\sigma(\mathcal{Y}_{i}),\mathcal{V}))\\
  =&\sum_{1\le i<j\le p+2}(-1)^{i+j+p}\beta(\mathcal{Y}_{ij})(\gamma(Y_i, Y_j),\mathcal{V})\\
    =&\, (-1)^{p} i_{\gamma}(\beta)(\mathcal{Y})(\mathcal{V})
\end{align*}
Note that only the first sum yields non-zero contributions to the third equality as all the other terms do not have enough sections of $K$ to be non-zero, and we have $\kappa\circ \sigma =0$. By a similar computation $\delta_{i}=0$, for $3\le i$.
\end{proof}

We obtain a slight improvement of results in \cite[Section 7.4]{mack05}, which is classical for Lie algebras (see e.g.\ \cite[Theorem 8]{Hoch1953}):

\begin{corollary}\label{corollary: ladch}
For a regular Lie algebroid $K\hookrightarrow A\twoheadrightarrow T\F$ with abelian isotropy $K$, there is a natural spectral sequence which converges to the Lie algebroid cohomology of $A$:
\[ H^p(\F,\wedge^q K^*)\Rightarrow H^{p+q}(A).\]
Moreover, the differential on the second page is given by the cup product with the extension class:
\[(-1)^{p}i_{[\gamma]}:H^p(\F,\wedge^q K^*)\to H^{p+2}(\F,\wedge^{q-1} K^*).\]
\end{corollary}
\begin{proof}
The natural, convergent spectral sequence was obtained in \cite[Theorem 7.4.6]{mack05}; it is associated with the filtration 
\begin{align}\label{eq: filtration}
    \Omega^{p+q}_{p}(A):= \{\beta\in \Omega^{p+q}(A)| i_{V_0}\dots i_{V_q}\beta =0 \text{ for all } V_j\in \Gamma(K)\}. 
\end{align}
Under the isomorphism from  Proposition \ref{proposition: ladcx}, this filtration corresponds to 
\[\bigoplus_{0\leq i\leq q} \Omega^{p+i}(\F,\wedge^{q-i}K^*).\]
The explicit formula for the differential on the second page follows from the proposition. 
\end{proof}



\subsubsection{Poisson cohomology via Lie algebroids}
Given a Poisson manifold $(M,\pi)$ one has a naturally associated Lie algebroid structure on the cotangent bundle $T^*M$ with the anchor map $\pi^{\sharp}:T^*M \to TM$ and the bracket given by
\[ [\alpha,\beta]_{\pi}:= \Lie _{\pi^{\sharp}(\alpha)}(\beta)-\Lie _{\pi^{\sharp}(\beta)}(\alpha)-\dif \pi(\alpha,\beta).\]
We denote this Lie algebroid by $T^*_{\pi}M$. The complex computing Lie algebroid cohomology of $T^*_{\pi}M$ can be identified with the complex computing the Poisson cohomology of $(M,\pi)$:
\begin{align*}
    (\Omega^{\bullet}(T^*_{\pi}M),\dif) = (\mathfrak{X}^{\bullet}(M),\dif_{\pi}).
\end{align*}

From now on we will assume that $(M,\pi)$ is \textbf{regular}. Then we are in the setting of the previous subsection, i.e., the Lie algebroid $T^*_{\pi}M$ fits into the short exact sequence
\begin{align}\label{eq: ses poisson lad}
    0\to \nu^* \hookrightarrow T^*_{\pi}M\twoheadrightarrow T\F\to 0
\end{align}
where $T\F=\im \pi^{\sharp}$ and $\nu^*$ is the conormal bundle of $\F$, which is an abelian ideal. The leafwise symplectic form will be denoted by: 
\[\omega\in \Omega^2(\F).\]

A splitting $\sigma:T\F\to T^*_{\pi}M$ of \eqref{eq: ses poisson lad} induces an extension $\tilde{\omega}\in \Omega^2(M)$ of $\omega$, uniquely determined by $\ker\tilde{\omega}=\ker (\sigma^*:TM\to T^*\F)$. The representative $\gamma$ of the extension class in $H^2(\F,\nu^*)$ of \eqref{eq: ses poisson lad} corresponding to $\sigma$ is then:
\begin{align*}
    \gamma(Y_1,Y_2)=i_{Y_2}i_{Y_1} \dif\tilde{\omega}\in \Gamma(\nu^*),
\end{align*}
for $Y_1,Y_2\in \Gamma(T\F)$. This follows by a standard calculation using the formula of the Lie bracket on $T^*_{\pi}M$ and that $ \sigma(v)=i_v\tilde{\omega}$.

\smallskip

We apply this discussion to the linear Poisson structure $\pi$ restricted to 
\[\spl^{\times}:=\spl\backslash\{0\}.\] 
The extension $\tilde{\omega}_1$ of the leafwise symplectic structure from Lemma \ref{lemma: extension omega} corresponds to the splitting $\sigma$ whose image annihilates the vector fields $V_1$ and $V_2$ defined in \eqref{eq: v}. We obtain linear maps
\begin{align*}
    a^{p,q}:\mathfrak{X}^{p+q}(\spl^{\times}) \to \Omega^p(\F|_{\spl^{\times}}, \wedge^q\nu)
\end{align*}
as described in \eqref{eq: surjection ladch} with right inverses given by
\begin{align*}
    b^{p,q}:\Omega^p(\F|_{\spl^{\times}}, \wedge^q\nu)\to \mathfrak{X}^{p+q}(\spl^{\times})
\end{align*}
as described in \eqref{eq: ri ladch}.

The normal vector fields $V_1$ and $V_2$ induce a flat frame of the normal bundle, and so give an isomorphism $\nu\simeq \R^2\times{\spl^{\times}}$ of $T\F$-representations.

\begin{lemma}\label{lemma: maps mpq} There are linear isomorphisms:
\[m^{p,q}:\Omega^p(\F|_{\spl^{\times}}, \wedge^q\nu)\simeq
e_{\varphi}(\Omega^p(\spl^{\times}))\otimes \wedge^q\R^2,
\]
under which the operators $\delta_1=\dif_{\F}$ and $\delta_2=(-1)^{p}i_{\gamma}$ correspond to the operators $\dif$ and $\delta$ from Proposition \ref{proposition:PCH as forms}.
\end{lemma}

\begin{proof}
Any form $\eta\in \Omega^{p}(\F|_{\spl^{\times}}, \wedge^{\bullet}\nu)$ can be uniquely written as
\[\eta=\eta_0+\eta_1\otimes [V_1] +\eta_2\otimes[V_2]+\eta_{3}\otimes[V_1\wedge V_2],\quad \eta_i\in \Omega^{p}(\F|_{\spl^{\times}}).\]
The isomorphism $m=\oplus_{p,q} m^{p,q}$ sends such a form to:
\[m(\eta)=e_{\varphi}(\eta_0)+e_{\varphi}(\eta_1)\otimes e_1+e_{\varphi}(\eta_2)\otimes e_2+ e_{\varphi}(\eta_3)\otimes e_1\wedge e_2,\]
where $e_1,e_2$ is the standard basis of $\R^2$. That $\dif_{\F}$ corresponds to $\dif$ follows because $\dif_{\F}[V_i]=0$ (see \eqref{eq: flat}) and because $\dif \varphi=0$. Using \eqref{eq: contraction gamma} we obtain 
\begin{align*}
\delta_2(\eta)&=(-1)^p(i_{\gamma}\eta_0+i_{\gamma}\eta_1\otimes [V_1]+i_{\gamma}\eta_2\otimes [V_2]+i_{\gamma}\eta_3\otimes[V_1\wedge V_2])\\
&=(-1)^p(e_{\gamma_1}(\eta_1)+e_{\gamma_2}(\eta_2)+e_{\gamma_1}(\eta_3)\otimes[V_2]-e_{\gamma_2}(\eta_3)\otimes[V_1])
\end{align*}
since $\gamma$ can be written as
\[\gamma=\gamma_1|_{\F}\otimes \dif f_1+\gamma_2|_{\F}\otimes \dif f_2.\]
This implies the statement.
\end{proof}

Due to the mild singularities of $V_1$,  $V_2$ and $\tilde{\omega}_1$ at the origin, the maps $m^{p,q}\circ a^{p,q}$ induce well-defined, surjective maps between the complexes of flat multivector fields and flat foliated forms:
\begin{align}\label{eq: tilde a}
    \tilde{a}^{p,q}:\mathfrak{X}^{p+q}_{0}(\spl) \to \CC^p\otimes \wedge^q \R^2.
\end{align}
These maps have right inverses induced by $b^{p,q}\circ (m^{p,q})^{-1}$ which we denote
\begin{align}\label{eq: tilde b}
    \tilde{b}^{p,q}: \CC^p\otimes \wedge^q\R^2\to \mathfrak{X}^{p+q}_{0}(\spl).
\end{align}

Putting these maps together into \[\tilde{a}:=\oplus_{p,q}\tilde{a}^{p,q}\quad \textrm{and} \quad \tilde{b}:=\oplus_{p,q}\tilde{b}^{p,q}\] we obtain the linear isomorphism from Proposition \ref{proposition:PCH as forms} and its inverse. That these maps intertwine the Poisson differential and the differential $\dif+\delta$ follows from Proposition \ref{proposition: ladcx} and Lemma \ref{lemma: maps mpq}. To conclude the proof of Proposition \ref{proposition:PCH as forms} we need to show that the map $\tilde{a}$, $\tilde{b}$ and $\delta$ satisfy the claimed SLB property. For this, let us note that these operators are induced by vector bundle maps with a singularity at the origin. For example, $\tilde{a}^{1,1}$ is induced by the vector bundle map:
\begin{align*}
&A^{1,1}:\wedge^{2}T(\spl^{\times})\to \wedge^{3} T^*(\spl^{\times})\otimes \R^2,\\
&A^{1,1}(w)=-\sum_{i=1}^2\varphi\wedge \tilde{\omega}_1^{\flat}(i_{\dif f_i}w)\otimes e_i.
\end{align*}
Similarly, $\tilde{a}^{4,0}$ is induced by the vector bundle map:
\begin{align*}
&A^{4,0}:\wedge^{4}T(\spl^{\times})\to \wedge^{6} T^*(\spl^{\times}),\\
&A^{4,0}(w)=\varphi\wedge (\otimes^4 \tilde{\omega}_1^{\flat})(w).
\end{align*}
The maps $\tilde{b}^{p,q}$ are restrictions of singular vector bundle maps. For example, $\tilde{b}^{2,1}$ is induced by the restriction of the map:
\begin{align*}
&B^{2,1}:\wedge^{4} T^*(\spl^{\times})\otimes \R^2\to \wedge^{3}T(\spl^{\times}),\\
&B^{2,1}\Big(\sum_{i=1}^2\alpha_i\otimes e_i\Big)=
\sum_{i=1}^2(\otimes^2\pi^{\sharp})(i_{V_1\wedge V_2}\alpha_i)\wedge V_i.
\end{align*}
Similarly, $\tilde{b}^{0,2}$ comes from the map:
\begin{align*}
&B^{0,2}:\wedge^{2} T^*(\spl^{\times})\otimes \wedge^2\R^2\to \wedge^{2}T(\spl^{\times}),\\
&B^{0,2}\big(\beta\otimes e_1\wedge e_2\big)=
i_{V_1\wedge V_2}(\beta)\, V_1\wedge V_2.
\end{align*}
A similar description holds also for $\delta$. These vector bundle maps fit in the setting of the following lemma.

\begin{lemma}\label{lemma:singular:vb:maps} Let $V$ and $W$ be two vector bundles over an inner product space $H$. Consider a vector bundle map with a singularity at the origin, i.e., a vector bundle map: 
\[\Phi:V|_{H\backslash\{0\}}\to W|_{H\backslash\{0\}}.\]
Assume that the singularity is such that, for some $l\geq 0$, 
$R^{l}\Phi$ is smooth and that it vanishes at the origin up to order $d\geq 0$, where $R$ denotes the induced norm on $H$. Then $\Phi$ induces a linear operator between flat sections:
\[\Phi_{*}:\Gamma_0(V) \to \Gamma_0(W),\]
which satisfies property SLB for $(0,0,\mathrm{max}(l-d,0))$.
\end{lemma}

\begin{proof}
Without loss of generality we may assume that the vector bundles $V$ and $W$ are trivial. Therefore, $\Phi$ is described by a matrix of the form
\begin{align*}
    \Phi = \begin{pmatrix}
    \frac{1}{R^{l}}\phi_{ij}
    \end{pmatrix} 
\end{align*}
where $\phi_{ij}\in C^{\infty}(H)$ vanish up to order $d$ at the origin. It is enough to show that for $\phi\in C^{\infty}(H)$ vanishing at the origin up to order $d$, we have: 
\begin{align*}
    \fnorm{\frac{1}{R^{l}}\phi\, g}_{n,k,r}\le C\fnorm{g}_{n,\mathrm{max}(0,k+l-d),r}
\end{align*}
for all $g\in C^{\infty}_0(H)$, $n,k\in \N_0$, $r>0$ and a constant $C$. First, by the equivalence of norms from Lemma \ref{lemma: equivalence}, we have that:
\begin{align*}
    \fnorm{\frac{1}{R^{l}}\phi\, g}_{n,k,r}\le C\fnorm{\phi\, g}_{n,k+l,r}.
\end{align*}

By the general Leibniz rule we obtain for $a\in \N_0^{\dim(V)}$ with $|a|=n$ that
\begin{align*}
    D^a (\phi\, g) & =\sum_{a^1+a^2=a} D^{a^1}\phi\, D^{a^2}g.
\end{align*}
Next, Taylor's formula with integral remainder for $|a^2|<n$ yields: 
\[ D^{a^2}g(x)=\sum_{|b|=|a^1|}x^{b}\int_{0}^1|a^1|(1-s)^{|a^1|-1}(D^{b+a^2} g)(sx)\dif s.\]
Combining these yields for $x\in B_r\subset H$ and any $m=k+l\in \N_0$ the estimate
\begin{align*}
    \frac{|D^a \phi g|}{R^{m}} (x) &\le \sum_{a^1+a^2=a} \frac{1}{R^{m}}|D^{a^1}\phi||D^{a^2}g |(x)\\
    &\le C\Big(\sum_{0<|b|= n- |a^2|}\frac{R^{\max(|b|,d)}}{R^{m}}\int_{0}^1(1-s)^{|b|-1}|D^{b+a^2} g|(sx)\dif s\\
    &\qquad \quad + \frac{R^{d}}{R^{m}}|D^ag|(x)\Big)\\
    &\le C\Big(\sum_{0<|b|= n- |a^2|}\int_{0}^1\frac{s^{\max(0,m-d)}(1-s)^{|b|-1}}{(sR)^{\max(0,m-d)}}|D^{b+a^2} g|(sx)\dif s\\
    &\qquad \quad + \frac{1}{R^{\max(0,m-d)}}|D^ag|(x)\Big)\\
    &\le C \,\fnorm{g}_{n,\max(0,m-d),r}. \qedhere
\end{align*}
\end{proof}

The lemma implies that the maps $\tilde{a}$, $\tilde{b}$ and $\delta$ satisfy the claimed SLB properties. This follows by analyzing the singularities of our vector bundle maps, for which we obtain:
\begin{itemize}
    \item[-] for $A^{p,q}$: $l=2p$, $d=p+q+2$; hence $l-d\leq 2$;
    \item[-] for $B^{p,q}$: $l=4+2q$, $d=p+q+2$; hence $l-d\leq 4$;
    \item[-] for the map inducing $\delta$: $l=6$ and $d=3$; hence $l-d=3$.
\end{itemize}
This concludes the proof of Proposition \ref{proposition:PCH as forms}. 


\subsection{Cochain homotopies}\label{section: perturbation Lemma}

By Proposition \ref{proposition:PCH as forms}, the complex 
\begin{equation}\label{eq:beautiful:complex}
    \Big(\bigoplus_{p+q=\bullet}\CC^{p}\otimes \wedge^{q}\R^2,\dif +\delta\Big)
\end{equation}
computes the flat Poisson cohomology of $(\spl,\pi)$. This complex admits the filtration by the $p$-degree, as in Corollary \ref{corollary: ladch}. The second page of the associated spectral sequence is given by:
\begin{equation*}
    \begin{tikzpicture}[baseline= (a).base]
    \node[scale=1] (a) at (0,0){
    \begin{tikzcd}[row sep=small]
    H^0_0(\F)\otimes\wedge^2\R^2\arrow{rrd}{\phantom{1}i_{[\gamma]}}&0&H^2_0(\F)\otimes\wedge^{2}\R^2 \\
    H^0_0(\F)\otimes\wedge^1\R^2\arrow{rrd}{\phantom{1}i_{[\gamma]}}&0&H^2_0(\F)\otimes\wedge^{1}\R^2\\
    H^0_0(\F)\otimes\wedge^{0}\R^2 &0&H^2_0(\F)\otimes\wedge^{0}\R^2
    \end{tikzcd}
    };
    \end{tikzpicture}
\end{equation*}
where we used that $H^{p}_0(\F)=0$, for $p\notin\{0,2\}$. In particular, all differentials on higher pages vanish, and so the cohomology is determined by the third page. The kernel and cokernel of the maps $i_{[\gamma]}$ will be calculated explicitly in the Subsections \ref{section: cohomology second page} and \ref{section: HE data}. This will provide the complete description of the Poisson cohomology in Subsection \ref{section: flat pch}. The construction of homotopy operators will be obtained by applying the Perturbation Lemma, which is done in the first subsection.


\subsubsection{The Perturbation Lemma}

For the proof of Theorem \ref{theorem: nondegenerate} it does not suffice to calculate the Poisson cohomology, but we need explicit cochain homotopies satisfying estimates as in Definition \ref{definition: property H}. In this subsection we show how the deformation retraction $(p_{\F},h_{\F})$ of $(\CC^{\bullet},\dif)$ induces a deformation retraction of the complex \eqref{eq:beautiful:complex}. For this we use the Perturbation Lemma following \cite{Cr04} and the terminology therein, which we first recall. 

\begin{definition}
A \textbf{homotopy equivalence data} (HE data):
\begin{align}\label{eq: he data}
    (B,\mathrm{b} )\stackrel[\iota]{p }{\leftrightarrows} (C,\dif),h
\end{align}
consists of two complexes $(B,\mathrm{b})$ and $(C,\dif)$ together with two quasi-isomorphisms $p$ and $\iota$, and a cochain homotopy $h$ between $\iota \circ p$ and the identity, i.e.,
\begin{align*}
    \iota \circ p -\id = h\circ \dif +\dif \circ h
\end{align*}
\end{definition}
\begin{remark}
Note that any deformation retraction (see Definition \ref{definition: dr}) defines an HE data. In particular, by Proposition \ref{proposition: property H fol} we have the HE data
\begin{align*}
    (p_{\F}(\CC),0 )\stackrel[\iota]{p_{\F} }{\leftrightarrows} (\CC,\dif),h_{\F}
\end{align*}
\end{remark}
Given an HE data one considers perturbations of this data as follows:
\begin{definition}
A \textbf{perturbation} $\delta$ of an HE data as in \eqref{eq: he data} is a map on $C$ of the same degree as $\dif$ such that $\dif+\delta$ is a differential:
\begin{align*}
    (\dif+\delta)^2=0.
\end{align*}
The perturbation $\delta$ is called \textbf{small} if $(\id - \delta h)$ is invertible. Then we set
\begin{align*}
    A:= (\id -\delta \circ h)^{-1}\circ \delta.
\end{align*}
The \textbf{perturbation data} of the small perturbation $\delta$ is the data: \begin{align}\label{eq: perturbation data}
    (B,\tilde{\mathrm{b}})\stackrel[\tilde{\iota}]{ \tilde{p}}{\leftrightarrows} (C,\dif +\delta),\tilde{h}
\end{align}
%with
\begin{equation*}
    \begin{array}{rclcrcl}
         \tilde{\iota} &=& (\id +h\circ A)\circ \iota, &\ \ \ \ \ & \tilde{p}&=& p\circ (\id +A\circ h), \\
         \tilde{h} &=& h\circ (\id +A\circ h),& &\tilde{\mathrm{b}} &=&\mathrm{b} +p\circ A\circ \iota.
    \end{array}
\end{equation*}
\end{definition}
The main statement in \cite{Cr04} states:
\begin{lemma}\label{lemma: perturbation lemma}
If $\delta$ is a small perturbation of an HE data as in \eqref{eq: he data}, then the associated perturbation data \eqref{eq: perturbation data} is an HE data.
\end{lemma}


We apply the Perturbation Lemma to our complex $(\CC\otimes \wedge \R^2, \dif+\delta)$, which we regard as a perturbation of the differential $\dif$, admitting the deformation retraction $(p_{\F},h_{\F})$. Here we extend all these operators from $\CC$ to $\CC\otimes \wedge \R^2$ by $- \otimes \id_{\wedge\R^2}$. These maps fit in the diagram: 
\begin{equation}\label{eq: complex diag}
    \begin{tikzpicture}[baseline= (a).base]
    \node[scale=.9] (a) at (0,0){
    \begin{tikzcd}
    \CC^0\otimes\wedge^2\R^2\arrow[bend left=5]{r}{\dif}\arrow{rrd}{\delta}&\CC^1\otimes\wedge^2\R^2\arrow[bend left=5]{r}{\dif}\arrow[bend left=5]{l}\arrow{rrd}{\delta}&\CC^2\otimes\wedge^2\R^2\arrow[bend left=5]{r}{\dif}\arrow[bend left=5]{l}&\CC^3\otimes\wedge^2\R^2\arrow[bend left=5]{l}{h_{\F}} \\
    \CC^0\otimes\wedge^1\R^2\arrow[bend left=5]{r}{\dif}\arrow{rrd}{\delta}&\CC^1\otimes\wedge^1\R^2\arrow[bend left=5]{r}\arrow[bend left=5]{l}\arrow{rrd}{\delta}&\CC^2\otimes\wedge^1\R^2\arrow[bend left=5]{r}\arrow[bend left=5]{l}&\CC^3\otimes\wedge^1\R^2 \arrow[bend left=5]{l}{h_{\F}} \\
    \CC^0\otimes\wedge^0\R^2\arrow[bend left=5]{r}{\dif}&\CC^1\otimes\wedge^0\R^2\arrow[bend left=5]{r}\arrow[bend left=5]{l}{h_{\F}}&\CC^2\otimes\wedge^0\R^2\arrow[bend left=5]{r}\arrow[bend left=5]{l}{h_{\F}}&\CC^3\otimes\wedge^0\R^2\arrow[bend left=5]{l}{h_{\F}}
    \end{tikzcd}
    };
    \end{tikzpicture}
\end{equation}

As an immediate consequence of the Perturbation Lemma we obtain:
\begin{corollary}\label{corollary: homotopy}
The complex $(\CC\otimes \wedge\R^2,\dif+\delta)$ admits the HE data
\begin{align*}
    (p_{\F}(\CC)\otimes \wedge\R^2,\tilde{\delta})\stackrel[\tilde{\iota}]{\tilde{p}}{\leftrightarrows}(\CC\otimes \wedge\R^2 ,\dif+ \delta),\tilde{h}
\end{align*}
where the maps $\tilde{\iota}$, $\tilde{p}$ and $\tilde{h}$ are given by
\begin{align*}
    \tilde{\iota} =&\ \sum_{i=0}^2 (h_{\F}\circ \delta)^i\circ \iota,\ \ \ \ \ \ \  \tilde{p} = p_{\F}+p_{\F}\circ \delta\circ h_{\F},\\
    \tilde{h}=&\ h_{\F}\circ \sum_{i=0}^2 (\delta\circ h_{\F})^i, \ \ \ \ \ \ \tilde{\delta} = p_{\F}\circ \delta.
\end{align*}
The maps $\tilde{\iota}$, $\tilde{p}$ and the homotopy $\tilde{h}$ satisfy property SLB for $(0,10,76)$, $(1,10,83)$ and $(0,15,111)$, respectively.
\end{corollary}
\begin{proof}
From Proposition \ref{proposition: property H fol} we know that the complex $(C^{\bullet},\dif)$ given by \begin{align}\label{eq: complex short}
    C^k := \underset{p+q=k}{\bigoplus} \CC^p\otimes \wedge ^q\R^2
\end{align}
admits the HE data 
\begin{align*}
    (p_{\F}(C),0)\stackrel[\iota]{p_{\F} }{\leftrightarrows}(C,\dif),h_{\F}
\end{align*}
Note that $\delta$ is a small perturbation of $\dif$ since $\delta \circ h_{\F}$ is nilpotent:
\begin{align*}
    (\delta \circ h_{\F})^3=0
\end{align*}
and hence
\begin{align*}
    (\id -\delta\circ h_{\F})^{-1}=\sum_{i=0}^2 (\delta\circ h_{\F})^i.
\end{align*}
Hence we can apply Lemma \ref{lemma: perturbation lemma}. The formulas for $\tilde{\iota}$, $\tilde{p}$, $\tilde{h}$ and $\tilde{\delta}$ follow now immediately, by looking at the $(p,q)$ degrees and using that $p_{\F}(\CC^{p})=0$, for $p\notin \{0,2\}$, by Proposition \ref{proposition:flat foliated ch}.


By Proposition \ref{proposition:PCH as forms}, $\delta$ satisfies property SLB for $(0,0,3)$ and, by Proposition \ref{proposition: property H fol} and the remark following it, $p_{\F}$ and $h_{\F}$ satisfy property SLB for $(1,5,40)$ and $(0,5,35)$, respectively. Therefore, by Lemma \ref{lemma: slb property}, the operators $\tilde{\iota}$, $\tilde{p}$ and $\tilde{h}$ satisfy the claimed SLB properties.
\end{proof}






\subsubsection{The differential $\tilde{\delta}$ and its partial inverses}\label{section: cohomology second page}



Corollary \ref{corollary: homotopy} reduces the calculation of the cohomology of the complex $(\CC\otimes \wedge\R^2,\dif +\delta)$ and the construction of ``good'' homotopy operators for it, to the similar questions for the complex $(p_{\F}(\CC)\otimes \wedge\R^2,\tilde{\delta})$:
\begin{equation}\label{eq: diagram}
    \begin{tikzpicture}[baseline= (a).base]
    \node[scale=1] (a) at (0,0){
    \begin{tikzcd}[row sep=small]
    p_{\F}(\CC^0)\otimes\wedge^2\R^2\arrow{rrd}{\phantom{1}\tilde{\delta}}&0&p_{\F}(\CC^2)\otimes\wedge^{2}\R^2 \\
    p_{\F}(\CC^0)\otimes\wedge^1\R^2\arrow{rrd}{\phantom{1}\tilde{\delta}}&0&p_{\F}(\CC^2)\otimes\wedge^{1}\R^2\\
    p_{\F}(\CC^0)\otimes\wedge^{0}\R^2 &0&p_{\F}(\CC^2)\otimes\wedge^{0}\R^2
    \end{tikzcd}
    };
    \end{tikzpicture}
\end{equation}
Here we only pictured the non-trivial differentials and spaces.
In this section we determine these differentials explicitly, we compute partial inverses to them, and give estimates for the latter.

\begin{lemma}\label{lemma: second differential degree one}
The map $\tilde{\delta}$ in degree $(0,q)\to (2,q-1)$ is given by
\begin{align*}
         \tilde{\delta}: p_{\F}(\CC^0)\otimes \wedge^q\R^2&\to  p_{\F}(\CC^2)\otimes \wedge^{q-1}\R^2\\
  e_{\varphi}(g\circ f)\otimes e_i&\mapsto \frac{(-1)^{i+1}}{2\nf}  p_{\F}(e_{\varphi}(g\circ f)\wedge \tilde{\omega}_i)\otimes 1\\
   e_{\varphi}(g\circ f)\otimes e_1\wedge e_2&\mapsto \frac{1}{2\nf}\sum_{i=1}^{2} p_{\F}(e_{\varphi}(g\circ f)\wedge \tilde{\omega}_i)\otimes e_{3-i}
\end{align*}
with $g\in C^{\infty}_0(\C)$, where we used the isomorphism \eqref{eq: zero fol iso}.
\end{lemma}

\begin{proof}
We prove the result in two steps.\\
\noindent\underline{Step 1}: By Proposition \ref{proposition: chain isomorphism}, the map $\rho^*$ from \eqref{eq:cohomology map} fits into a commutative diagram
\begin{equation*}
    \begin{tikzpicture}[baseline= (a).base]
    \node[scale=.9] (a) at (0,0){
    \begin{tikzcd}
    p_{\F}(\CC^0)\otimes\wedge^q\R^2\arrow{d}{\simeq}\arrow{d}[swap]{\rho^*}\arrow{r}{\tilde{\delta}}&p_{\F}(\CC^{2})\otimes\wedge^{q-1}\R^2\arrow{d}{\simeq}\arrow{d}[swap]{\rho^*}\\
    \mathscr{D}^0\otimes\wedge^q\R^2\arrow{r}{\delta_{\mathscr{D}}}&\mathscr{D}^{2}\otimes\wedge^{q-1}\R^2 
    \end{tikzcd}
    };
    \end{tikzpicture}
\end{equation*}
We claim that the map $\delta_{\mathscr{D}}$ is given by
\begin{align}\label{eq:delta:on:skeleton}
 -\frac{\lambda_1}{2|\lambda|^2}e_{\omega_{S^2}}\otimes i_{\varepsilon^1}- \frac{\lambda_2}{2|\lambda|^2}e_{\omega_{S^2}}\otimes i_{\varepsilon^2}
\end{align}
where $\lambda=\lambda_1+i\lambda_2$ are the coordinates on $\C$ and $\varepsilon^i\in (\R^2)^*$ denotes the dual basis to $e_i\in \R^2$. For this, we first recall from \eqref{eq:pullback forms} that
\[ \rho^*\tilde{\omega}_1 =-\lambda_1\cdot \omega_{S^2}\in \Omega^2(S^2\times \C)^{SU(2)\times \Z_2}\]
Hence we obtain 
\[ \rho^*\dif\tilde{\omega}_1 =-\omega_{S^2}\wedge \dif \lambda_1.\]
Next, we define \begin{align}\label{eq: w}
    W_1:=  \frac{\lambda_1\partial_{\lambda_1}-\lambda_2\partial_{\lambda_2}}{2|\lambda |^2}\quad \text{and}\quad
    W_2:= \frac{\lambda_2\partial_{\lambda_1}+\lambda_1\partial_{\lambda_2}}{2|\lambda |^2}. 
\end{align}
Using \eqref{eq:cohomology map explicit} it is easy to check that $V_i$ and $W_i$ are $\rho$-related, i.e.,
\begin{align*}
    \rho_*(W_i)=V_i|_{\Sk\backslash\{0\}}
\end{align*}
From the definition of the $\gamma_i$ in \eqref{eq: gammai} we obtain
\[ \rho^*\gamma_i = \frac{-\lambda_i}{2|\lambda|^2}\omega_{S^2}.\]
Recall from Proposition \ref{proposition:PCH as forms} that $\delta=e_{\gamma_1}\otimes i_{\epsilon^1}+e_{\gamma_2}\otimes i_{\epsilon^2}$. This implies that for $\xi\in p_{\F}(\CC^0)\otimes\wedge^q\R^2$, we have that $\delta_{0}\rho^*(\xi)=\rho^*\delta(\xi)$, where 
$\delta_0$ is the operator in \eqref{eq:delta:on:skeleton}. On the other hand $\tilde{\delta}(\xi)-\delta(\xi)=\dif h_{\F} \delta(\xi)$. Note that $h_{\F}\delta(\xi)$ is $SU(2)$-invariant, and therefore 
\[\rho^*(h_{\F}\delta(\xi))\in e_{\rho^*(\varphi)}(\Omega^1(S^2\times \C)^{SU(2)\times \mathbb{Z}_2})\otimes \wedge^{q-1} \R^2=0.\]
Thus $\rho^*\tilde{\delta}(\xi)=\rho^*\delta(\xi)=\delta_0\rho^*(\xi)$, and this concludes the proof of the claim.


\noindent\underline{Step 2}: The map $\tilde{\delta}$ in degree $(0,1)\to (2,0)$ is obtained as the composition of the following maps. The map $\rho^*$ identifies $p_{\F}(\CC^0)$ with $\mathscr{D}^0$ by
\begin{align*}
    e_{\varphi}(g \circ f)\otimes e_i&\ \mapsto  e_{\rho^*(\varphi)}(g \circ \mathrm{sq})\otimes e_i
\end{align*}
Then we use the map $\delta_{\mathscr{D}}$ from Step 1 to get
\begin{align*}
    e_{\rho^*(\varphi)}(g \circ \mathrm{sq})\otimes e_i&\, \mapsto -\frac{\lambda_i}{2|\lambda|} g (\lambda^2)\, e_{\rho^*(\varphi)}(\omega_{S^2})\otimes 1
\end{align*}
By \eqref{eq:pullback forms}, the inverse of $\rho^*$ in the diagram in Step 1 is given by:
\begin{align*}
    -\frac{\lambda_i}{2|\lambda|}g (\lambda^2)\, e_{\rho^*(\varphi)}(\omega_{S^2})\otimes 1&\, \mapsto \frac{(-1)^{i+1}}{2\nf}p_{\F}( e_{\varphi}(g \circ f)\wedge \tilde{\omega}_{i})\otimes 1
\end{align*}
So we obtain the form of $\tilde{\delta}$ from the statement. The case $(0,2)\to (2,1)$ follows similarly. 
\end{proof}


% \begin{corollary}
% The map $\tilde{\delta}$ in degree $(0,1)\to (2,0)$ is surjective and in degree $(0,2)\to (2,1)$ is injective. Hence, 
% \[H^2(\spl,\pi)=0.\]
% \end{corollary}
% \begin{proof}
% By Proposition \ref{proposition: property H fol} we can identify $p_{\F}(\CC^{\bullet})\simeq H^{\bullet}_0(\F)$, and we use the description from Proposition \ref{proposition:flat foliated ch} of $H^{\bullet}_0(\F)$. That $\tilde{\delta}$ is surjective in degree $(0,1)\to (2,0)$ follows because the map \eqref{eq: quotient} is surjective, and that $\tilde{\delta}$ is injective in degree $(0,2)\to (2,1)$ follows by the description of the kernel of the same map. As discussed at the beginning of Section \ref{section: perturbation Lemma}, the cohomology of $\tilde{\delta}$ is isomorphic to flat Poisson cohomology. Since the formal Poisson cohomology vanishes, the result follows.
% \end{proof}


To obtain homotopy operators for the Poisson complex, we need explicit inverses for the map $\tilde{\delta}$.

\begin{lemma}\label{lemma: right inverse}
A right inverse for $\tilde{\delta}$ in degree $(0,1)\to (2,0)$ is given by 
\begin{align}\label{eq: right inverse map}
    &\mathscr{R}: p_{\F}(\CC^2)\otimes \wedge^0\R^2 \to p_{\F}(\CC^0)\otimes \wedge^1\R^2 \\
    &\sum_{i=1}^2  p_{\F}(e_{\varphi}(g_i\circ f)\wedge \tilde{\omega}_i) \otimes 1 \mapsto  2\nf \sum_{i=1}^2 (-1)^{i+1} e_{\varphi}(g_i\circ f)\otimes e_i\nonumber
\end{align}
with $(g_1,g_2)\in \mathcal{M}$. %Here $p_{\F}(\CC^0_{-\tilde{\tau}})$ denotes the $-1$ eigenspace in $p_{\F}(\CC^0)$ of pullback by complex conjugation $\tilde{\tau}:\spl\diffto \spl$. 
\end{lemma}


\begin{proof} By Propositions \ref{proposition:flat foliated ch} and \ref{proposition: property H fol}, every element in $p_{\F}(\CC^2)$ is of the form
\begin{align*}
    \sum_{i=1}^2 p_{\F}(e_{\varphi}(g_i\circ f) \wedge  \tilde{\omega}_i), \quad \text{ for unique }\ (g_1,g_2)\in \mathcal{M}.
\end{align*}
Hence $\mathscr{R}$ is well-defined, and it is clearly an right inverse to $\tilde{\delta}$.
\end{proof}

Next, we describe a left inverse for $\tilde{\delta}$ in degree $(0,2)\to (2,1)$. For this we will use the following:


\begin{lemma}\label{lemma: trivial module 3}
We have an isomorphism of $C^{\infty}_0(\C)$-modules:
\[C^{\infty}_0(\C)\oplus C^{\infty}_0(\C) \simeq  p_{\F}(\CC^2)\otimes \R^2.\]
More explicitly, for every element $\xi\in p_{\F}(\CC^2)\otimes\R^2$ there exist unique elements $g_1,g_2\in C^{\infty}_0(\C)$ such that
\begin{align}\label{eq: trivialization in (2,1)}
    \xi= g_1\circ f\cdot b_1 +g_2\circ f\cdot b_2,
\end{align}
where $b_1$ and $b_2$ are the sections on the set $\spl\setminus S_0$ given by:
\begin{align*}
    b_1 :=&\,e_{\varphi}\big(p_{\F}(\tilde{\omega}_1)\otimes e_1 - 
    p_{\F}(\tilde{\omega}_2)\otimes e_2\big)\\
    b_2 :=&\,e_{\varphi}\big(p_{\F}(\tilde{\omega}_2)\otimes e_1 + p_{\F}(\tilde{\omega}_1)\otimes e_2\big).
\end{align*}
\end{lemma}
\begin{proof}
First recall that by Proposition \ref{proposition: twisted module} and Proposition \ref{proposition:flat foliated ch} we have the isomorphisms of $C^{\infty}_0(\C)$-modules:
\begin{equation}\label{eq:composition of isomorphisms}
C^{\infty}_0(\C)\oplus C^{\infty}_0(\C)=\mathcal{M}\oplus \mathcal{K}\simeq 
 \mathcal{M}\oplus  \mathcal{M} %\overset{(1,-1)}{\simeq}\mathcal{M}\oplus  \mathcal{M}
 \simeq  p_{\F}(\CC^2)\otimes \R^2.
\end{equation}
The statement follows by applying these isomorphism to a basis on the left. More explicitly, consider the map $\chi:C^{\infty}_0(\C)\oplus C^{\infty}_0(\C)\to p_{\F}(\CC^2)$ given by 
\[\chi(g_1,g_2):=\sum_{i=1}^2 p_{\F}(e_{\varphi}(g_i\circ f) \wedge  \tilde{\omega}_i).\]
We know that $\ker \chi=\mathcal{K}$ and its restriction to $\mathcal{M}$ is an isomorphism. Denote $J(g_1,g_2)=(-g_2,g_1)$. Using that $\id=p_{\mathcal{M}}+ p_{\mathcal{K}}$ and that $J(\mathcal{M})=\mathcal{K}$, we obtain the isomorphism from the statement:
\begin{align*}
(g_1,g_2)\mapsto& (\chi \circ p_{\mathcal{M}}(g_1,g_2))\otimes e_1 +
(\chi \circ (-J)\circ p_{\mathcal{\mathcal{K}}}(g_1,g_2))\otimes e_2=\\
&= \chi (g_1,g_2)\otimes e_1+ \chi(g_2,-g_1)\otimes e_2=\\
&=g_1\circ f \cdot b_1+ g_2\circ f\cdot b_2.\qedhere
\end{align*}

\end{proof}
With the notation from the lemma, $\tilde{\delta}$ in degree $(0,2)\to (2,1)$ becomes:
\begin{align}\label{eq: delta degree 2}
    \tilde{\delta}(e_{\varphi}(g\circ f)\otimes e_1\wedge e_2)= \frac{1}{2|f|}g\circ f\cdot b_2.
\end{align}
Therefore, the lemma implies the following: 

\begin{lemma}\label{lemma: second differential degree two}
A left inverse of $\tilde{\delta}$ in degree $(0,2)\to (2,1)$ is given by 
\begin{align}\label{eq: left inverse}
\mathscr{L}&: p_{\F}(\CC^2)\otimes \wedge^1\R^2 \to p_{\F}(\CC^0)\otimes \wedge^2\R^2 \\
&\sum_{i=1}^2 g_i\circ f\cdot b_i\mapsto  2\nf\, e_{\varphi}(g_2\circ f)\otimes e_1\wedge e_2.\nonumber
\end{align}
\end{lemma}


Next, we estimate these maps. 

\begin{lemma}\label{lemma: r}
The maps $\mathscr{R}$ and $\mathscr{L}$ satisfy property SLB for $(0,1,2)$.
\end{lemma}
\begin{proof} 
In order to obtain the estimate for the map $\mathscr{R}$ \eqref{eq: right inverse map}, we write it as a composition of several maps which we estimate one by one: 
\begin{equation}\label{eq: op contraction}
    \begin{array}{ccccccc}
        p_{\F}(\CC^2)&\xrightarrow{\rho^*}&\mathscr{D}^{2}&\xrightarrow{\zeta }&\mathscr{D}^{0} \otimes \R^2&\xrightarrow{(\rho^*)^{-1}\otimes \id }&p_{\F}(\CC^0)\otimes \R^2 
    \end{array}
\end{equation}
where we use the cochain isomorphism $\rho^*$ from Proposition \ref{proposition: chain isomorphism}, and
\[ \zeta :=-2\lambda_1 i_{\pi_{S^2}}\otimes e_1-2\lambda_2 i_{\pi_{S^2}}\otimes e_2\]
with $\pi_{S^2}=\omega_{S^2}^{-1}$ the Poisson structure on $S^2$ dual to $\omega_{S^2}$. Next, let us see that this composition is indeed $\mathscr{R}$. Using \eqref{eq:pullback forms} for $\rho^*(\tilde{\omega}_i)$ and \eqref{eq:final:to:prove} we obtain for $(g_1,g_2)\in \mathcal{M}$ that
\begin{align*}
    \sum_{i=1}^2g_i\circ f\cdot e_{\varphi}(p_{\F}(\tilde{\omega}_i))\mapsto &\ \sum_{i=1}^2(-1)^{i}\lambda_i g_i\circ \mathrm{sq}\cdot  \rho^*(\varphi)\wedge \omega_{S^2}\\
    \mapsto &\ 2\sum_{j=1}^2(-1)^{j+1}(|z|\cdot g_j)\circ \mathrm{sq}\cdot \rho^*(\varphi)\otimes e_j\\
    \mapsto &\ 2\nf \sum_{j=1}^2(-1)^{j+1} e_{\varphi}(g_j\circ f)\otimes e_j
\end{align*}
Here we used for the second map that
\begin{align*}
    (g_1,g_2)\in \mathcal{M} \quad \Longleftrightarrow \quad \lambda_2 g_1\circ \mathrm{sq}=-\lambda_1 g_2\circ \mathrm{sq}  
\end{align*}
by pulling back the relation in \eqref{eq: definition M} by $\mathrm{sq}:\C\to \C$ and hence, for $j=1,2$:
\begin{align*}
    -\lambda_j\sum_{i=1}^2(-1)^{i}\lambda_i g_i\circ \mathrm{sq}=(-1)^{j+1}|\lambda|^2\cdot g_j\circ\mathrm{sq} =(-1)^{j+1}(|z|\cdot g_j)\circ \mathrm{sq}.
\end{align*}
In the following we estimate each of the maps in \eqref{eq: op contraction} separately.\\
 \noindent\underline{Step 1}: We have for $\beta\in \Omega_0^{\bullet}(\spl)$ the inequality
\begin{align}\label{Step four crazy Lemma}
    \fnorm{\rho^*(\beta)}_{n,k,\frac{r}{\sqrt{2}}}^{S^2\times \C}\le C\cdot \fnorm{\beta}_{n,k,r}
\end{align}
for a constant $C=C(n,k,r)$ depending continuously on $r>0$. Here the semninorms on the left are defined as follows. Equip the $n$-th jet bundle of the vector bundle
\begin{align*}
    \wedge^\bullet T^*(S^2\times\C)\to S^2\times\C
\end{align*}
with a norm $|\cdot|^{jet}$. Then, for $\alpha \in \Omega^{\bullet}_0(S^2\times \C)$, define: 
\begin{align*}
    \fnorm{\alpha}_{n,k,s}^{S^2\times \C}:= \sup_{(w,\lambda)\in S^2\times\overline{B}_s}\ |\lambda|^{-k}|j^n\alpha(w,\lambda)|^{jet}.
\end{align*}
We obtain \eqref{Step four crazy Lemma} by compactness of $S^2$ and using
\begin{align*}
    \sqrt{2}|\lambda| = R\circ \rho (w,\lambda),
\end{align*}
which follows by Lemma \ref{lemma: characterization skeleton} (3) and by Lemma \ref{lemma:identification of skeleton} (2). 

\noindent\underline{Step 2}: Note that for $\alpha\in \mathscr{D}^2$ we have
\begin{align}\label{Step three crazy Lemma}
    \fnorm{\zeta (\alpha)}_{n,k,s}^{\C} \le C\cdot \fnorm{\alpha}_{n,k,s}^{S^2\times \C}
\end{align}
for a constant $C(n,k,s)$ depending continuously on $0<s$. Here we used the seminorms $\fnorm{\cdot }_{n,k,s}^{\C}$ on $C^{\infty}_0(\C)$, defined as in \eqref{eq: flat norms}.


\noindent\underline{Step 3}: We show that for $g\in C^{\infty}_0(\C)$ we have
\begin{align}\label{Step one in crazy lemma}
    \fnorm{g\circ f\cdot \varphi }_{n,k,r}\le C\cdot \fnorm{g\circ \mathrm{sq}\cdot \rho^*(\varphi)
    }^{\C}_{n,k+n+2,\frac{r}{\sqrt{2}}}.
\end{align}
Clearly, we have that:
\begin{align*}
    \fnorm{g\circ f\cdot \varphi}_{n,k,r}\le C\cdot \fnorm{g\circ f}_{n,k,r}
\end{align*}
By the explicit form of the vector fields $W_1$ and $W_2$ from \eqref{eq: w}, we have that, for any $g\in C^{\infty}_0(\C)$, and for $i=1,2$:
\begin{align*}
    (\partial_i g)\circ \mathrm{sq} = \Lie_{W_i} (g\circ \mathrm{sq}). 
\end{align*}
For all $u\in C^{\infty}_0(\C)$ and $i=1,2$ we have:
\begin{align}\label{eq:norm of Lie W}
    \fnorm{\Lie_{W_i}u}_{n,k,s}^{\C}\le C\cdot \fnorm{u}_{n+1,k+1,s}^{\C}.
\end{align}
This follows by Lemma \ref{lemma:singular:vb:maps} applied to the coefficients of $W_i$. Using the general chain rule from Subsection \ref{subsection: derivatives} and $2\nf\le R^2$ from \eqref{eq:norm-fiber inequality}, we obtain for $a\in \N_0^6$, $k\in \N_0$, $0< R \le r$ and $g\in C^{\infty}_0(\C)$ that
\[\frac{|D^a(g\circ f)|}{R^k} \le  C\cdot \frac{1}{\nf^{\frac{k}{2}}} \sum_{1\leq |b|\leq |a|}|D^b( g)\circ f|.\]
By $2\nf\le R^2$ and by applying $f$ to diagonal matrices, we note that:
\[f(\overline{B}_r)=\overline{B}_{r^2/2}.\]
For $A\in \overline{B}_r$, let $\lambda\in \overline{B}_{r/\sqrt{2}}$ such that $f(A)=\lambda^2$. Then the above gives:
\begin{align*}
    \frac{|D^a(g\circ f)|}{R^k}     \le &\ C\cdot \frac{1}{|\lambda|^{k}} \sum_{1\leq |b|\leq |a|}|D^b( g)\circ \mathrm{sq}|\\
    = &\ C\cdot \frac{1}{|\lambda|^{k}}\sum_{1\leq |b|\leq |a|}|\Lie_{W_1}^{b_1}\Lie_{W_2}^{b_2} (g\circ \mathrm{sq})|\\
    \le &\ C\cdot\sum_{1\leq |b|\leq |a|}\fnorm{\Lie_{W_1}^{b_1}\Lie_{W_2}^{b_2} (g\circ \mathrm{sq})}_{0,k,\frac{r}{\sqrt{2}}}^{\C}\\
    \le &\ C\cdot \fnorm{g\circ \mathrm{sq}}_{|a|,k+|a|,\frac{r}{\sqrt{2}}}^{\C},
\end{align*}
where in the last step we used \eqref{eq:norm of Lie W} inductively. This proves \eqref{Step one in crazy lemma} using Lemma \ref{lemma:singular:vb:maps} and the form of $\rho^*(\varphi)$ \eqref{eq:pull back of varphi}. 

Applying the estimates from Step 1 to 3 in reverse order proves that the map $\mathscr{R}$ satisfies property SLB for $(0,1,2)$. 

To estimate $\mathscr{L}$ we denote by $e_{e_j}$ and $i_{\varepsilon^j}$ the exterior and interior product on $\wedge^q\R^2$ with $e_j$ and $\varepsilon^j$, respectively. We claim that:
\begin{align*}
%    \mathscr{L}&: p_{\F}(\CC^2)\otimes \wedge^1\R^2 \to p_{\F}(\CC^0)\otimes \wedge^2\R^2 \\
    \mathscr{L}=-(\id\otimes e_{e_1})\circ \mathscr{R}\circ (\id \otimes i_{\varepsilon ^1})-(
    \id\otimes e_{e_2})\circ \mathscr{R}\circ (\id \otimes i_{\varepsilon^2})
\end{align*}
For this, consider an arbitrary element $g_1\circ f\cdot b_1+g_2\circ f\cdot b_2\in p_{\F}(\CC^2)\otimes \R^2$. 
Then applying the first operator in the sum, we obtain:
\begin{align*}
g_1\circ f\cdot b_1+g_2\circ f\cdot b_2\ \  \stackrel{\id\otimes i_{\varepsilon^1}}{\mapsto}\quad \, &  g_1\circ f\cdot p_{\F}(e_{\varphi}(\tilde{\omega}_1))+g_2\circ f \cdot p_{\F}(e_{\varphi}(\tilde{\omega}_2))\\
=\qquad & \big(\frac{1}{2|z|}((|z|+x)g_1-yg_2)\big)\circ f\cdot p_{\F}(e_{\varphi}(\tilde{\omega}_1))\\
&+\big(\frac{1}{2|z|}((|z|-x)g_2-yg_1)\big)\circ f \cdot p_{\F}(e_{\varphi}(\tilde{\omega}_2))\\
\stackrel{-(\id\otimes e_{e_1})\circ \mathscr{R}}{\mapsto} &\,((|z|-x)g_2-yg_1)\circ f\cdot \varphi\otimes e_1\wedge e_2,
\end{align*}
where in the equality we have used the projection $p_{\mathcal{M}}$. Similarly, for the second operator, one obtains:
\begin{align*}
g_1\circ f\cdot b_1+g_2\circ f\cdot b_2\ \  \stackrel{\id\otimes i_{\varepsilon^2}}{\mapsto}\quad \, &  -g_1\circ f\cdot p_{\F}(e_{\varphi}(\tilde{\omega}_2))+g_2\circ f \cdot p_{\F}(e_{\varphi}(\tilde{\omega}_1))\\
=\qquad & \big(\frac{1}{2|z|}((|z|+x)g_2+yg_1)\big)\circ f\cdot p_{\F}(e_{\varphi}(\tilde{\omega}_1))\\
& -\big(\frac{1}{2|z|}((|z|-x)g_1+yg_2)\big)\circ f \cdot p_{\F}(e_{\varphi}(\tilde{\omega}_2))\\
\stackrel{-(\id\otimes e_{e_2})\circ \mathscr{R}}{\mapsto} &\,((|z|+x)g_2+yg_1)\circ f\cdot \varphi\otimes e_1\wedge e_2,
\end{align*}
% \begin{align*}
% g_1\circ f\cdot b_1+g_2\circ f\cdot b_2\mapsto  &\,((|z|+x)g_1-yg_2)\circ f\cdot \varphi\otimes e_1\wedge e_2,
% \end{align*}
which yields the claim. Since $\mathscr{L}$ is obtained by combining $\mathscr{R}$ with the exterior and interior products by $e_i$ and $\varepsilon^i$, respectively, it follows that $\mathscr{L}$ also satisfies property SLB for $(0,1,2)$.
\end{proof}

\subsubsection{A homotopy equivalence data}\label{section: HE data}

Corollary \ref{corollary: homotopy} reduces the complex $(\CC^{\bullet}\otimes \wedge^{\bullet}\R^2,\dif +\delta)$, and the construction of ``good'' homotopy operators for it, to the complex $(p_{\F}(\CC^{\bullet})\otimes \wedge^{\bullet}\R^2,\tilde{\delta})$. The previous subsection allows us to deal with the latter.   
\begin{corollary}\label{proposition: homotopy}
The complex $(p_{\F}(\CC^{\bullet})\otimes \wedge^{\bullet}\R^2,\tilde{\delta})$ admits the HE data
\begin{align}\label{eq: HE data E}
    (\widetilde{\mathscr{E}}^{\bullet},0)\stackrel[\iota ]{p}{\leftrightarrows}(p_{\F}(\CC)\otimes \wedge\R^2,\tilde{\delta}),h
\end{align}
where $\widetilde{\mathscr{E}}$ is the subcomplex given by 
\begin{align*}%\label{eq: he data}
    \widetilde{\mathscr{E}}^k:= \begin{cases}
        p_{\F}(\CC^0)\otimes \wedge^0\R^2 &\text{ for } k=0\\
        \ker \tilde{\delta}&\text{ for } k=1\\
        \mathrm{coker}\, \tilde{\delta}&\text{ for } k=3\\
        p_{\F}(\CC^2)\otimes \wedge^2\R^2 &\text{ for } k=4\\
        0&\text{ for }k=2,5,6
    \end{cases}
\end{align*}
satisfying
\begin{align*}
    p \circ \iota =\id_{\widetilde{\mathscr{E}}},
\end{align*}
and $h$ satisfy property SLB for $(0,1,2)$. \end{corollary}

\begin{proof}
The maps $\iota$ are the standard inclusions. We give the maps $p$ and $h$ in every degree. \\
\noindent\textbf{In degree $0$}: The map $p=\id$ and $h=0$.\\
\noindent\textbf{In degree $1$}: The map $p$ is defined by
\begin{align*}
    p:= \id -\mathscr{R}\circ \tilde{\delta}
\end{align*}
and the map $h$ is given by
\begin{equation*}
    \begin{array}{cccc}
         h:& p_{\F}(\CC^0)\otimes \wedge ^2\R^2\oplus\, 0 \oplus p_{\F}(\CC^2)\otimes \wedge ^0\R^2&\to & p_{\F}(\CC^0)\otimes \wedge ^1\R^2\oplus\, 0 \\
         & (\alpha^{0,2},0,\alpha^{2,0})&\mapsto &(-\mathscr{R}(\alpha^{2,0}),0)
    \end{array}
\end{equation*}
\noindent\textbf{In degree $2$}: Here $p=0$ and $h$ is defined by
\begin{equation*}
    \begin{array}{cccc}
         h:& 0\oplus p_{\F}(\CC^2)\otimes \wedge ^1\R^2\oplus \, 0&\to &p_{\F}(\CC^0)\otimes \wedge ^2\R^2\oplus\, 0 \oplus p_{\F}(\CC^2)\otimes \wedge ^0\R^2 \\
         & (0,\alpha^{2,1},0)&\mapsto &(-\mathscr{L}(\alpha^{2,1}),0,0)
    \end{array}
\end{equation*}
where the map $\mathscr{L}$ is given in \eqref{eq: left inverse}.

\noindent\textbf{In degree $3$}: The projection map $p$ is given by
\begin{align*}
    p := \id -\tilde{\delta}\circ \mathscr{L} 
\end{align*}
and $h$ is the zero map.\\
\noindent\textbf{In degree $4$}: Here $p=\id$ and $h=0$. 

Finally, by Lemma \ref{lemma: r}, $h$ has property SLB for $(0,1,2)$.
\end{proof}




\subsubsection{The flat Poisson cohomology of $\spl$}\label{section: flat pch}

As a corollary of the previous subsections, we obtain the description of the flat Poisson cohomology groups of $(\spl,\pi)$ together with a deformation retraction to a complex with trivial differential. The algebraic structure of the flat Poisson cohomology groups is discussed in Subsection \ref{section: algebra}.

\begin{theorem}\label{main theorem}
The flat Poisson complex $(\mathfrak{X}^{\bullet}_0(\spl),\dif_{\pi})$ admits HE data
\[ \begin{tikzcd}[every arrow/.append style={shift right}] 
(\mathscr{E}^{\bullet},0) \arrow{r}[swap]{\iota _{\spl}} &(\mathfrak{X}^{\bullet}_0(\spl) ,\dif_{\pi}),h_{\spl} \arrow{l}[swap]{p_{\spl}}
\end{tikzcd}\]
where $\mathscr{E}$ is given by 
\begin{align*}%\label{eq: he data}
    \mathscr{E}^k:= \begin{cases}
    C^{\infty}_0(\C) &\text{ for } k=0,3\\
    \mathcal{M}&\text{ for } k=1,4\\
        0&\text{ for }k=2,5,6
    \end{cases}
\end{align*}
such that
\[ p_{\spl}\circ \iota_{\spl}=\id_{\mathscr{E}},\]
and such that the maps $\iota_{\spl}\circ p_{\spl}$ and $h_{\spl}$ satisfies property SLB for $(2,21,188)$ and $(1,21,167)$, respectively. 

In particular, the map $\iota_{\spl}$ induces an isomorphism of $C^{\infty}_0(\mathbb{C})$-modules
\begin{equation}\label{eq: isoPC}
    I^{\bullet}:\mathscr{E}^{\bullet}\diffto H^{\bullet}_0(\spl,\pi)
\end{equation}
and in degree $2$ we have the homotopy relation
\begin{align*}
    \id_{\mathfrak{X}^{2}_0(\spl)}=h_{\spl}\circ \dif_{\pi}+\dif_{\pi}\circ h_{\spl}
\end{align*}
\end{theorem}

\begin{proof}
Note that we have an isomorphism $\epsilon:\mathscr{E}^{\bullet}\diffto \widetilde{\mathscr{E}}^{\bullet}$ given as follows:\\ 
\noindent\textbf{In degree $0$}, $\epsilon$ is the isomorphism from \eqref{eq: zero fol iso}.\\
\noindent\textbf{In degree $1$}, $\epsilon$ is given by
\begin{align}\label{eq: kernel 01}
   \epsilon: \quad \mathcal{M}\quad &\diffto \qquad\qquad  \ker \tilde{\delta} \\
    (g_1,g_2)  &\mapsto  \ e_{\varphi}(g_2\circ f)\otimes e_1  + e_{\varphi}( g_1\circ f) \otimes e_2\nonumber
\end{align}
That this map is a well-defined isomorphism follows by Lemma \ref{lemma: second differential degree one}, the description of the kernel of the map \eqref{eq: quotient} in Proposition \ref{proposition:flat foliated ch}, and the isomorphism $\mathcal{M}\simeq \mathcal{K}$ from Proposition
\ref{proposition: twisted module}.\\
\noindent\textbf{In degree $3$}, $\epsilon$ is given by
\begin{align}\label{eq: iso degree 3}
    \epsilon: C^{\infty}_{0}(\C)&\diffto \quad \mathrm{coker}\, \tilde{\delta}   \\
     g&\mapsto\ g\circ f\cdot e_{\varphi}(b_1)  \nonumber
\end{align}
This is an isomorphism by Lemma \ref{lemma: trivial module 3} and \eqref{eq: delta degree 2}.\\
\noindent\textbf{In degree $4$}, $\epsilon$ is given by
\begin{align}\label{eq: iso degree 4}
    \epsilon: \mathcal{M}&\diffto p_{\F}(\CC^2)\otimes \wedge^2\R^2 \\
    (g_1,g_2)\mapsto &\sum_{i=1}^2 p_{\F}(g_i\circ f\cdot e_{\varphi}(\tilde{\omega}_i))\otimes e_1\wedge e_2\nonumber
\end{align}
which, by Proposition \ref{proposition:flat foliated ch}, is an isomorphism. 

The HE data is obtained from the cochain isomorphism $\tilde{a}$ in Proposition \ref{proposition:PCH as forms}, the isomorphism $\epsilon$ and the HE data from Corollary \ref{corollary: homotopy} and Corollary \ref{proposition: homotopy}.
By using that HE data behave functorial \cite[Lemma 2.4]{LS87}, the formulas for the composition yield:
\begin{align*}
    \iota_{\spl}:= \tilde{a}^{-1}\circ \tilde{\iota} \circ \iota\circ \epsilon,& \qquad p_{\spl}:= \epsilon^{-1}\circ p\circ \tilde{p} \circ \tilde{a} \\ h_{\spl}=\tilde{a}^{-1}\, \circ &\, (\tilde{\iota}\circ h\circ  \tilde{p}+\tilde{h})\circ \tilde{a}.
\end{align*}
That these form an HE data, can be checked directly:
\begin{align*}
    \iota _{\spl} \circ p_{\spl}-\id =&\ \tilde{a}^{-1}\circ \tilde{\iota}\circ \iota\circ p \circ  \tilde{p}\circ \tilde{a}-\id\\
    =&\ \tilde{a}^{-1}\circ \tilde{\iota}\circ (\iota \circ p -\id ) \circ  \tilde{p}\circ \tilde{a}+\tilde{a}^{-1}\circ\big(\tilde{\iota} \circ  \tilde{p}- \id\big)\circ \tilde{a}\\
    =&\ \tilde{a}^{-1}\circ \big( \tilde{\iota}\circ (\tilde{\delta}\circ h+h\circ \tilde{\delta} ) \circ  \tilde{p}\big) \circ \tilde{a} \\
    &\ +\tilde{a}^{-1}\circ\big((\dif +\delta) \circ \tilde{h} +\tilde{h}\circ (\dif+\delta)\big)\circ \tilde{a}\\
    =&\ \tilde{a}^{-1}\circ \big( (\dif+ \delta) \circ \big( \tilde{\iota}\circ h\circ  \tilde{p}+\tilde{h}\big)\big)\circ \tilde{a}\\
    &\ + \tilde{a}^{-1}\circ \big( \tilde{\iota}\circ h\circ  \tilde{p}+\tilde{h}\big) \circ (\dif+\delta)\big)\circ \tilde{a}\\
    =&\ \tilde{a}^{-1}\circ (\dif+ \delta)\circ \tilde{a}\circ   h_{\spl} + 
     h_{\spl}\circ \tilde{a}^{-1}\circ  (\dif+ \delta)\circ \tilde{a}\\
     =&\ \dif_{\pi}\circ h_{\spl}+h_{\spl}\circ \dif_{\spl}.
\end{align*}
Finally, Proposition \ref{proposition:PCH as forms}, Corollary \ref{corollary: homotopy}, Corollary \ref{proposition: homotopy} and Lemma \ref{lemma: slb property} imply that  $h_{\spl}$ satisfy the SLB property for $(1,21,188)$. Since $\dif_{\pi}$ satisfies the SLB property for $(1,0,0)$, again Lemma \ref{lemma: slb property} implies the claimed SLB property for $\iota_{\spl}\circ p_{\spl}$.
\end{proof}

% {\color{red}
% \subsubsection{A homotopy equivalence data}\label{section: HE data}

% Corollary \ref{corollary: homotopy} reduces the complex $(\CC^{\bullet}\otimes \wedge^{\bullet}\R^2,\dif +\delta)$, and the construction of ``good'' homotopy operators for it, to the complex $(p_{\F}(\CC^{\bullet})\otimes \wedge^{\bullet}\R^2,\tilde{\delta})$. The previous subsection allows us to deal with the latter.   
% \begin{proposition}\label{proposition: homotopy}
% The complex $(\CC\otimes \wedge\R^2,\dif+\delta)$ admits the HE data
% \begin{align}\label{eq: HE data E}
%     (\mathscr{E},0)\stackrel[\iota _{\mathscr{E}}]{p_{\mathscr{E}}}{\leftrightarrows}(\CC\otimes \wedge\R^2 ,\dif+\delta),h_{\mathscr{E}}
% \end{align}
% where $\mathscr{E}$ is given by 
% \begin{align*}%\label{eq: he data}
%     \mathscr{E}^k:= \begin{cases}
%     C^{\infty}_0(\C) &\text{ for } k=0,3\\
%     \mathcal{M}&\text{ for } k=1,4\\
%         0&\text{ for }k=2,5,6
%     \end{cases}
% \end{align*}
% satisfying
% \begin{align*}
%     p_{\mathscr{E}} \circ \iota_{\mathscr{E}} =\id_{\mathscr{E}},
% \end{align*}
% and the maps $\iota_{\mathscr{E}}\circ p_{\mathscr{E}}$ and $h_{\mathscr{E}}$ satisfy property SLB for $(2,21,185)$ and $(1,21,161)$, respectively. In particular, $(\iota_{\mathscr{E}}\circ p_{\mathscr{E}}, h_{\mathscr{E}})$ is a deformation retract onto a subcomplex with 0 differential.
% \end{proposition}

% \begin{proof}
% We prove the proposition in two steps.\\
% \noindent\underline{Step 1}: We use the previous subsections to construct an HE data
% \begin{align*}
%     (\mathscr{E},0)\stackrel[\iota]{p}{\leftrightarrows}(p_{\F}(C),\tilde{\delta}),h 
% \end{align*}
% where $C$ denotes the complex defined in \eqref{eq: complex short}. We describe the maps $\iota$, $p$ and $h$ in every degree. \\
% \noindent\textbf{In degree $0$}: The map $\iota$ is the isomorphism from \eqref{eq: zero fol iso}, $p=\iota^{-1}$ and $h=0$.\\
% \noindent\textbf{In degree $1$}: 
% We define $\iota$ in degree $1$ by
% \begin{align}\label{eq: kernel 01}
%   \iota: \mathcal{M}&\diffto \ker \tilde{\delta}\subset p_{\F}(\CC^0)\otimes\wedge^1\R^2 \\
%     (g_1,g_2)  \mapsto  &\ e_{\varphi}(g_2\circ f)\otimes e_1  + e_{\varphi}( g_1\circ f) \otimes e_2\nonumber
% \end{align}
% That this map is a well-defined isomorphism follows by Lemma \ref{lemma: second differential degree one}, the description of the kernel of the map \eqref{eq: quotient} in Proposition \ref{proposition:flat foliated ch}, and the isomorphism $\mathcal{M}\simeq \mathcal{K}$ from Proposition
% \ref{proposition: twisted module}. The map $p$ is defined by
% \begin{align*}
%     p:= \iota^{-1}\circ (\id -\mathscr{R}\circ \tilde{\delta})
% \end{align*}
% and the map $h$ is given by
% \begin{equation*}
%     \begin{array}{cccc}
%          h:& p_{\F}(C^2)&\to &p_{\F}(C^1) \\
%          & (\alpha^{0,2},0,\alpha^{2,0})&\mapsto &(-\mathscr{R}(\alpha^{2,0}),0)
%     \end{array}
% \end{equation*}
% \noindent\textbf{In degree $2$}: $\iota =0$, $p=0$ and $h$ is defined by
% \begin{equation*}
%     \begin{array}{cccc}
%          h:& p_{\F}(C^3)&\to &p_{\F}(C^2) \\
%          & (0,\alpha^{2,1},0)&\mapsto &(-\mathscr{L}(\alpha^{2,1}),0,0)
%     \end{array}
% \end{equation*}
% where the map $\mathscr{L}$ is given in \eqref{eq: left inverse}.

% \noindent\textbf{In degree $3$}: We define $\iota$ by
% \begin{align}\label{eq: iso degree 3}
%     \iota: C^{\infty}_{0}(\C)&\diffto \ker \mathscr{L} \subset p_{\F}(\CC^2)\otimes \wedge^1 \R^2  \\
%      g&\mapsto g\circ f\cdot e_{\varphi}(b_1)  \nonumber
% \end{align}
% This is an isomorphism by Lemma \ref{lemma: second differential degree two}. The projection map $p$ is given by
% \begin{align*}
%     p := \iota^{-1}\circ(\id -\tilde{\delta}\circ \mathscr{L}) 
% \end{align*}
% and $h$ is the zero map.\\
% \noindent\textbf{In degree $4$}: As $\tilde{\delta}=0$, Proposition \ref{proposition:flat foliated ch} implies that 
% \begin{align}\label{eq: iso degree 4}
%     \iota: \mathcal{M}&\diffto p_{\F}(\CC^2)\otimes \wedge^2\R^2 \\
%     (g_1,g_2)\mapsto &\sum_{i=1}^2 p_{\F}(g_i\circ f\cdot e_{\varphi}(\tilde{\omega}_i))\otimes e_1\wedge e_2\nonumber
% \end{align}
% is an isomorphism. Take $p=\iota^{-1}$ and $h=0$. 

% \noindent\underline{Step 2}: Since HE data behave functorial \cite[Lemma 2.4]{LS87}, the desired HE data is obtained by combing Step 1 with Corollary \ref{corollary: homotopy}. With the notation there, the maps $\iota_{\mathscr{E}}$ and $p_{\mathscr{E}}$ are defined by 
% \begin{align*}
%     \iota_{\mathscr{E}}:= \tilde{\iota} \circ \iota, \ \ \ \ \ \ p_{\mathscr{E}}:= p\circ \tilde{p}.
% \end{align*}
% Note that by definition we have
% \begin{align*}
%     p\circ \iota = \id _{\mathscr{E}}
% \end{align*}
% The map $\tilde{p}\circ \tilde{\iota}$ is the identity on all degrees except for total degree 2. However, since $\mathscr{E}^2=0$, the above implies that:
% \begin{align*}
%     p_{\mathscr{E}}\circ \iota_{\mathscr{E}} =\id_{\mathscr{E}}
% \end{align*}
% To obtain the homotopy $h_{\mathscr{E}}$ we note that we have
% \begin{align*}
%     \iota _{\mathscr{E}} \circ p_{\mathscr{E}}-\id =&\ \tilde{\iota}\circ \iota\circ p \circ  \tilde{p}-\id\\
%     =&\ \tilde{\iota}\circ (\iota \circ p -\id ) \circ  \tilde{p}+\tilde{\iota} \circ  \tilde{p}- \id\\
%     =&\ \tilde{\iota}\circ (\tilde{\delta}\circ h+h\circ \tilde{\delta} ) \circ  \tilde{p} +(\dif +\delta) \circ \tilde{h} +\tilde{h}\circ (\dif+\delta)\\
%     =&\ (\dif+ \delta) \circ \big( (\tilde{\iota}\circ h\circ  \tilde{p})+\tilde{h}\big) + \big( (\tilde{\iota}\circ h\circ  \tilde{p})+\tilde{h}\big) \circ (\dif+\delta)\\
%     =&\ (\dif+ \delta)\circ  h_{\mathscr{E}} + 
%      h_{\mathscr{E}}\circ (\dif+ \delta), 
% \end{align*}
% where we define: 
% \[ h_{\mathscr{E}}:=\tilde{\iota}\circ h\circ  \tilde{p}+\tilde{h}.\]

% By Lemma \ref{lemma: r}, $h$ has property SLB for $(0,1,2)$. Therefore, by using Corollary \ref{corollary: homotopy}, Lemma \ref{lemma: slb property} implies that $h_{\mathscr{E}}$ has property SLB for $(1,21,161)$. Next, since $(\dif+\delta)$ has SLB property for $(1,0,3)$, the homotopy relation and again Lemma \ref{lemma: slb property} imply that $\iota _{\mathscr{E}} \circ p_{\mathscr{E}}$ has the SLB property for $(2,21,185)$.
% \end{proof}




% \subsubsection{The flat Poisson cohomology of $\spl$}\label{section: flat pch}

% As a corollary of the previous subsections, we obtain the description of the flat Poisson cohomology groups of $(\spl,\pi)$ together with a deformation retraction to a complex with trivial differential. The algebraic structure of the flat Poisson cohomology groups is discussed in Subsection \ref{section: algebra}.

% \begin{theorem}\label{main theorem}
% The flat Poisson complex $(\mathfrak{X}^{\bullet}_0(\spl),\dif_{\pi})$ admits HE data
% \[ \begin{tikzcd}[every arrow/.append style={shift right}] 
% (\mathscr{E}^{\bullet},0) \arrow{r}[swap]{\iota _{\spl}} &(\mathfrak{X}^{\bullet}_0(\spl) ,\dif_{\pi}),h_{\spl} \arrow{l}[swap]{p_{\spl}}
% \end{tikzcd}\]
% where $\mathscr{E}$ is defined in Proposition \ref{proposition: homotopy}, such that
% \[ p_{\spl}\circ \iota_{\spl}=\id_{\mathscr{E}},\]
% and such that the maps $\iota_{\spl}\circ p_{\spl}$ and $h_{\spl}$ satisfies property SLB for $(2,21,191)$ and $(1,21,167)$, respectively. 

% In particular, the map $\iota_{\spl}$ induces an isomorphism of $C^{\infty}_0(\mathbb{C})$-modules
% \[I^{\bullet}:\mathscr{E}^{\bullet}\diffto H^{\bullet}_0(\spl,\pi)\]
% and in degree $2$ we have the homotopy relation
% \begin{align*}
%     \id_{\mathfrak{X}^{2}_0(\spl)}=h_{\spl}\circ \dif_{\pi}+\dif_{\pi}\circ h_{\spl}
% \end{align*}
% \end{theorem}

% \begin{proof}
% The HE data is obtained by using the cochain isomorphisms $\tilde{a}$ and $\tilde{b}=\tilde{a}^{-1}$ from Proposition \ref{proposition:PCH as forms} and the HE data from Proposition \ref{proposition: homotopy}:
% \begin{align*}
%     \iota_{\spl}:= \tilde{b}\circ \iota_{\mathscr{E}}, \qquad p_{\spl}:= p_{\mathscr{E}} \circ \tilde{a} \qquad h_{\spl}=\tilde{b}\circ h_{\mathscr{E}}\circ \tilde{a}.
% \end{align*}
% Finally, by Proposition \ref{proposition:PCH as forms}, Proposition \ref{proposition: homotopy} and Lemma \ref{lemma: slb property} we obtain that $\iota_{\spl}\circ p_{\spl}$ and $h_{\spl}$ satisfy the claimed SLB properties.
% \end{proof}}

\subsection{The proof of Theorem \ref{theorem: PC}}\label{section: algebra}

In degree 0, the isomorphism was already proven in Proposition \ref{prop:Casimirs}. For the other degrees, we will give an explicit description for the isomorphism $I^{\bullet}$ in \eqref{eq: isoPC}. First of all, to identify the $C^{\infty}(\C)$-module structure, note that the maps $I^{\bullet}$ are $C^{\infty}(\C)$-linear (where we identify $H^{0}(\spl,\pi)\simeq C^{\infty}(\C)$). 

First, we claim that, for $(g_1,g_2)\in \mathcal{M}$ the class $I^1(g_1,g_2)\in H^1_0(\spl,\pi)$ acts on $C^{\infty}(\C)$ via the derivation 
\[\frac{1}{2|z|}(g_1\cdot Y_1+ g_2\cdot Y_2)\in \out.\]
Note that this suffices to obtain the description from the theorem of the first Poisson cohomology group: it shows that the claimed map is an isomorphism, and since the Lie bracket is determined by the action on functions, it follows that the isomorphism preserves the Lie bracket. 

Indeed, applying the maps $\epsilon$ in \eqref{eq: kernel 01}, the inclusion $\iota$ in Corollary \ref{proposition: homotopy} and $\tilde{\iota}$ in Corollary \ref{corollary: homotopy}, we obtain that
\[ I^1(g_1,g_2)=\tilde{a}^{-1} (\epsilon(g_1,g_2)+h_{\F}\circ \delta(\epsilon(g_1,g_2))).\]
Note that, since $h_{\F}\circ \delta(\epsilon(g_1,g_2))\in \CC^1\otimes \wedge^0\R^2$, we have that, for $i=1,2$:
\[ i_{\dif f_i} (\tilde{a}^{-1} \circ h_{\F}\circ \delta(\epsilon(g_1,g_2)))=0.\]
By definition of $\tilde{a}^{-1}$ in \eqref{eq: tilde b} and of $\epsilon$ we get for the first term
\begin{equation}\label{eq: deg 1 top part}
    \tilde{a}^{-1} (\epsilon(g_1,g_2))= g_2\circ f\cdot V_1+g_1\circ f\cdot V_2.
\end{equation}
By using \eqref{eq:v transversality}, we conclude that $I^1(g_1,g_2)$ acts on $C^{\infty}(\C)$ as:
\[g_2\cdot \partial_x+ g_1\cdot \partial_y=\frac{1}{2|z|}(g_1\cdot Y_1+ g_2\cdot Y_2),\]
where in the last step we used the relation \eqref{eq: definition M} defining $\mathcal{M}$.

% {\color{red}
% The key point in the proof above is that the relevant term in cohomology is the transverse part of the Poisson vector field, i.e. the part coming from the map $\tilde{a}^{-1}\circ \epsilon$. More generally, the bi-grading from Proposition \ref{proposition:PCH as forms} induces a bi-grading of multivector fields. By the discussions in the previous subsections, in particular by Theorem \ref{main theorem}, flat Poisson cohomology classes are uniquely determined by the form of there representatives in certain bi-degrees. In particular Poisson vector fields are determined by their $(0,1)$-part, Poisson $3$-vector fields by their $(2,1)$-part and Poisson $4$-vector fields are uniquely determined by their $(2,2)$-part. Hence we may focus on these parts for all computations.}

In degree $3$ we want to show that every class in $H^3(\spl,\pi)$ is uniquely associated to $(g_1,[g_2])\in C^{\infty}(\C)\oplus C^{\infty}(\C)/C^{\infty}_0(\C)$ via: 
    \[[g_1\circ f\cdot C_{\mathcal{R}}+g_2\circ f \cdot C_{\mathcal{I}}] \in H^3(\spl,\pi).\]
Note that by Proposition \ref{ses smooth formal} and the formal Poisson cohomology in Proposition \ref{formal cohomology sl2} we only need to show that any flat cohomology class is uniquely determined by a $g\in C^{\infty}_0(\C)$ via
\[[g\circ f\cdot C_{\mathcal{R}}] \in H^3_0(\spl,\pi).\]
To obtain this result we note that the cocycle $C_{\mathcal{R}}$ satisfies for $i=1,2$ that 
 \begin{align}\label{eq: max trans 3}
     i_{\dif f_i} (C_{\mathcal{R}})= \pi_i.
 \end{align}
Hence the only non-trivial parts of  $\tilde{a}(C_{\mathcal{R}})$ are in bi-degrees $(2,1)$ and $(3,0)$, see \eqref{eq: complex diag}. Moreover, using the relations:
\begin{align}\label{eq: bivector to forms}
    \tilde{\omega}_1^{\flat}(\pi_1)= -\tilde{\omega}_1 \quad \textrm{ and } \quad  \tilde{\omega}_1^{\flat}(\pi_2)= \tilde{\omega}_2,
\end{align}
which can be checked directly, we obtain: 
%for $g\in C^{\infty}_0(\C)$ the previous computations imply that
\begin{align*}
    \big(\tilde{a}(g\circ f\cdot C_{\mathcal{R}})\big)^{(2,1)}=&\, \tilde{a}(g\circ f\cdot (V_1\wedge \pi_1 +V_2\wedge \pi_2))\\
    =& \, g\circ f\cdot e_{\varphi}\big(-\tilde{\omega}_1\otimes e_1 +
    \tilde{\omega}_2\otimes e_2\big)
\end{align*}
Applying the map $\tilde{p}$ from Corollary \ref{corollary: homotopy} we note that the only non trivial part is the $(2,1)$-part (see \eqref{eq: diagram}). Hence we get using \eqref{eq: iso degree 3} that
\begin{align*}
    \tilde{p}\circ \tilde{a}(g\circ f\cdot C_{\mathcal{R}})=&\,  p_{\F}\otimes \id\big(g\circ f\cdot e_{\varphi}(-\tilde{\omega}_1\otimes e_1 +
    \tilde{\omega}_2\otimes e_2)\big)\\
    =&\, -g\circ f \cdot b_1 =\epsilon(-g).
\end{align*}
Therefore the statement holds by Theorem \ref{main theorem}.

Next we show that in degree $4$ we have an isomorphism: 
\[[X]\in H^1(\spl,\pi)\quad \leftrightarrow \quad [X\wedge C_\mathcal{R}]\in H^4(\spl,\pi).\]
From \eqref{eq: deg 1 top part} and \eqref{eq: max trans 3} we get for $(g_1,g_2)\in \mathcal{M}$ that
\[ i_{\dif f_1\wedge \dif f_2}(I(g_1,g_2)\wedge C_{\mathcal{R}})= g_2\circ f\cdot \pi_2- g_1\circ f\cdot \pi_1 \]
and therefore using \eqref{eq: bivector to forms}, Corollary \ref{corollary: homotopy} and \eqref{eq: iso degree 4} we obtain
\[ \tilde{p}\circ \tilde{a}(I(g_1,g_2)\wedge C_{\mathcal{R}})=\epsilon(g_1,g_2),\]
which implies the claim by Theorem \ref{main theorem}.

Finally, we prove the relation
\[[[X,C_{\mathcal{R}}]]=[[X,C_{\mathcal{I}}]]=0\in H^3(\spl,\pi)\]
for any $[X]\in H^1(\spl,\pi)$. For the proof we need the following lemma.
{\color{red}
\begin{lemma}\label{lemma: second differential}
The bracket $[\pi_2,\cdot]$ corresponds under $\tilde{p}\circ \tilde{a}$ to a map $\tilde{\delta}_2$ {\color{red} induced by $\tilde{a}\circ \dif_{\pi_{2}}\circ \tilde{a}^{-1}$} on the complex $p_{\F}(\CC)\otimes \wedge \R^2$, which is in degree $(0,1)\to (2,0)$ given by
\begin{align*}
    e_{\varphi}(g\circ f)\otimes e_i&\mapsto \frac{1}{2\nf}  p_{\F}(e_{\varphi}(g\circ f)\wedge \tilde{\omega}_{3-i})\otimes 1
\end{align*}
\end{lemma}
{\color{red} why is there an induced differential on $p_{\F}(\CC)\otimes \wedge \R^2$??}
\begin{proof}
We apply the discussion in Section \ref{section: Poisson cohomology in terms of foliated cohomology} and Section \ref{section: perturbation Lemma} to the Lie algebroid associated with $\pi_2$ and the splitting $\tilde{\omega}_2$. In particular, these yields isomorphism $\tilde{a}_2$ and $\tilde{b}_2$ from Proposition \ref{proposition:PCH as forms}. Lemma \ref{lemma: second differential degree one} implies that the map $\tilde{\delta}_2$ induced by $\dif_{\pi_2}$ under these identifications is on $p_{\F}(\CC)\otimes\wedge\R^2$ given by
\begin{align*}
    e_{\varphi}(g\circ f)\otimes e_i&\mapsto -\frac{1}{2\nf}  p_{\F}(e_{\varphi}(g\circ f)\wedge \tilde{\omega}_{3-i})\otimes 1
\end{align*}
To obtain the result note that for any $g\in C^{\infty}_0(\C)$ and $i=1,2$ we have
\[ \tilde{p}\circ \tilde{a}\circ \dif _{\pi_2}(g\circ f\cdot V_i)=\tilde{\delta}_2(e_{\varphi}(g\circ f)\otimes e_i). \] 
Moreover, for a flat vector field $T$ which is tangent to the foliation we obtain that
\[ \tilde{p}\circ \tilde{a} \]
This is equivalent to show that 
\begin{align*}
    \tilde{\omega}_1^{\flat}\circ \pi^{\sharp}_2 (\tilde{\omega}_i)=-\tilde{\omega}_i \qquad \text{for }i=1,2.
\end{align*}
which follows from \eqref{eq: bivector to forms} and
\begin{equation*}
    \tilde{\omega}_2^{\flat}(\pi_1)= \tilde{\omega}_1 \quad \textrm{ and } \quad  \tilde{\omega}_2^{\flat}(\pi_2)= -\tilde{\omega}_2.\qedhere
\end{equation*}
\end{proof}

To show that the first bracket is trivial in cohomology note that using \eqref{eq: deg 1 top part} and \eqref{eq: max trans 3} we obtain
\begin{align*}
    \iota_{\dif f_j}([I^1(g_1,g_2),-C_{\mathcal{R}}])=&\ -\sum_{i=1}^2\partial_ig_{3-j} \circ f\cdot \pi_i+ g_{3-i} \circ f\cdot [\pi_j,V_i]
\end{align*}
To obtain the corresponding cohomology class we look at its image in $p_{\F}(\CC^2)\wedge^1\R^2$ using $\tilde{a}$ from Proposition \ref{proposition:PCH as forms} and $\tilde{p}$ from Corollary \ref{corollary: homotopy}. We obtain for the image the expresssion
\begin{align*}
    -\sum_{i,j=1}^2(-1)^{i}\partial_ig_{3-j} \circ f\cdot e_{\varphi}(p_{\F}(\tilde{\omega}_i))\otimes e_j+g_{3-i} \circ f\cdot \tilde{\delta}_j(e_i)\otimes e_j
\end{align*}
where $\tilde{\delta}_1=\tilde{\delta}$ and $\tilde{\delta}_2$ are the maps from Lemma \ref{lemma: second differential degree one} and Lemma \ref{lemma: second differential}, respectively. Using the formulas for $\tilde{\delta}_j$ for $j=1,2$ and the identification in the proof of Lemma \ref{lemma: trivial module 3} we obtain for the sum of the second term that
\begin{align*}
    -\frac{xg_2+yg_1}{2|z|^2} \circ f\cdot b_1 -\frac{xg_1-yg_2}{2|z|^2} \circ f\cdot b_2 &\, \overset{\eqref{eq: projection m}}{=}\sum_{i=1}^2(-1)^{i+1}\frac{g_{3-i}}{2|z|}\circ f \cdot b_i 
\end{align*}
For the sum over the first term we use the identifications from the proof of Lemma \ref{lemma: trivial module 3} to obtain the expression
\begin{align*}
    \frac{1}{2\nf}\cdot\sum_{i=1}^2&\, \Big(\frac{|z|+x}{y}\Big)^{2-i} \big( y\partial_x +(|z|-x)\partial_y\big) g_{3-i}\circ f \cdot b_1 \\
    + \frac{1}{2\nf}\cdot\sum_{i=1}^2&\, (-1)^{i}\Big(\frac{|z|+x}{y}\Big)^{i-1} \big( y\partial_x +(|z|-x)\partial_y\big) g_{3-i}\circ f \cdot b_2
\end{align*}
Note that the $b_2$-term is trivial in cohomology. For the $b_1$-term we use that $(g_1,g_2)\in \mathcal{M}$ and the explicit formula for the projection $p_{\mathcal{M}}$ in \eqref{eq: projection m} to obtain
\begin{align}
    (|z|+x)\partial_x g_2 =&\ \frac{y}{|z|^2}\cdot \Big( xg_1 -yg_2  \Big) -y\partial_x g_1\label{eq: differentiate in M1}\\
    (|z|-x)\partial_y g_1 =&\, -\frac{x}{|z|^2}\cdot \Big( yg_1 +xg_2  \Big) -y\partial_y g_2\label{eq: differentiate in M2}
\end{align}
which implies that the first bracket in (????)  is zero. 

For the second bracket we first note that we have
 \begin{align*}%\label{eq: max trans 3}
     i_{\dif f_1} (C_{\mathcal{I}})= \pi_2 \quad\text{ and }\quad i_{\dif f_2} (C_{\mathcal{I}})= -\pi_1.
 \end{align*}
Therefore, we argue as for $C_{\mathcal{R}}$ to obtain
\begin{align*}
    (p_{\F}\otimes \id)\circ \tilde{a}(g\circ f \cdot C_{\mathcal{I}})=&\, g\circ f \cdot b_2
\end{align*}
for any $g\in C^{\infty}_0(\C)$.
and the following lemma.


 A similar computation yields that the second bracket is zero. 

}



% {\color{red}
% The wedge product and the Schouten-Nijenhuis bracket 
% \[ [\cdot ,\cdot]:\ \mathfrak{X}^{k}(\spl)\times \mathfrak{X}^{l}(\spl)\to \mathfrak{X}^{k+l-1}(\spl)\]
% descend to Poisson cohomology. In the following we describe these induced operations explicitly. This subsection is independent of the rest of the paper. 

% % Throughout this subsection we will use implicitly the following decomposition of smooth functions:
% % \begin{equation}\label{eq: casimir id}
% %     \begin{array}{ccc}
% %          C^{\infty}_0(\C)& \xrightarrow{\simeq}& C^{\infty}_{0,\tau}(\C)\oplus C^{\infty}_{0,\tau}(\C)\\
% %          g& = &g_1+y\cdot g_2 
% %     \end{array}
% % \end{equation}
% % depending on which expression is better suited for the situation. 
% Before we describe the algebraic structures of Poisson cohomology we take a closer look at the third Poisson cohomology group, which is next to the Casimir functions, the only degree where we have non-trivial formal and flat cohomology classes.

% \noindent\underline{\textbf{The Poisson cohomology group $H^3(\spl, \pi)$:}} We can describe cohomology classes in terms of the generators $C_{\mathcal{R}}$ and $C_{\mathcal{I}}$ by the isomorphism  
% \begin{align}\label{eq: trivial cocycle}
%     C^{\infty}(\C)\oplus &\, C^{\infty}(\C)/C^{\infty}_0(\C)\ \to \qquad H^3(\spl,\pi)\nonumber\\
%      (h_1,&\, h_2)\qquad \qquad \qquad \mapsto h_1\circ f \cdot C_{\mathcal{R}}+h_2\circ f\cdot C_{\mathcal{I}}
% \end{align}
% In particular, we have the relations
% \begin{align*}
%     \forall g\in C^{\infty}_0(\C):\quad I^3(g)= -g\circ f \cdot C_{\mathcal{R}} \quad \text{ and } \quad
%     g\circ f \cdot C_{\mathcal{I}} = 0
% \end{align*}
% \noindent\underline{\textbf{The wedge product:}} The only non-trivial part is in degrees $1\times 3\to 4$. In terms of the isomorphism in Theorem \ref{main theorem} and the description of $H^3(\spl,\pi)$, the wedge product is given by
% \begin{align}
%     \wedge:\mathcal{M}\times C^{\infty}(\C)\oplus &\, C^{\infty}(\C)/C^{\infty}_0(\C) \to \quad \mathcal{M}\nonumber\\
%     ((g_1,g_2),h_1,&\,h_2)\qquad \qquad \quad \ \mapsto h_1\cdot (g_1,g_2)\label{eq: wedge}
% \end{align}

% For the Schouten-Nijenhuis bracket we obtain the following:

% \noindent\underline{\textbf{In degree (1,1):}}
% All non-trivial Poisson vector fields are transverse to the foliation $\F$ and hence these vector fields are determined by their action on Casimir functions. {\color{red} The action is described by the two derivations
% \begin{align*}
%         Y_1:= (|z|+x)\partial_y-y\partial_x  \quad \text{ and }\quad     Y_2:= (|z|-x)\partial_x -y\partial_y
%  \end{align*}
% on the space $\C\setminus \{0\}$, which satisfy, similar to \eqref{relation:omega's}, the relation
%  \begin{align*}%\label{eq: relation y's}
%     (|z|-x)\cdot Y_1 =&\ -y\cdot Y_2
% \end{align*}
% It is straightforward to check that these two generators satisfy the relation
% \begin{align*}
%     [Y_1,Y_2]=Y_2.
% \end{align*}
% The Lie bracket in degree one is uniquely determined by the Leibniz identity and the Lie algebra isomorphism
% \begin{align}\label{eq: la isomorphism}
%     (g_1,g_2)\in \mathcal{M}\overset{I^1}{\simeq} H^1_0(\spl,\pi)\mapsto \sum_{i=1}^2 \frac{g_i}{2|z|}\cdot Y_i
% \end{align}
% }
% \noindent\underline{\textbf{In degree (1,3):}}
% In degree three we obtain for $(g_1,g_2)\in \mathcal{M}$ and the generators $C_{\mathcal{R}}$ and $C_{\mathcal{I}}$ of the formal Poisson cohomology that
% \begin{align}
%     \Big[I^1(g_1,g_2),C_{\mathcal{R}} \Big]=\Big[I^1(g_1,g_2),C_{\mathcal{I}} \Big]= 0 \ \in\ H^3_0(\spl,\pi) \label{eq: br degree 31}
%     % \Big[I^1(g_1,g_2),-C_{\mathcal{R}} \Big]=I^3\Big(\frac{1}{2|z|}\big(g_2+\frac{xg_2+yg_1}{|z|}\big)\Big)\label{eq: br degree 31}\\
%     % \Big[I^1(g_1,g_2),C_{\mathcal{I}} \Big]=&\ 0 \quad \in\ H^3_0(\spl,\pi) \label{eq: br degree 32}
%     % \Big[\sum_{i=1}^2g_i\circ f \cdot \tilde{Y}_i,C_{\mathcal{R}} \Big] =\Big[\sum_{i=1}^2g_i\circ f \cdot \tilde{Y}_i,C_{\mathcal{I}} \Big]=0 \ \in H^3_0(\spl,\pi) \label{eq: br degree 31}
%     % \Big[\sum_{i=1}^2\frac{g_i}{2|z|}\circ f \cdot \tilde{Y}_i,C_{\mathcal{R}} \Big]=&\ \frac{g_2}{|z|}\circ f \cdot C_{\mathcal{R}}\label{eq: br degree 31}\\
%     % \Big[\sum_{i=1}^2\frac{g_i}{2|z|}\circ f \cdot \tilde{Y}_i,C_{\mathcal{I}} \Big]=&\ -\frac{g_1}{|z|}\circ f \cdot C_{\mathcal{R}} \label{eq: br degree 32}
% \end{align}
% The other relations follow from the Leibniz identity and \eqref{eq: trivial cocycle}.
% % and because in cohomology we have
% % \begin{align}\label{eq: trivial cocycle}
% %     \forall g\in C^{\infty}_0(\C):\quad I^3(g)= -g\circ f \cdot C_{\mathcal{R}} \quad \text{ and } \quad
% %     g\circ f \cdot C_{\mathcal{I}} = 0
% % \end{align}

% \noindent\underline{\textbf{In degree (0,4):}}
% For $ g\in C^{\infty}(\C)$ and $(h_1,h_2)\in \mathcal{M}$ we obtain
% \begin{align*}
%     [g\circ f,I^4(h_1,h_2) ]= I^3(h_1 \partial_y g )
%     % [g\circ f,\sum_{j=1}^2 h_j\circ f\cdot W_j ]= -(h_2 \partial_x g +h_1\partial_yg)\circ f \cdot C_{\mathcal{R}} 
% \end{align*}
% % Here $W_i\in \mathfrak{X}^4(\spl\setminus S_0)$ for $i=1,2$ are the $4$-vector fields on $\spl \setminus S_0$ such that
% % \begin{align*}
% %     I^4(h_1,h_2)=[h_1\circ f\cdot W_1 +h_2\circ f\cdot W_2]\in H^4_0(\spl,\pi)
% % \end{align*}
% % to the elements 
% % \begin{align*}
% %     \tilde{b} \circ \tilde{\iota} (p_{\F}(e_{\varphi}(\tilde{\omega}_i))\otimes e_1\wedge e_2)
% % \end{align*}

% \noindent\underline{\textbf{In degree (1,4):}} The bracket is determined by \eqref{eq: wedge} - \eqref{eq: br degree 31} and the relation 
% \begin{align*}
%     [X,Y\wedge Z]= [X,Y]\wedge Z +(-1)^{|Y|(|X|-1)}Y\wedge[X,Z]
% \end{align*}
% for multivector fields $X,Y,Z\in \mathfrak{X}^{\bullet}(\spl)$.
% % with a Poisson vector field associated to $(g_1,g_2)\in \mathcal{M}$ yields 
% % \begin{align*}
% %     \Big[I^1(g_1,g_2), I^4(h_1,h_2)\Big]=&\,
% %     I^4(l_1,l_2)
% %     % \Big[\sum_{i=1}^2\frac{g_i}{2|z|}\circ f \cdot \tilde{Y}_i, \sum_{j=1}^2h_j\circ f\cdot W_j\Big]=&\,  \sum_{i,j=1}^2\Big(g_{3-i}\partial_ih_j -\partial_ig_{3-i}\cdot h_j\Big)\circ f \cdot W_j \\
% %     % &\, - \frac{g_2h_1}{|z|}\circ f \cdot W_1 +\frac{g_1h_1-g_2h_2}{2|z|}\circ f\cdot W_2
% % \end{align*}
% % where $(l_1,l_2)\in \mathcal{M}$ is given by
% % \begin{align*}
% %     l_1=&\,\sum_{i=1}^2\Big(g_{3-i}\partial_ih_1 -\partial_ig_{3-i}\cdot h_1\Big)- \frac{g_2h_1}{|z|} \\
% %     l_2=&\, \sum_{i=1}^2\Big(g_{3-i}\partial_ih_2 -\partial_ig_{3-i}\cdot h_2\Big) +\frac{g_1h_1-g_2h_2}{2|z|}
% % \end{align*}



% This gives a complete description of all non-trivial operations of \[(H^{\bullet}(\spl,\pi),\wedge, [\cdot,\cdot ]).\]

% % \subsubsection{The Lie algebra $H^1_0(\spl,\pi)$}

% % All non-trivial Poisson vector fields are transverse to the foliation $\F$ and hence these vector fields are determined by their action on Casimir functions. The action is described by the two derivations
% % \begin{align*}
% %         Y_1:= (|z|+x)\partial_y-y\partial_x  \quad \text{ and }\quad     Y_2:= (|z|-x)\partial_x -y\partial_y
% %  \end{align*}
% % on the space $\C\setminus \{0\}$, which satisfy, similar to \eqref{relation:omega's}, the relation
% %  \begin{align*}%\label{eq: relation y's}
% %     (|z|-x)\cdot Y_1 =&\ -y\cdot Y_2
% % \end{align*}
% % It is straightforward to check that these two generators satisfy the relation
% % \begin{align}\label{eq: degree one bracket}
% %     [Y_1,Y_2]=Y_2.
% % \end{align}
% % The Lie bracket in degree one is uniquely determined by the Leibniz identity and the Lie algebra isomorphism
% % \begin{align*}
% %     (g_1,g_2)\in \mathcal{M}\overset{I^1}{\simeq} H^1_0(\spl,\pi)\mapsto \sum_{i=1}^2 \frac{g_i}{2|z|}\cdot Y_i
% % \end{align*}

% \begin{proof}
% For the proof of these statements let us first note that the bi-grading from Proposition \ref{proposition:PCH as forms} induces a bi-grading of multivector fields. Flat Poisson cohomology classes are uniquely determined by the form of there representatives in certain bi-degrees by Corollary \ref{corollary: homotopy} (see also \eqref{eq: diagram}). In particular Poisson vector fields are determined by their $(0,1)$-part, Poisson $3$-vector fields by their $(1,2)$-part and Poisson $4$-vector fields are uniquely determined by their $(2,2)$-part. Hence it is for all computations enough to focus on these parts.

% To show \eqref{eq: trivial cocycle} we note that the cocycles $C_{\mathcal{R}}$ and $C_{\mathcal{I}}$ satisfy
%  \begin{align*}%\label{eq: max trans 3}
%      \dif f_1 (C_{\mathcal{R}})= \pi_1 \quad \dif f_2 (C_{\mathcal{R}})= \pi_2 \quad \dif f_1 (C_{\mathcal{I}})= \pi_2 \quad \dif f_2 (C_{\mathcal{I}})= -\pi_1
%  \end{align*}
% Hence the $(1,2)$-parts of $C_{\mathcal{R}}$ and $C_{\mathcal{I}}$ on $\spl\setminus S_0$ are given by
% \begin{align}\label{eq: Poisson formal gen}
%     % \begin{rcases}
%     C_{\mathcal{R}}=V_1\wedge \pi_1 +V_2\wedge \pi_2\quad \text{ and }\quad
%     C_{\mathcal{I}}=V_1\wedge \pi_2 -V_2\wedge \pi_1
%     % \end{rcases}
%     % \mod \underset{j=1,2}{\bigcap} \ker \iota_{\dif f_j}
% \end{align}
% Moreover, a direct calculation yields
% \begin{align}\label{eq: bivector to forms}
%     \tilde{\omega}_1^{\flat}(\pi_1)= -\tilde{\omega}_1 \quad \textrm{ and } \quad  \tilde{\omega}_1^{\flat}(\pi_2)= \tilde{\omega}_2.
% \end{align} 
% Using the isomorphism $\tilde{a}$ from Proposition \ref{proposition:PCH as forms} we obtain
% \begin{align*}
% % \begin{rcases*}
% (p_{\F}\otimes \id)\circ \tilde{a}(g\circ f \cdot C_{\mathcal{R}})=&\,  -g\circ f \cdot b_1 \\
%     (p_{\F}\otimes \id)\circ \tilde{a}(g\circ f \cdot C_{\mathcal{I}})=&\, g\circ f \cdot b_2
% % \end{rcases*}
%     % \mod (\dif +\delta)\big(\underset{i=0,1}{\bigoplus}\CC^{1+i}\otimes \wedge^{1-i}\R^2\big)
% \end{align*}
% for any $g\in C^{\infty}_0(\C)$. Hence \eqref{eq: trivial cocycle} follows from \eqref{eq: delta degree 2},\eqref{eq: iso degree 3} and Proposition \ref{formal cohomology sl2}. 

% To prove that the wedge product is given by \eqref{eq: wedge} note that for $(g_1,g_2)\in\mathcal{M}$ the $(0,1)$-part of the associated Poisson vector field is described by
%  \begin{align}\label{eq: Poisson vf}
%      g_2\circ f\cdot V_1 +g_1\circ f \cdot V_2.
%  \end{align}
% The $(2,2)$-part of a Poisson $4$-vector field representing $I^4(h_1,h_2)$ by
% \begin{align}\label{eq: Poisson 4-vf}
%     \sum_{j=1}^2(-1)^{j}h_j\circ f\cdot V_1\wedge V_2\wedge \pi_j
% \end{align}
% for $(h_1,h_2)\in \mathcal{M}$ and moreover we have that
% \begin{align*}
%     (p_{\F}\circ \id)\circ \tilde{a}\Big(\sum_{j=1}^2h_j\circ f\cdot V_1\wedge V_2\wedge \pi_{3-j}\Big)=0
% \end{align*}
% which together with \eqref{eq: Poisson formal gen} implies \eqref{eq: wedge}.

% To show \eqref{eq: la isomorphism} note that 
% %  from \eqref{eq: kernel 01} and Theorem \ref{main theorem} we obtain that every Poisson vector field is uniquely determined by its part transverse to the foliation $\F$. For $(g_1,g_2)\in\mathcal{M}$ the transverse part of the associated Poisson vector field is described by
% Poisson vector fields as in \eqref{eq: Poisson vf}
% %  \begin{align*}
% %      g_2\circ f\cdot V_1 +g_1\circ f \cdot V_2
% %  \end{align*}
% % for $(g_1,g_2)\in\mathcal{M}$ 
% are $f$-projectable: 
%  \begin{align*}
%      \dif f (g_2\circ f\cdot V_1 +g_1\circ f \cdot V_2) = \frac{1}{2|z|}\sum_{i=1}^2g_i\cdot Y_i
%  \end{align*}
% where we used the formula for the projection $p_{\mathcal{M}}$ in \eqref{eq: projection m}. Hence we obtain an isomorphism of Lie algebras.


% % For the description of the bracket in higher degrees we denote by $\tilde{Y}_i\in \mathfrak{X}^1(\spl\setminus S_0)$  for $i=1,2$ two Poisson vector fields which satisfy
% % \begin{align*}
% %     I^1(g_1,g_2)= [\sum_{i=1}^2\frac{g_i}{2|z|}\circ f\cdot \tilde{Y}_i]
% % \end{align*}
% % In particular,  $\tilde{Y}_i$ is $f$-related to $Y_i$ for $i=1,2$, i.e.
% % \begin{align}\label{eq: ytilde on cas}
% %     \tilde{Y}_i (g\circ f)=Y_i(g)\circ f \qquad \forall g\in C^{\infty}_0(\C)
% % \end{align}
% % {\color{red}
% % \begin{remark}
% % The corresponding bracket relation 
% % \begin{align*}
% %     [\tilde{Y}_1,\tilde{Y}_2]=\tilde{Y}_2
% % \end{align*}
% % associated to \eqref{eq: degree one bracket} may not be satisfied on the level of vector fields, but only on the level of cohomology.
% % \end{remark}
% % }

% % \subsubsection{The Schouten-Nijenhuis bracket in degree three}

% % In degree three we obtain for the generators $C_{\mathcal{R}}$ and $C_{\mathcal{I}}$ of the formal Poisson cohomology from Proposition \ref{formal cohomology sl2} that
% % \begin{align}
% %     \Big[I^1(g_1,g_2),C_{\mathcal{R}} \Big]=\Big[I^1(g_1,g_2),C_{\mathcal{I}} \Big]= 0 \ \in\ H^3_0(\spl,\pi) \label{eq: br degree 31}
% %     % \Big[I^1(g_1,g_2),-C_{\mathcal{R}} \Big]=I^3\Big(\frac{1}{2|z|}\big(g_2+\frac{xg_2+yg_1}{|z|}\big)\Big)\label{eq: br degree 31}\\
% %     % \Big[I^1(g_1,g_2),C_{\mathcal{I}} \Big]=&\ 0 \quad \in\ H^3_0(\spl,\pi) \label{eq: br degree 32}
% %     % \Big[\sum_{i=1}^2g_i\circ f \cdot \tilde{Y}_i,C_{\mathcal{R}} \Big] =\Big[\sum_{i=1}^2g_i\circ f \cdot \tilde{Y}_i,C_{\mathcal{I}} \Big]=0 \ \in H^3_0(\spl,\pi) \label{eq: br degree 31}
% %     % \Big[\sum_{i=1}^2\frac{g_i}{2|z|}\circ f \cdot \tilde{Y}_i,C_{\mathcal{R}} \Big]=&\ \frac{g_2}{|z|}\circ f \cdot C_{\mathcal{R}}\label{eq: br degree 31}\\
% %     % \Big[\sum_{i=1}^2\frac{g_i}{2|z|}\circ f \cdot \tilde{Y}_i,C_{\mathcal{I}} \Big]=&\ -\frac{g_1}{|z|}\circ f \cdot C_{\mathcal{R}} \label{eq: br degree 32}
% % \end{align}
% % for $(g_1,g_2)\in \mathcal{M}$. The other relations follow from the Leibniz identity and because in cohomology we have
% % \begin{align}\label{eq: trivial cocycle}
% %     \forall g\in C^{\infty}_0(\C):\quad I^3(g)= -g\circ f \cdot C_{\mathcal{R}} \quad \text{ and } \quad
% %     g\circ f \cdot C_{\mathcal{I}} = 0
% % \end{align}


% To show \eqref{eq: br degree 31} we use the following lemma.
% \begin{lemma}\label{lemma: second differential}
% The map $\tilde{\delta}_2$ induced by $\dif_{\pi_{2}}$ on the complex $p_{\F}(\CC)\otimes \wedge \R^2$ using the identification $\tilde{a}$ in degree $(0,1)\to (2,0)$ is given by
% \begin{align*}
%     e_{\varphi}(g\circ f)\otimes e_i&\mapsto \frac{1}{2\nf}  p_{\F}(e_{\varphi}(g\circ f)\wedge \tilde{\omega}_{3-i})\otimes 1
% \end{align*}
% \end{lemma}
% \begin{proof}
% We apply the discussion in Section \ref{section: Poisson cohomology in terms of foliated cohomology} and Section \ref{section: perturbation Lemma} to the Lie algebroid associated with $\pi_2$ and the splitting $\tilde{\omega}_2$. In particular, these yields isomorphism $\tilde{a}_2$ and $\tilde{b}_2$ from Proposition \ref{proposition:PCH as forms}. Lemma \ref{lemma: second differential degree one} implies that the map induced by $\dif_{\pi_2}$ and this identification is on $p_{\F}(\CC)\otimes\wedge\R^2$ given by
% \begin{align*}
%     e_{\varphi}(g\circ f)\otimes e_i&\mapsto -\frac{1}{2\nf}  p_{\F}(e_{\varphi}(g\circ f)\wedge \tilde{\omega}_{3-i})\otimes 1
% \end{align*}
% To obtain the result we need to show that the map induced by $\tilde{a}\circ \tilde{b}_2$ on the image is given by $-\id$. This is equivalent to show that 
% \begin{align*}
%     \tilde{\omega}_1^{\flat}\circ \pi^{\sharp}_2 (\tilde{\omega}_i)=-\tilde{\omega}_i \qquad \text{for }i=1,2.
% \end{align*}
% which follows from \eqref{eq: bivector to forms} and
% \begin{equation*}
%     \tilde{\omega}_2^{\flat}(\pi_1)= \tilde{\omega}_1 \quad \textrm{ and } \quad  \tilde{\omega}_2^{\flat}(\pi_2)= -\tilde{\omega}_2.\qedhere
% \end{equation*}
% \end{proof}
% % Similar to the case of Poisson vector fields we note that every Poisson cohomology class is uniquely characterized by the maximal non-trivial transverse part with respect to $\F$ of the corresponding representatives. Hence it is enough to compute the bracket of the maximal transverse parts of the representatives.
% %for a Poisson vector field of the form
% % we can use the isomorphisms $\tilde{a}$ and $\tilde{b}$ from Proposition \ref{proposition:PCH as forms} Corollary \ref{corollary:chain:proj} to do the computations on $p_{\F}(\CC)\otimes \wedge \R^2$. Under this identifications the brackets transform as
% % \begin{align*}
% %     [V_i,V_j] \in \Gamma(T\F|_{\spl\setminus S_0}) \ \leadsto \ [e_i,e_j]=0 \quad \text{ and } \quad [V_i,\pi_j ] \  \leadsto \ -\tilde{\delta}_j(e_i)
% % \end{align*}
% % where $\tilde{\delta}_1=\tilde{\delta}$ from Lemma \ref{lemma: second differential degree one}.
% % to and the Poisson cohomology classes are uniquely characterized by the maximal non-zero transverse parts of there representatives with respect to $\F$, Hence it is enough to consider the maximal transverse parts of the Poisson vector field and the Poisson $3$-vector field on $\spl \setminus S_0$. We observe that for 
% % Using that for a Poisson vector field of the form
% % \begin{align*}
% %     \sum_{i=1}^2\frac{g_i}{2|z|}\circ f \cdot \tilde{Y}_i
% % \end{align*}
% % The maximal transverse part of a representative of $I^1(g_1,g_2)$ is given by
% % \begin{align*}
% %     g_2\circ f \cdot V_1 +g_1\circ f\cdot V_2.
% % \end{align*}
% % For $C_{\mathcal{R}}$ this part on $\spl\setminus S_0$ is given by
% % \begin{align*}
% %     V_1\wedge \pi_1 +V_2\wedge \pi_2
% % \end{align*}
% Using \eqref{eq: Poisson formal gen} a direct calculation on $\spl \setminus S_0$ yields
% \begin{align*}
%     \iota_{\dif f_j}([I^1(g_1,g_2),-C_{\mathcal{R}}])=&\ -\sum_{i=1}^2\partial_ig_{3-j} \circ f\cdot \pi_i+ g_{3-i} \circ f\cdot [\pi_j,V_i]
% \end{align*}
% where we use $\partial_1 =\partial_x$ and $\partial_2=\partial_y$. To obtain the corresponding cohomology class we look at its image in $p_{\F}(\CC^2)\wedge^1\R^2$ using $\tilde{a}$ from Proposition \ref{proposition:PCH as forms} and $\tilde{p}$ from Corollary \ref{corollary: homotopy}. We obtain for the image the expresssion
% \begin{align*}
%     -\sum_{i,j=1}^2(-1)^{i}\partial_ig_{3-j} \circ f\cdot e_{\varphi}(p_{\F}(\tilde{\omega}_i))\otimes e_j+g_{3-i} \circ f\cdot \tilde{\delta}_j(e_i)\otimes e_j
% \end{align*}
% where $\tilde{\delta}_1=\tilde{\delta}$ and $\tilde{\delta}_2$ are the maps from Lemma \ref{lemma: second differential degree one} and Lemma \ref{lemma: second differential}, respectively. Using the formulas for $\tilde{\delta}_j$ for $j=1,2$ and the identification in the proof of Lemma \ref{lemma: trivial module 3} we obtain for the sum of the second term that
% \begin{align*}
%     -\frac{xg_2+yg_1}{2|z|^2} \circ f\cdot b_1 -\frac{xg_1-yg_2}{2|z|^2} \circ f\cdot b_2 &\, \overset{\eqref{eq: projection m}}{=}\sum_{i=1}^2(-1)^{i+1}\frac{g_{3-i}}{2|z|}\circ f \cdot b_i 
% \end{align*}
% For the sum over the first term we use the identifications from the proof of Lemma \ref{lemma: trivial module 3} to obtain the expression
% \begin{align*}
%     \frac{1}{2\nf}\cdot\sum_{i=1}^2&\, \Big(\frac{|z|+x}{y}\Big)^{2-i} \big( y\partial_x +(|z|-x)\partial_y\big) g_{3-i}\circ f \cdot b_1 \\
%     + \frac{1}{2\nf}\cdot\sum_{i=1}^2&\, (-1)^{i}\Big(\frac{|z|+x}{y}\Big)^{i-1} \big( y\partial_x +(|z|-x)\partial_y\big) g_{3-i}\circ f \cdot b_2
% \end{align*}
% Note that the $b_2$-term is trivial in cohomology. For the $b_1$-term we use that $(g_1,g_2)\in \mathcal{M}$ and the explicit formula for the projection $p_{\mathcal{M}}$ in \eqref{eq: projection m} to obtain
% \begin{align}
%     (|z|+x)\partial_x g_2 =&\ \frac{y}{|z|^2}\cdot \Big( xg_1 -yg_2  \Big) -y\partial_x g_1\label{eq: differentiate in M1}\\
%     (|z|-x)\partial_y g_1 =&\, -\frac{x}{|z|^2}\cdot \Big( yg_1 +xg_2  \Big) -y\partial_y g_2\label{eq: differentiate in M2}
% \end{align}
% which implies that the first bracket in \eqref{eq: br degree 31} is zero. A similar computation yields that the second bracket is zero. 

% % Similarly, by applying $\tilde{a}$ and $\tilde{p}$ to the bracket in \eqref{eq: br degree 32} we obtain
% % \begin{align*}
% %     -\sum_{i,j=1}^2\partial_ig_{3-j} \circ f\cdot e_{\varphi}(p_{\F}(\tilde{\omega}_{3-i}))\otimes e_j+(-1)^{j+1} g_{3-i} \circ f\cdot \tilde{\delta}_{3-j}(e_i)\otimes e_j
% % \end{align*}
% % The sum over the second term yields using the identifications from the proof of Lemma \ref{lemma: trivial module 3} the expression
% % \begin{align*}
% %     -\sum_{i=1}^2 \frac{g_{i}}{2|z|} \circ f\cdot b_i
% % \end{align*}
% % The sum over the first term gives
% % \begin{align*}
% %     \frac{1}{2\nf}\cdot\sum_{i=1}^2&\, \Big(\frac{|z|-x}{y}\Big)^{i-1} \big( y\partial_x -(|z|+x)\partial_y\big) g_{3-i}\circ f \cdot b_1 \\
% %     + \frac{1}{2\nf}\cdot\sum_{i=1}^2&\, (-1)^{i}\Big(\frac{|z|-x}{y}\Big)^{2-i} \big( y\partial_x -(|z|+x)\partial_y\big) g_{3-i}\circ f \cdot b_2
% % \end{align*}
% % which implies the result using
% % \begin{align*}
% %     (|z|-x)\partial_x g_1 =&\ \frac{y}{|z|^2}\cdot \Big( yg_1 +xg_2  \Big) -y\partial_x g_2\\
% %     (|z|+x)\partial_y g_2 =&\ \frac{x}{|z|^2}\cdot \Big( yg_2 -xg_1  \Big) -y\partial_y g_1
% % \end{align*}
% % the result.



% % \subsubsection{The algebraic structure in degree four}
% % For Poisson $4$-vector fields we need to describe there action on Casimir functions and the bracket with Poisson vector fields.

% % For a Casimir function $ g\in C^{\infty}(\C)$ and $(h_1,h_2)\in \mathcal{M}$ we obtain
% % \begin{align*}
% %     [g\circ f,I^4(h_1,h_2) ]= I^3(-(h_2 \partial_x g +h_1\partial_yg))
% %     % [g\circ f,\sum_{j=1}^2 h_j\circ f\cdot W_j ]= -(h_2 \partial_x g +h_1\partial_yg)\circ f \cdot C_{\mathcal{R}} 
% % \end{align*}
% % % Here $W_i\in \mathfrak{X}^4(\spl\setminus S_0)$ for $i=1,2$ are the $4$-vector fields on $\spl \setminus S_0$ such that
% % % \begin{align*}
% % %     I^4(h_1,h_2)=[h_1\circ f\cdot W_1 +h_2\circ f\cdot W_2]\in H^4_0(\spl,\pi)
% % % \end{align*}
% % % to the elements 
% % % \begin{align*}
% % %     \tilde{b} \circ \tilde{\iota} (p_{\F}(e_{\varphi}(\tilde{\omega}_i))\otimes e_1\wedge e_2)
% % % \end{align*}
% % The bracket with a Poisson vector field associated to $(g_1,g_2)\in \mathcal{M}$ yields 
% % \begin{align*}
% %     \Big[I^1(g_1,g_2), I^4(h_1,h_2)\Big]=&\,
% %     I^4(l_1,l_2)
% %     % \Big[\sum_{i=1}^2\frac{g_i}{2|z|}\circ f \cdot \tilde{Y}_i, \sum_{j=1}^2h_j\circ f\cdot W_j\Big]=&\,  \sum_{i,j=1}^2\Big(g_{3-i}\partial_ih_j -\partial_ig_{3-i}\cdot h_j\Big)\circ f \cdot W_j \\
% %     % &\, - \frac{g_2h_1}{|z|}\circ f \cdot W_1 +\frac{g_1h_1-g_2h_2}{2|z|}\circ f\cdot W_2
% % \end{align*}
% % where $(l_1,l_2)\in \mathcal{M}$ is given by
% % \begin{align*}
% %     l_1=&\,\sum_{i=1}^2\Big(g_{3-i}\partial_ih_1 -\partial_ig_{3-i}\cdot h_1\Big)- \frac{g_2h_1}{|z|} \\
% %     l_2=&\, \sum_{i=1}^2\Big(g_{3-i}\partial_ih_2 -\partial_ig_{3-i}\cdot h_2\Big) +\frac{g_1h_1-g_2h_2}{2|z|}
% % \end{align*}

% % Moreover, the wedge product induces a map in cohomology. The only non-trivial part is in the degrees $1\times 3\to 4$. In terms of the isomorphism in Theorem \ref{main theorem} the product is given by
% % \begin{align*}
% %     \wedge:\mathcal{M}\times C^{\infty}_0(\C)\to \mathcal{M},\qquad ((g_1,g_2),h)\mapsto h\cdot (g_1,g_2)
% % \end{align*}

% % The maximal non-trivial transverse part of a Poisson $4$-vector field representing $I^4(h_1,h_2)$ is given by
% % \begin{align*}
% %     \sum_{j=1}^2(-1)^{j+1}h_j\circ f\cdot V_1\wedge V_2\wedge \pi_j
% % \end{align*}
% % To compute the brackets we proceed similarly as before, by taking only the maximal non-trivial transverse parts into account. 
% Finally, for the bracket of a Casimir function and a Poisson $4$-vector field we obtain using \eqref{eq: Poisson 4-vf} that
% \begin{align*}
%     \iota_{\dif f_i}([g\circ f, I^4(h_1,h_2) ])= \sum_{j=1}^2 (-1)^{i+j}(h_j\partial_{3-i}g)\circ f\cdot \pi_j.
%     % \iota_{\dif f_i}([g\circ f, \sum_{j=1}^2 h_i\circ f\cdot W_j ])= \sum_{j=1}^2 (-1)^{i+j-1}(h_j\partial_{3-i}g)\circ f\cdot \pi_j.
% \end{align*}
% Using $\tilde{a}$ and $\tilde{p}$ from Proposition \ref{proposition:PCH as forms} and Corollary \ref{corollary: homotopy}, respectively, together with the identifications from Lemma \ref{lemma: trivial module 3} we obtain the result, i.e.
% \begin{align*}
%     \tilde{p}\circ \tilde{a}([g\circ f, I^4(h_1,h_2) ])=&\, \sum_{i=1}^2 (h_i\partial_{2}g)\circ f\cdot b_i 
%     % \\
%     % &\, +\sum_{i=1}^2 (-1)^{i}(h_i\partial_{i}g)\circ f\cdot b_2 
%     \qedhere
% \end{align*}

% % For the bracket with Poisson vector fields we first compute that
% % \begin{align*}
% %     \iota_{\varphi}\Big(\Big[I^1(g_1,g_2), I^4(h_1,h_2)\Big]\Big)
% %     =&\, \sum_{i,j=1}^2(-1)^{j+1}(g_{3-i}h_j)\circ f\cdot [\pi_j,V_i]\\
% %     &\, +\sum_{i,j=1}^2(-1)^j(g_{3-i}\partial_ih_j-h_j\partial_ig_{3-i})\circ f\cdot \pi_j
% %     % \iota_{\varphi}\Big(\Big[\sum_{i=1}^2&\,\frac{g_i}{2|z|}\circ f \cdot \tilde{Y}_i, \sum_{j=1}^2h_j\circ f\cdot W_j\Big]\Big)\\
% %     % =&\, \sum_{i,j=1}^2(-1)^j\Big((g_{3-i}\partial_ih_j-h_j\partial_ig_{3-i})\circ f\cdot \pi_j-(g_{3-i}h_j)\circ f\cdot [\pi_j,V_i]\Big)
% % \end{align*}
% % Using $\tilde{a}$ from Proposition \ref{proposition:PCH as forms} and $\tilde{p}$ from Corollary \ref{corollary: homotopy} we get
% % \begin{align*}
% %     \tilde{p}\circ\tilde{a}\Big(\Big[I^1(g_1,g_2), I^4(h_1,h_2)\Big]\Big)= \sum_{i,j=1}^2(-1)^{j+1}(g_{3-i}h_j)&\,\circ f\cdot \tilde{\delta}_j(e_i)\otimes e_1\wedge e_2\\
% %     +\sum_{i,j=1}^2(g_{3-i}\partial_ih_j-h_j\partial_ig_{3-i})\circ f\cdot &\,p_{\F}(e_{\varphi}(\tilde{\omega}_j))\otimes e_1\wedge e_2
% % \end{align*}
% % By Lemma \ref{lemma: second differential degree one} and Lemma \ref{lemma: second differential} the first sum is given by
% % \begin{align*}
% %     \Big(\frac{g_{2}h_1-g_{1}h_2}{2|z|}\circ f \cdot p_{\F}(e_{\varphi}(\tilde{\omega}_1))-\frac{g_{1}h_1+g_{2}h_2}{2|z|}\circ f \cdot p_{\F}(e_{\varphi}(\tilde{\omega}_2))\Big)\otimes e_1\wedge e_2
% % \end{align*}
% % which yields, using the projection $p_{\mathcal{M}}$ from Proposition \ref{proposition: twisted module} and the induced relations for $(g_1,g_2)\in \mathcal{M}$ together with the identification \eqref{eq: iso degree 4}, the element
% % \begin{align*}
% %     -\frac{ h_2}{2|z|}\cdot(g_1,g_2 )\in \mathcal{M}
% % \end{align*}
% % Similarly, by using $p_{\mathcal{M}}$, \eqref{eq: differentiate in M1} and \eqref{eq: differentiate in M2} for $(h_1,h_2)\in \mathcal{M}$ together with the identification \eqref{eq: iso degree 4}, the second sum yields 
% % \begin{align*}
% %     \sum_{i=1}^2g_{3-i}\partial_i(h_1,h_2)& -\partial_ig_{3-i}\cdot (h_1,h_2) \\
% %     +\frac{1}{2|z|^3}\Big((|z|-x)g_2&\,(yh_2-xh_1)+xg_1(yh_1+xh_2), (yg_2-xg_1)(yh_2-xh_1)\Big)
% % \end{align*}
% % Using the relations from $p_{\mathcal{M}}$ once more for $g$ and $h$ respectively, implies that the last term is equal to
% % \begin{align*}
% %     \frac{1}{2|z|}(g_1h_2-2g_2h_1,g_1h_1)
% % \end{align*}
% % which proves the statement.

% % Finally, the result for the wedge product follows immediately by wedging the maximal non-trivial transverse parts of the corresponding representatives.
% \end{proof}}



















% Hence the result follows immediately from \eqref{eq: transverse degree 1}, \eqref{eq: derivation Casimir} and Lemma \ref{lemma:eigenspaces} making use of the relations induced by \eqref{eq: relation y's}:


% From Theorem \ref{main theorem} we know that Poisson cohomology in degree one is uniquely described by elements in $\mathcal{M}$. To obtain explicit representatives of these cohomology classes we follow the map $\iota_{\spl}$, in particular we use \eqref{eq: kernel 01} and Proposition \ref{proposition:PCH as forms}, to obtain for $(g_1,g_2)\in \mathcal{M}$ the Poisson vector fields:
% \begin{align*}
%     \sum_{i=1}^2g_i\circ f\cdot V_{3-i} +\tilde{b}^{1,1}\circ (h_{\F}\otimes 1)\circ \delta ( \sum_{i=1}^2g_i\circ f\cdot e_{3-i})
% \end{align*}
% We note that all these vector fields are transverse to the foliation $\F$ away from $S_0$. Using the projection $f$ to the leaf space $\C$, these vector fields correspond by \eqref{eq:v transversality} uniquely to the vector fields:
% \begin{align*}
%     g_1\cdot \partial_y +g_2\cdot \partial_x
% \end{align*}
% We write the bracket in terms of the left-hand side of the isomorphisms in Theorem \ref{main theorem}.
% The pairs for $(k,l)$ for which the induced map is not trivial are as follows
% \begin{itemize}
%     \item for $(k,l)=(1,0):$
%     \begin{align*}
%         [(g_1,g_2),h_1+yh_2]= &\ \begin{array}{c}
%              g_1Y_1(h_1)+(|z|+x)\big(g_2Y_1(h_2)-g_2h_2\big)\\
%              +y\cdot\Big(g_1Y_1(h_2)-g_1h_2+\frac{g_2Y_1(h_1)}{|z|-x}\Big) 
%         \end{array}
%     \end{align*} 
%     where 
%     $Y_1$ is defined by
%     \begin{align*}
%         Y_1:=&\ (|z|-x)\partial_x -y\partial_y
%     \end{align*}
%     \item for $(k,l)=(1,1):$
%     \begin{align*}
%         [(g_1, 0),(h_1,h_2)]=&\ \begin{pmatrix}
%         g_1Y_1(h_1) -h_1Y_1(g_1) \\
%         g_1Y_1(h_2) -h_2Y_1(g_1)+g_1h_2
%         \end{pmatrix}^t\\
%         [(0, g_2),(h_1,h_2)]=&\ \begin{pmatrix}
%         \frac{|z|+x}{|z|-x}(g_2Y_1(h_2)-h_2Y_1(g_2))\\
%         -h_1Y_1(g_2) +g_2Y_1(h_1)-h_1g_2
%         \end{pmatrix}^t
%     \end{align*}
% \end{itemize}

% \begin{proof}
%  For the proof we recall that non-trivial flat Poisson cohomology classes are uniquely characterized by the maximally transverse part of one of its representatives by Proposition \ref{proposition: Poisson homotopy}. In degree zero that is trivial, in degree $1$ we have for $g_1,g_2\in C^{\infty}_{0,\tau}(\C)$ that
%  \begin{align}\label{eq: transverse degree 1}
%      I^1(g_1,g_2) = g_1 \cdot \tilde{Y_1}+g_2\cdot \tilde{Y}_2 
%  \end{align}
%  where $\tilde{Y}_1, \tilde{Y}_2 \in \mathfrak{X}^1(\spl\setminus S_0)$ are given by
%  \begin{align*}
%      \tilde{Y}_1:= &\  (|z|-x)\circ f\cdot V_1 - y\circ f\cdot V_2 \mod \mathfrak{X}^1_{1}(\spl\setminus S_0)\\
%      \tilde{Y}_2:= &\ y \circ f\cdot V_1 -(|z|+x)\circ f\cdot V_2 \mod \mathfrak{X}^1_{1}(\spl\setminus S_0)
%  \end{align*}
%  Note that we have the relations
% \begin{align}\label{eq: relation ytildes}
%     \frac{|z|+x}{y}\circ f\cdot \tilde{Y}_1 =&\ \tilde{Y}_2 \qquad  \tilde{Y}_1 = \frac{|z|-x}{y}\circ f\cdot \tilde{Y}_2
% \end{align}
% Note that for the Schouten-Nijenhuis bracket we have for $g\in C^{\infty}_0(\C)$ the relations
%  \begin{align}\label{eq: derivation Casimir}
%      V_1 (g\circ f)= \partial_xg \circ f \quad \text{ and } \quad V_2 (g\circ f)= \partial_yg \circ f 
%  \end{align}
%  Moreover, we have that
%  \begin{align}\label{eq: transverse bracket}
%      \dif f_j ([V_1,V_2])=0 \quad \text{ and }\dif f_j (T)=0
%  \end{align}
%  for any foliated multivector field $T\in \mathfrak{X}^p_p(\spl)$. Hence we may conclude that the induced Schouten-Nijenhuis bracket in cohomology is determined by the bracket of the maximally transverse parts of the representatives as just listed and their projection to $E$. In the following we denote by 
%  \[[I^i(g),I^j(h)] \] 
%  simply the bracket between the maximally transverse parts of the representatives of the corresponding cohomology classes as described in \eqref{eq: transverse degree 1}, \eqref{eq: transverse degree 3} and \eqref{eq: transverse degree 4}, or a flat Casimir function if $j=0$. 
 
%  For the different pairs $(k,l)$ we now obtain:\\
%  \noindent{\underline{For $(k,l)=(1,0)$}:} We define $Y_2$ by
%  \begin{align*}
%      Y_2:= y\partial_x-(|z|+x)\partial_y
%  \end{align*}
% and we note that we have for $g\in C^{\infty}_0(\C)$ the relation
% \begin{align}\label{eq: ytilde on cas}
%     \tilde{Y}_i (g\circ f)=Y_i(g)\circ f
% \end{align}
%  Hence the result follows immediately from \eqref{eq: transverse degree 1}, \eqref{eq: derivation Casimir} and Lemma \ref{lemma:eigenspaces} making use of the relations induced by \eqref{eq: relation y's}:
%  \begin{align}\label{eq: relation y's}
%     (|z|+x)\cdot Y_1 =&\ y\cdot Y_2 \qquad  y\cdot Y_1 = (|z|-x)\cdot Y_2
% \end{align}
% \noindent{\underline{For $(k,l)=(1,1)$}:} We first note that we have the relations
% \begin{equation}\label{eq: derivatives leaf space}
%     \begin{array}{rclcrcl}
%          \partial_x(|z|+x)&=&\frac{|z|+x}{|z|}&\qquad & \partial_y(|z|+x)&=&\frac{y}{|z|} \\
%          \partial_x(|z|-x)&=& \frac{x-|z|}{|z|}&\qquad &  \partial_y(|z|-x)&=&\frac{y}{|z|} 
%     \end{array}
% \end{equation}
% which implies by \eqref{eq: ytilde on cas} that
% \begin{align*}
%     [\tilde{Y}_1,\tilde{Y}_2]= \tilde{Y}_2 \mod \mathfrak{X}^1_1(\spl \setminus S_0)
% \end{align*}
% As a consequence we obtain using \eqref{eq: transverse degree 1} and \eqref{eq: derivation Casimir} that
% \begin{align*}
%   [I^1(g_1,g_2),I^1(h_1,h_2)]&\, =  \\
%   \big(g_1Y_1(h_1) -h_1Y_1(g_1)& +\frac{|z|+x}{y}(g_2Y_2(h_2)-h_2Y_2(g_2))\big)\circ f \cdot \tilde{Y}_1\\
%   \big(g_1Y_1(h_2) -h_1Y_1(g_2)& +\frac{|z|-x}{y}(g_2Y_2(h_1)-h_2Y_2(g_1))+g_1h_2-h_1g_2\big)\circ f \cdot \tilde{Y}_2
% \end{align*}
% modulo elements in $\mathfrak{X}^1_{1,0}(\spl)$. Hence the results follow from \eqref{eq: relation y's}.
% \end{proof}

% \subsubsection{$H^3(\spl,\pi)$: a closer look}
% As degree three is, besides degree zero, the only degree where the formal and flat Poisson cohomology groups are non-trivial, we want to analyse in this subsection how the generators $C_{\mathcal{R}}$ and $C_{\mathcal{I}}$ defined in Proposition \ref{formal cohomology sl2} behave in flat cohomology.
% \begin{corollary}
% We obtain in cohomology the relation
% \begin{align*}
%     [l\circ f \cdot C_{\mathcal{R}} +m\circ f\cdot C_{\mathcal{I}}] = I^3(\frac{y\cdot l-x\cdot m}{|z|})
% \end{align*}
% where $l,m\in C^{\infty}_0(\C)$. In particular, we have
% \begin{align*}
%     [l\circ f \cdot \big(f_1\cdot C_{\mathcal{R}} +f_2\cdot C_{\mathcal{I}}\big)]=0
% \end{align*}
% In particular, every element in $H^3_0(\spl,\pi)$ has a unique representative of the form  
% $g\circ f\cdot C$, with $g\in C^{\infty}_0(\C)$, where
% \[C:=f_2C_{\mathcal{R}}-f_1C_{\mathcal{I}}\in \mathfrak{X}^3(\spl).\]
% \end{corollary}
% To proof this statement we first note that non-trivial flat Poisson cohomology classes are uniquely characterized by the maximally transverse part of one of its representatives obtained by Proposition \ref{proposition: Poisson homotopy}. We will use this fact throughout this computational section. In degree $3$ we note that
%  \begin{align}\label{eq: projection cohomology}
%      g\circ f\cdot e_{\varphi}(p_{\F}(\tilde{\omega}_i)) = g\circ f\cdot e_{\varphi}(\tilde{\omega}_i+(\dif \circ h_{\F})(\tilde{\omega}_i))
%  \end{align}
% for any $g\in C^{\infty}_0(\C)$. Moreover, a direct calculation shows that
% \begin{align}\label{eq: bivector to forms}
%     \tilde{\omega}_1^{\flat}(\pi_1)= -\tilde{\omega}_1\ \ \ \ \ \textrm{ and } \ \ \ \ \    \tilde{\omega}_1^{\flat}(\pi_2)= \tilde{\omega}_2
% \end{align} 
% Hence we obtain for degree $3$ that
% \begin{align}\label{eq: transverse degree 3}
%     I^3(g)= g\circ f\cdot (V_1\wedge \pi_2 +V_2\wedge \pi_1) \mod \mathfrak{X}^{3}_{3,0}(\spl)
%     % + \dif_{\pi}\mathfrak{X}^2_{0.0}(\spl)
% \end{align}
%  for $g\in C^{\infty}_0(\C)$ which provides a unique representative for every flat Poisson cohomology class in degree three. 
%  \begin{proof}
%  For the cocycles $C_{\mathcal{R}}$ and $C_{\mathcal{I}}$ we have
%  \begin{align*}
%      \dif f_1 (C_{\mathcal{R}})= \pi_1 \quad \dif f_2 (C_{\mathcal{R}})= \pi_2 \quad \dif f_1 (C_{\mathcal{I}})= \pi_2 \quad \dif f_2 (C_{\mathcal{I}})= -\pi_1
%  \end{align*}
%  Hence we obtain using \eqref{eq: tilde a}, \eqref{eq: projection cohomology}, \eqref{eq: bivector to forms} and \eqref{relation:omega's} that
%  \begin{align*}
%      p_{\F}(\tilde{a}^{2,1}(l\circ f \cdot C_{\mathcal{R}} +m\circ f\cdot C_{\mathcal{I}}))= k 
%  \end{align*}
% where $l,m\in C^{\infty}_0(\C)$ and $k\in p_{\F}(\CC^2)\otimes \R^2 $ a general element as in \eqref{eq: general element} with
% \begin{align*}
%     k_1 = -l_1 -(|z|-x)m_2\quad k_2 =&\ m_1 +(|z|+x)l_2\\
%     k_3 = \ m_1 -(|z|-x)l_2\quad k_4 =&\ l_1 +(|z|+x)m_2
% \end{align*}
% By \eqref{eq: trivialization in (2,1)} and \eqref{eq: trivial bundle} we obtain
% \begin{align*}
%     p_{\F}(\tilde{a}^{2,1}(l\circ f \cdot C_{\mathcal{R}} +m\circ f\cdot C_{\mathcal{I}}))= g\circ f \cdot e_{\varphi}(b_1)+h\circ f\cdot e_{\varphi}(b_2)
% \end{align*}
% where $g,h\in C^{\infty}_0(\C)$ are given by
% \begin{align*}
%     g= -\frac{x\cdot l +y\cdot m}{|z|} \qquad h= \frac{y\cdot l-x\cdot m}{|z|}
% \end{align*}
% which proves the statement by \eqref{eq: iso degree 3}.
% \end{proof}




% \subsubsection{The module structure}
% Every flat Poisson cohomology group is a module over the zeroth cohomology group, i.e.\ the Casimir functions with standard multiplication.

% In the following we use for Casimir functions the description in terms of $C^{\infty}(\C)$ as given in Proposition \ref{prop:Casimirs}. In general, we describe the module structures as operations on the left handsides of the identifications in Theorem \ref{main theorem}. For the following let $k\in C^{\infty}$ be a Casimir function. 

% \noindent{\underline{In degree $0$}:} For $g\in C^{\infty}_0(\C)$ the ring structure is given by standard multiplication of functions.\\
% \noindent{\underline{In degree $1$}:} For $(g_1,g_2)\in C^{\infty}_{0,\tau}(\C)\oplus C^{\infty}_{0,\tau}(\C)$ the module multiplication is given by
% \begin{align*}
%     k_1+y\cdot k_2\odot_1 (g_1,g_2):= (k_1g_1+(|z|+x)k_2g_2 ,k_1g_2+(|z|-x) k_2g_1)
% \end{align*}
% which follows from the identification in \eqref{eq: kernel 01}.\\
% \noindent{\underline{In degree $3$}:} The module multiplication is given by the standard multiplications of functions by \eqref{eq: iso degree 3}.\\
% \noindent{\underline{In degree $4$}:} Here the module structure is for $(g_1,h_1)\in C^{\infty}_{0,\tau}(\C)\oplus C^{\infty}_{0,\tau}(\C)$ given by
% \begin{align*}
%     k_1+y\cdot k_2\odot_4 (g_1,g_2):=(k_1g_1-(|z|-x)k_2g_2 ,k_1g_2-(|z|+x) k_2g_1)
% \end{align*}
% \begin{align*}
%     k_1+y\cdot k_2\odot_4 (g_2,-g_1):=(k_1g_2+(|z|-x)k_2g_1 ,-(k_1g_1+(|z|+x) k_2g_2))
% \end{align*}
% which follows from \eqref{eq: iso degree 4} and \eqref{relation:omega's}.




% \subsubsection{The ring structure}
% To describe the ring structure for the flat Poisson cohomology, we present the multiplication using the isomorphisms from Theorem \ref{main theorem}. 

% The only non-trivial map is in degree $1\times 3 \to 4$, which is the map
% \begin{equation*}
%     \begin{array}{cccc}
%          \wedge :& C^{\infty}_{0,\tau}(\C)\oplus C^{\infty}_{0,\tau}(\C) \times  C^{\infty}_{0}(\C)&\to &C^{\infty}_{0,\tau}(\C)\oplus C^{\infty}_{0,\tau}(\C)
%     \end{array}
% \end{equation*}
% which is given by
% \begin{equation*}
%     \begin{array}{rcl}
%          (g_1,g_2)\wedge h&\mapsto& 2\cdot \big(-y^2h_2g_2 -(|z|-x)h_1g_1,y^2h_2g_1 +(|z|+x)h_1g_2\big)
%     \end{array}
% \end{equation*}
% We obtain this result by the following observation: the wedge product induces on the complex $\CC\otimes\wedge\R^2$ the map
% \begin{equation*}
%     \begin{array}{cccc}
%          \tilde{\wedge}:& \CC^{p}\otimes \wedge^q\R^2 \times \CC^{p'}\otimes \wedge^{q'}\R^2& \to &\CC^{p+p'}\otimes \wedge^{q+q'}\R^2\\
%          & (\alpha\otimes v ,\beta\otimes w)&\mapsto & (-1)^{p'q} e_{\varphi}((i_{V}\alpha)\wedge(i_V\beta))\otimes v\wedge w
%     \end{array}
% \end{equation*}
% This map descends to the HE data $E$ as defined in Proposition \ref{proposition: homotopy}. The identifications of $E$ with the flat Poisson cohomology groups (see Theorem \ref{main theorem}) imply that $\tilde{\wedge}$ on $E$ can be identified with the wedge product in cohomology. Hence the identifications of $E$ with the left-hand side in Theorem \ref{main theorem} as given in \eqref{eq: kernel 01}, \eqref{eq: iso degree 3} and \eqref{eq: iso degree 4} imply the statement.




% \subsubsection{The Lie bracket in cohomology}
% The Schouten-Nijenhuis bracket descends to a map in cohomology:
% \[ [\cdot ,\cdot]: H^{k}(\spl,\pi)\times H^{l}(\spl,\pi)\to H^{k+l-1}(\spl,\pi)\]
% We write the bracket in terms of the left-hand side of the isomorphisms in Theorem \ref{main theorem}.
% The pairs for $(k,l)$ for which the induced map is not trivial are as follows
% \begin{itemize}
%     \item for $(k,l)=(1,0):$
%     \begin{align*}
%         [(g_1,g_2),h_1+yh_2]= &\ \begin{array}{c}
%              g_1Y_1(h_1)+(|z|+x)\big(g_2Y_1(h_2)-g_2h_2\big)\\
%              +y\cdot\Big(g_1Y_1(h_2)-g_1h_2+\frac{g_2Y_1(h_1)}{|z|-x}\Big) 
%         \end{array}
%     \end{align*} 
%     where 
%     $Y_1$ is defined by
%     \begin{align*}
%         Y_1:=&\ (|z|-x)\partial_x -y\partial_y
%     \end{align*}
%     \item for $(k,l)=(4,0):$
%     \begin{align*}
%         [(g_1,g_2),h_1+yh_2] =&\ k_1+yk_2
%     \end{align*}
%     where 
%     \begin{align*}
%         k_1=&\ \frac{1}{2|z|}\big( -g_1X_1(h_1) +(|z|-x)g_2(Y_1(h_2)-h_2)\big)\\
%         k_2=&\ \frac{1}{2|z|}\big(\frac{g_2}{|z|+x} X_1(h_1) -g_1(X_1(h_2)-h_2)\big)\\
%     \end{align*}
%     and $X_1$ is defined by
%     \begin{align*}
%         X_1:=(|z|+x)\partial_x -y\partial_y
%     \end{align*}
%     \item for $(k,l)=(1,1):$
%     \begin{align*}
%         [(g_1, 0),(h_1,h_2)]=&\ \begin{pmatrix}
%         g_1Y_1(h_1) -h_1Y_1(g_1) \\
%         g_1Y_1(h_2) -h_2Y_1(g_1)+g_1h_2
%         \end{pmatrix}^t\\
%         [(0, g_2),(h_1,h_2)]=&\ \begin{pmatrix}
%         \frac{|z|+x}{|z|-x}(g_2Y_1(h_2)-h_2Y_1(g_2))\\
%         -h_1Y_1(g_2) +g_2Y_1(h_1)-h_1g_2
%         \end{pmatrix}^t
%     \end{align*}
%     \item for $(k,l)=(3,1):$
%     \begin{align*}
%         [(g_1, g_2),(h_1,0)]=&\ k_1+yk_2
%     \end{align*}
%     where $k_1,k_2\in C^{\infty}_{0,\tau}(\C)$ are given by
%     \begin{align*}
%         k_1=&\ -h_1Y_1(g_1)-\frac{xg_1}{|z|}Y_4(h_1)-\frac{|z|(|z|-x)+2x^2}{2|z|^2}g_1h_1 \\
%         k_2=&\ -h_1Y_1(g_2)-\frac{xg_2}{|z|}Y_4(h_1)+\frac{|z|(|z|+x)-2x^2}{2|z|^2}g_2h_1
%     \end{align*}
%     and $Y_4$ is defined by
%     \begin{align*}
%         Y_4:= (|z|-x)\partial_x+y\partial_y.
%     \end{align*}
%     For the other generators we obtain
%     \begin{align*}
%         [(g_1, g_2),(0,h_2)]=&\ k_1+yk_2
%     \end{align*}
%     where $k_1,k_2\in C^{\infty}_{0,\tau}(\C)$ are given by
%     \begin{align*}
%         k_1=&\ -(|z|+x)\Big(h_2Y_1(g_2)+\frac{x}{|z|}g_2Y_4(h_2)-\frac{|z|(|z|-x)+2x^2}{2|z|^2}g_2h_2\Big) \\
%         k_2=&\ -\frac{|z|+x}{y^2}\Big(h_2Y_1(g_1)+\frac{x}{|z|}g_1Y_4(h_2)\Big)-\frac{|z|+2x}{2|z|^2}g_1h_2
%     \end{align*}
%     \item for $(k,l)=(4,1):$
%     \begin{align*}
%         [(g_1, g_2),(h_1,0)]=&\ (k_1,k_2)
%     \end{align*}
%     where
%     \begin{align*}
%         k_i=&\ g_iY_1(h_1)-h_1Y_1(g_i) -\Big(2-\frac{x}{|z|}\Big)g_ih_1
%     \end{align*}
%     for $i=1,2$ and 
%     \begin{align*}
%           [(g_1, g_2),(0,h_2)]=&\ (k_1,k_2)
%     \end{align*}
%     where
%     \begin{align*}
%         k_1=&\ h_2Y_1(g_2)-g_2Y_1(h_2) +\Big(1-\frac{x}{|z|}\Big) g_2h_2\\
%         k_2=&\ \frac{|z|+x}{|z|-x}\Big(h_2Y_1(g_1)-g_1Y_1(h_2)+\big(1-\frac{x}{|z|}\big)g_1h_2\Big)
%     \end{align*}
% \end{itemize}

% \begin{proof}
%  For the proof we recall that non-trivial flat Poisson cohomology classes are uniquely characterized by the maximally transverse part of one of its representatives by Proposition \ref{proposition: Poisson homotopy}. In degree zero that is trivial, in degree $1$ we have for $g_1,g_2\in C^{\infty}_{0,\tau}(\C)$ that
%  \begin{align}\label{eq: transverse degree 1}
%      I^1(g_1,g_2) = g_1 \cdot \tilde{Y_1}+g_2\cdot \tilde{Y}_2 
%  \end{align}
%  where $\tilde{Y}_1, \tilde{Y}_2 \in \mathfrak{X}^1(\spl\setminus S_0)$ are given by
%  \begin{align*}
%      \tilde{Y}_1:= &\  (|z|-x)\circ f\cdot V_1 - y\circ f\cdot V_2 \mod \mathfrak{X}^1_{1}(\spl\setminus S_0)\\
%      \tilde{Y}_2:= &\ y \circ f\cdot V_1 -(|z|+x)\circ f\cdot V_2 \mod \mathfrak{X}^1_{1}(\spl\setminus S_0)
%  \end{align*}
%  Note that we have the relations
% \begin{align}\label{eq: relation ytildes}
%     \frac{|z|+x}{y}\circ f\cdot \tilde{Y}_1 =&\ \tilde{Y}_2 \qquad  \tilde{Y}_1 = \frac{|z|-x}{y}\circ f\cdot \tilde{Y}_2
% \end{align}
% For degree $3$ we have \eqref{eq: transverse degree 3} and for degree $4$ we use \eqref{eq: projection cohomology} and \eqref{eq: bivector to forms} to obtain
%  \begin{align}\label{eq: transverse degree 4}
%      I^4(g_1,g_2)= \begin{rcases}
%      -g_1\circ f\cdot V_1\wedge V_2\wedge  \pi_1 \\
%      +g_2\circ f\cdot V_1\wedge V_2 \wedge \pi_2 \end{rcases} \mod \mathfrak{X}^{4}_{3,0}(\spl)
%  \end{align}
%  for $g_1,g_2\in C^{\infty}_{0,\tau}(\C)$. Note that for the Schouten-Nijenhuis bracket we have for $g\in C^{\infty}_0(\C)$ the relations
%  \begin{align}\label{eq: derivation Casimir}
%      V_1 (g\circ f)= \partial_xg \circ f \quad \text{ and } \quad V_2 (g\circ f)= \partial_yg \circ f 
%  \end{align}
%  Moreover, we have that
%  \begin{align}\label{eq: transverse bracket}
%      \dif f_j ([V_1,V_2])=0 \quad \text{ and }\dif f_j (T)=0
%  \end{align}
%  for any foliated multivector field $T\in \mathfrak{X}^p_p(\spl)$. Hence we may conclude that the induced Schouten-Nijenhuis bracket in cohomology is determined by the bracket of the maximally transverse parts of the representatives as just listed and their projection to $E$. In the following we denote by 
%  \[[I^i(g),I^j(h)] \] 
%  simply the bracket between the maximally transverse parts of the representatives of the corresponding cohomology classes as described in \eqref{eq: transverse degree 1}, \eqref{eq: transverse degree 3} and \eqref{eq: transverse degree 4}, or a flat Casimir function if $j=0$. 
 
%  For the different pairs $(k,l)$ we now obtain:\\
%  \noindent{\underline{For $(k,l)=(1,0)$}:} We define $Y_2$ by
%  \begin{align*}
%      Y_2:= y\partial_x-(|z|+x)\partial_y
%  \end{align*}
% and we note that we have for $g\in C^{\infty}_0(\C)$ the relation
% \begin{align}\label{eq: ytilde on cas}
%     \tilde{Y}_i (g\circ f)=Y_i(g)\circ f
% \end{align}
%  Hence the result follows immediately from \eqref{eq: transverse degree 1}, \eqref{eq: derivation Casimir} and Lemma \ref{lemma:eigenspaces} making use of the relations induced by \eqref{eq: relation y's}:
%  \begin{align}\label{eq: relation y's}
%     (|z|+x)\cdot Y_1 =&\ y\cdot Y_2 \qquad  y\cdot Y_1 = (|z|-x)\cdot Y_2
% \end{align}
%  \noindent{\underline{For $(k,l)=(4,0)$}:} By a direct calculation we obtain
%  \begin{align*}
%      [I^4(g_1,g_2),I^0(h)]=&\ \partial_x(h_1+yh_2) \circ f \cdot V_2\wedge(-g_1\circ f \cdot \pi_1 +g_2\circ f\cdot \pi_2)\\
%      &\ +\partial_y (h_1 +yh_2)\circ f \cdot V_1\wedge(g_1\circ f \cdot \pi_1 -g_2\circ f\cdot \pi_2)
%  \end{align*}
%  modulo elements in $\mathfrak{X}^3_3(\spl)$. Using the map $\tilde{a}^{2,1}$ we obtain
%  \begin{align*}
%      \tilde{a}^{2,1}([I^4(g_1,g_2),I^0(h)])=&\ \partial_x(h_1+yh_2)\circ f\cdot \sum_i g_i\circ f\cdot  e_{\varphi}(\tilde{\omega}_i)\otimes e_2 \\
%      &\ -\partial_y(h_1+yh_2)\circ f\cdot \sum_i g_i\circ f\cdot  e_{\varphi}(\tilde{\omega}_i)\otimes e_1
%  \end{align*}
%  In terms of cohomology we have by \eqref{relation:omega's} and \eqref{eq: projection cohomology} that
%  \begin{align*}
%      p_{\F}(\tilde{a}^{2,1}([& I^4(g_1,g_2), I^0(h)]))\\ 
%      =&\ (g_1\partial_xh_1-(|z|-x)g_2\partial_xh_2)\circ f\cdot e_{\varphi}(p_{\F}(\tilde{\omega}_1))\otimes e_2 \\
%      &\ +(g_2\partial_xh_1-(|z|+x)g_1\partial_xh_2)\circ f\cdot e_{\varphi}(p_{\F}(\tilde{\omega}_2))\otimes e_2 \\
%      &\ -(g_1(1+y\partial_y)h_2-(|z|-x)g_2\frac{\partial_yh_1}{y})\circ f\cdot e_{\varphi}(p_{\F}(\tilde{\omega}_1))\otimes e_1\\
%      &\ -(g_2(1+y\partial_y)h_2-(|z|+x)g_1\frac{\partial_yh_1}{y})\circ f\cdot e_{\varphi}(p_{\F}(\tilde{\omega}_2))\otimes e_1
%  \end{align*}
% Using \eqref{eq: trivial bundle} and the definition of $p_E$ in Proposition \ref{proposition: homotopy} we obtain that 
% \begin{align*}
%     p_{E}(\tilde{a}^{2,1}([I^4(g_1,g_2),&\, I^0(h)]))= k\circ f \cdot e_{\varphi}(b_2)
% \end{align*}
% where $k=k_1+yk_2\in C^{\infty}_0(\C)$ is given by
% \begin{align*}
%     k_1:=&\ \frac{1}{2|z|}\big( -g_1((|z|+x)\partial_x -y\partial_y)h_1 +(|z|-x)g_2(Y_1(h_2)-h_2)\big)\\
%     k_2:=&\ \frac{1}{2|z|}\big( \frac{|z|-x}{y^2}g_2((|z|+x)\partial_x-y\partial_y)h_1 -g_1((|z|+x)\partial_x -(1+y\partial_y))h_2\big)
% \end{align*}
% \noindent{\underline{For $(k,l)=(1,1)$}:} We first note that we have the relations
% \begin{equation}\label{eq: derivatives leaf space}
%     \begin{array}{rclcrcl}
%          \partial_x(|z|+x)&=&\frac{|z|+x}{|z|}&\qquad & \partial_y(|z|+x)&=&\frac{y}{|z|} \\
%          \partial_x(|z|-x)&=& \frac{x-|z|}{|z|}&\qquad &  \partial_y(|z|-x)&=&\frac{y}{|z|} 
%     \end{array}
% \end{equation}
% which implies by \eqref{eq: ytilde on cas} that
% \begin{align*}
%     [\tilde{Y}_1,\tilde{Y}_2]= \tilde{Y}_2 \mod \mathfrak{X}^1_1(\spl \setminus S_0)
% \end{align*}
% As a consequence we obtain using \eqref{eq: transverse degree 1} and \eqref{eq: derivation Casimir} that
% \begin{align*}
%   [I^1(g_1,g_2),I^1(h_1,h_2)]&\, =  \\
%   \big(g_1Y_1(h_1) -h_1Y_1(g_1)& +\frac{|z|+x}{y}(g_2Y_2(h_2)-h_2Y_2(g_2))\big)\circ f \cdot \tilde{Y}_1\\
%   \big(g_1Y_1(h_2) -h_1Y_1(g_2)& +\frac{|z|-x}{y}(g_2Y_2(h_1)-h_2Y_2(g_1))+g_1h_2-h_1g_2\big)\circ f \cdot \tilde{Y}_2
% \end{align*}
% modulo elements in $\mathfrak{X}^1_{1,0}(\spl)$. Hence the results follow from \eqref{eq: relation y's}.\\
% \noindent{\underline{For $(k,l)=(3,1)$}:} Using \eqref{eq: transverse degree 1} and \eqref{eq: transverse degree 3} we first focus on the bracket of the ``generator''
% of the third flat Poisson cohomology group where we obtain
% \begin{align*}
%     [V_1\wedge \pi_2+V_2\wedge \pi_1, \tilde{Y}_1 ] =&\ - \frac{\nf-f_1}{\nf}\cdot V_1\wedge \pi_2+\frac{f_2}{\nf}\cdot V_1\wedge \pi_1 - V_2\wedge \pi_1
% \end{align*}
% modulo $\mathfrak{X}^3_{3}(\spl\setminus S_0)$. Hence by \eqref{eq: tilde a}, \eqref{eq: bivector to forms}, \eqref{eq: projection cohomology} and \eqref{relation:omega's} we have that
% \begin{align*}
%     p_{\F}(\tilde{a}^{2,1}([V_1\wedge \pi_2&+V_2\wedge \pi_1, \tilde{Y}_1 ])) =\\
%     &\frac{2x}{|z|}\circ f\cdot e_{\varphi}(p_{\F}(\tilde{\omega}_2))\otimes e_1+ e_{\varphi}(p_{\F}(\tilde{\omega}_1))\otimes e_2
%     \end{align*}
% Using \eqref{eq: trivial bundle} we obtain
% \begin{align*}
%     p_{E}(\tilde{a}^{2,1}([V_1\wedge \pi_2&+V_2\wedge \pi_1, \tilde{Y}_1 ])= -\frac{|z|(|z|-x)+2x^2}{2|z|^2}\circ f \cdot e_{\varphi}(b_2)
% \end{align*}
% Similarly we compute
% \begin{align*}
%     [V_1\wedge \pi_2+V_2\wedge \pi_1, h_1\circ f ]\wedge \tilde{Y_1} =&\ \big( (|z|-x) \partial_xh_1 \big) \circ f\cdot V_1\wedge \pi_2\\
%     &\ -\big(y\partial_xh_1\big) \circ f \cdot V_2\wedge \pi_2\\
%     &\ +\big((|z|-x)\partial_yh_1 \big) \circ f \cdot V_1\wedge \pi_1\\
%     &\ -\big( y\partial_yh_1\big) \circ f\cdot V_2\wedge \pi_1
% \end{align*}
% modulo elements in $\mathfrak{X}^3_{3,0}(\spl)$. Hence we get further 
% \begin{align*}
%     p_{\F}(&\tilde{a}^{2,1}([V_1\wedge \pi_2+V_2\wedge \pi_1, h_1\circ f ]\wedge \tilde{Y_1}))\\
%     =&\ \big( (|z|-x) \partial_xh_1 +y\partial_yh_1\big) \circ f \cdot e_{\varphi}(p_{\F}(\tilde{\omega}_2))\otimes e_1\\
%     &\ +\big((|z|-x)\partial_xh_1+y\partial_yh_1\big) \circ f \cdot e_{\varphi}(p_{\F}(\tilde{\omega}_1))\otimes e_2
% \end{align*}
% which finally gives
% \begin{align*}
%     p_{E}(\tilde{a}^{2,1}([V_1\wedge \pi_2&+V_2\wedge \pi_1, h_1\circ f ]\wedge \tilde{Y_1})=-\frac{x}{|z|}((|z|-x)\partial_x+y\partial_y)h_1 
% \end{align*}
% The results follow from these calculations using the properties of the bracket together with \eqref{eq: relation ytildes}.
% \noindent{\underline{For $(k,l)=(4,1)$}:} We calculate using \eqref{eq: transverse degree 1} and \eqref{eq: transverse degree 4} that
% \begin{align*}
%     [I^4(g_1,g_2),&\, I^1(h_1,0)]= [\sum_i (-1)^i g_i \circ f \cdot V_1\wedge V_2\wedge \pi_i ,h_1\circ f\cdot\tilde{Y}_1]\\
%     =&\ \sum_i (-1)^i\big((|z|-x)(g_i\partial_xh_1-h_1\partial_xg_i -\frac{g_ih_1}{|z|})\big)\circ f \cdot V_1\wedge V_2\wedge \pi_i\\
%     &\ +\sum_i(-1)^i\big(-g_i(1+y\partial_y)h_1+yh_1\partial_yg_i)\big)\circ f \cdot V_1\wedge V_2\wedge \pi_i
% \end{align*}
% modulo elements in $\mathfrak{X}^4_{3,0}(\spl)$ and hence we obtain
% \begin{align*}
%     p_{\F}(\tilde{a}^{2,2}&([I^4(g_1,g_2), I^1(h_1,0)]))\\
%     =&\ \sum_i \big((|z|-x)(g_i\partial_xh_1-h_1\partial_xg_i -\frac{g_ih_1}{|z|})\big)\circ f \cdot e_{\varphi}(p_{\F}(\tilde{\omega}_i))\otimes e_1\wedge e_2\\
%     &\ +\sum_i\big(-g_i(1+y\partial_y)h_1+yh_1\partial_yg_i)\big)\circ f \cdot e_{\varphi}(p_{\F}(\tilde{\omega}_i))\otimes e_1\wedge e_2
% \end{align*}
% which yields the result. To last part follows from \eqref{eq: relation y's} and the fact that in cohomology we have 
% \begin{align*}
%     f_2 \cdot I^4(g_1,0) = I^4(0,-(|z|+x)g_1)
% \end{align*}
% by \eqref{relation:omega's}, \eqref{eq: tilde a} and \eqref{eq: bivector to forms}.
% \end{proof}


==> Setting_sl2c.tex <==


\section{The Poisson cohomology of $\mathfrak{sl}_2(\C)$}\label{section: main result}

In Subsection \ref{section: linear Poisson} we recall the interpretation of Poisson cohomology of a linear Poisson structure in terms of Lie algebra cohomology. We will see that for a semisimple Lie algebra $\g$ the Poisson cohomology of its associated linear Poisson structure can be described by its flat and formal Poisson cohomology. In Subsection \ref{section: setting} we fix some notation for the Lie algebra $\spl$, and then describe the symplectic foliation and the algebra of Casimirs. In Subsection \ref{section: formal poisson} we compute the formal Poisson cohomology groups of the linear Poisson structure associated with the real Lie algebra $\spl$. Finally, in Subsection \ref{section: PC statement}, we give the description of the Poisson cohomology groups of $\spl$, which will be proven in the following three sections. 


 

% \section{The formal Poisson cohomology of $\mathfrak{sl}_2(\C)$}\label{section: main result}
% In this section we compute the formal Poisson cohomology of the linear Poisson structure associated with the real Lie algebra $\spl$. In Subsection \ref{section: linear Poisson} we recall the interpretation of Poisson cohomology of a linear Poisson structure in terms of Lie algebra cohomology. 
% We will see that for a semisimple Lie algebra $\g$ the Poisson cohomology of its associated linear Poisson structure can be described by its flat and formal Poisson cohomology (Proposition \ref{ses smooth formal}). In Subsection \ref{section: setting} we fix some notation for the Lie algebra $\spl$, and then describe the symplectic foliation and the algebra of Casimirs. Finally in Subsection \ref{section: formal poisson} we compute the formal Poisson cohomology groups.

\subsection{Poisson cohomology of linear Poisson structures}\label{section: linear Poisson}

A Poisson structure on a vector space is called linear if the set of linear functions is closed under the Poisson bracket. Such Poisson structures are in one-to-one correspondence with Lie algebra structures on the dual vector space via \eqref{eq: linear Poisson}. Explicitly, for a Lie algebra $(\g,[\cdot,\cdot])$, the Poisson structure $\pi$ on $\mathfrak{g}^*$ is determined by the condition that the map $l:\mathfrak{g}\to C^{\infty}(\mathfrak{g}^*)$, which identifies $\g$ with $(\mathfrak{g}^*)^*$, %the linear function $l_X(\psi):=\psi(X)$, 
is a Lie algebra homomorphism:
\[\{l_X,l_Y\}_{\pi}=l_{[X,Y]},\]%\ \ \ \forall \ X,Y\in\mathfrak{g},\]
where $\{\cdot,\cdot\}_{\pi}$ is the Poisson bracket on $C^{\infty}(\mathfrak{g}^*)$ corresponding to $\pi$. In particular, $C^{\infty}(\mathfrak{g}^*)$ becomes a $\mathfrak{g}$-representation, with $X\cdot h:=\{l_X,h\}$. Moreover, the Poisson complex of $(\mathfrak{g}^*,\pi)$ is isomorphic to the Chevalley-Eilenberg complex of $\g$ with coefficients in $C^{\infty}(\mathfrak{g}^*)$ \cite[Prop 7.14]{Laurent2013}
\begin{equation}\label{iso_complexes}
(\mathfrak{X}^{\bullet}(\mathfrak{g}^*),\dif_{\pi})\simeq (\wedge^{\bullet}\mathfrak{g}^*\otimes C^{\infty}(\mathfrak{g}^*),\dif_{EC}).
\end{equation}
This identification allows for the use of techniques from Lie theory in the calculation of Poisson cohomology. 

Under the isomorphism \eqref{iso_complexes}, the subcomplex of multivector fields on $\mathfrak{g}^*$ that are flat at $0$ corresponds to the Eilenberg-Chevalley complex of $\mathfrak{g}$ with coefficients in the subrepresentation $C_0^{\infty}(\mathfrak{g}^*)\subset C^{\infty}(\mathfrak{g}^*)$ consisting of smooth functions that are flat at zero:
\begin{align}\label{eq: multivector fields identification}
    \mathfrak{X}^{\bullet}_0(\mathfrak{g}^*)\simeq \wedge^{\bullet}\mathfrak{g}^*\otimes C^{\infty}_0(\mathfrak{g}^*).
\end{align}
We call the cohomology of this complex the \textbf{flat Poisson cohomology} and denote it by $H^{\bullet}_0(\mathfrak{g}^*,\pi)$.
The quotient complex is naturally identified with 
\[(\wedge^{\bullet} \mathfrak{g}^*\otimes \R[[\mathfrak{g}]],\dif_{EC}),\]
where $\R[[\mathfrak{g}]]:=C^{\infty}(\mathfrak{g}^*)/C^{\infty}_0(\mathfrak{g}^*)$ is the ring of formal power series of functions on $\mathfrak{g}^*$. The resulting cohomology will be called the \textbf{formal Poisson cohomology at} $0\in \mathfrak{g}^*$ denoted by $H^{\bullet}_{F}(\mathfrak{g}^* ,\pi )$. By the above, this is isomorphic to the cohomology of $\mathfrak{g}$ with coefficients in $\R[[\mathfrak{g}]]$, i.e\ 
\[H^{\bullet}_{F}(\mathfrak{g}^*,\pi)\simeq H^{\bullet}(\mathfrak{g},\R[[\mathfrak{g}]]).\]
% As a representation, $\R[[\mathfrak{g}]]$ is isomorphic to the product of the symmetric powers of the adjoint representation: 
%   \[\R[[\mathfrak{g}]]\simeq \prod_{k\geq 0} S^k(\mathfrak{g}).\]
% As shown in \cite{MZ} the following two propositions hold: 
Moreover, the short exact sequence
 \begin{align*}
  0\to C^{\infty}_0(\mathfrak{g}^*)\to C^{\infty}(\mathfrak{g}^*)\stackrel{j^{\infty}_0}{\longrightarrow} \R[[\g]]\to 0,
 \end{align*}
 induces a long exact sequence in cohomology: 
\begin{equation}\label{jet}
\ldots \stackrel{j^{\infty}_0}{\to} H^{\bullet-1}_{F}(\mathfrak{g}^*,\pi)\stackrel{\partial}{\to} 
H^{\bullet}_{0}(\mathfrak{g}^*,\pi)\to H^{\bullet}(\mathfrak{g}^*,\pi)\stackrel{j^{\infty}_0}{\to}H^{\bullet}_{F}(\mathfrak{g}^*,\pi )\stackrel{\partial}{\to}\ldots
 \end{equation}

If the Lie algebra $\g$ is semisimple, we can say more:
\begin{proposition}\cite[Corollary 4.5]{MZ}\label{ses smooth formal}
For a semisimple Lie algebra $\g$, the Poisson cohomology of $(\mathfrak{g}^*,\pi)$ fits into the short exact sequence 
\[0\to H^{\bullet}_0(\mathfrak{g}^*,\pi)\to H^{\bullet}(\mathfrak{g}^*,\pi)\stackrel{j^{\infty}_0}{\to} H^{\bullet}_F(\mathfrak{g}^*,\pi)\to 0.\]
\end{proposition}

Elements in the $0$-th Poisson cohomology are called \emph{Casimir functions} 
\[\Cas(\mathfrak{g}^*,\pi):=H^0(\mathfrak{g}^*,\pi).\]
These are the same as functions on $\mathfrak{g}^*$ that are invariant under the coadjoint action. The flat and the formal Casimir functions will be denoted:
\[\Cas_0(\mathfrak{g}^*,\pi) \quad \textrm{and}\quad \Cas_F(\mathfrak{g}^*,\pi).\]

The formal Poisson cohomology of semisimple Lie algebras is well-known:   
\begin{proposition}\label{formal cohomology}
\cite[Proposition 4.2 \& 4.3]{MZ} Let $(\mathfrak{g}^*,\pi)$ be the linear Poisson structure associated to a semisimple Lie algebra $\mathfrak{g}$.
\begin{enumerate}
    \item There exist $n=\dim \mathfrak{g} - \max \mathrm{rank}(\pi)$ algebraically independent homogeneous polynomials $f_1 ,\dots , f_n$ such that
    \begin{align*}
        \Cas_F(\mathfrak{g}^*,\pi)=\R[[f_1 ,\dots ,f_n ]] \subset \R[[\mathfrak{g}]].
    \end{align*}
    Here $\R[[f_1,\dots ,f_n]]$ denotes formal power series in the polynomials $f_j$.
    \item For the formal Poisson cohomology of $\g$ at $0$ we have that: 
    \begin{align*}
        H^{\bullet}_{F}(\mathfrak{g}^*,\pi)&\simeq H^{\bullet}(\g)\otimes \Cas _{F}(\mathfrak{g}^*,\pi).
    \end{align*}
\end{enumerate}
\end{proposition}

In the next subsections we will use these results for $\spl$.


\subsection{The foliation and the Casimirs}\label{section: setting}
In this subsection we describe the linear Poisson structure associated with the real Lie algebra $\spl$ in terms of its complex counterpart, and we discuss its symplectic foliation and the algebra of Casimir functions. 

 
% {\color{blue}
% For this we first identify  $\mathfrak{sl}_2(\C)^*$ with $\spl$ using $4$ times the Killing form. With respect to a a specific choice of a $\C$-basis $\{z_j\}_{j=1}^3 $ on $\spl$ the identification takes the form
%  \begin{equation}\label{eq: identification}
%      \begin{array}{ccc}
%      \mathfrak{sl}_2^*(\C)&\simeq &\mathfrak{sl}_2(\C)\\
%      (z_1,z_2,z_3)&\mapsto&A:=
%      \begin{pmatrix}
%      z_2 &z_1-z_3 \\
%      z_1+z_3&-z_2
%      \end{pmatrix}
%      \end{array}
%  \end{equation}
% \begin{remark}
% The identification \eqref{eq: identification} allows us to view the linear Poisson structure as a Poisson structure on $\spl$ rather then $\mathfrak{sl}_2(\C)^*$. Therefore we speak from here on from the linear Poisson structure on $\spl$.
% \end{remark}
% }


We consider the following complex coordinates on $\spl$:
% \begin{equation}\label{eq: identification}
%      \C^3\simeq \mathfrak{sl}_2(\C)\quad
%      (z_1,z_2,z_3)\mapsto A:=
%      \begin{pmatrix}
%      z_2 &z_1-z_3 \\
%      z_1+z_3&-z_2
%      \end{pmatrix}
%  \end{equation}
\begin{equation}\label{eq: identification}
     \C^3\simeq \mathfrak{sl}_2(\C)\quad
     (z_1,z_2,z_3)\mapsto A:=
     \begin{pmatrix}
     iz_1 &-z_2+iz_3 \\
     z_2+iz_3&-iz_1
     \end{pmatrix}
 \end{equation}
Throughout the paper we identify $\spl\simeq \spl^*$ via the trace form:
\[\spl\diffto \spl^*, \quad A\mapsto \big(B\mapsto \mathrm{tr}(A\cdot B)\big).\]
We use this identification to regard the linear Poisson structure associated with the \emph{complex} Lie algebra $\spl$ as a complex Poisson structure on $\spl$. In the coordinates from above, this becomes: 
% \begin{align}\label{eq:complex basis}
%   \pi_{\C} &:=z_1\partial _{z_2} \wedge \partial _{z_3} +z_2 \partial_{z_3} \wedge \partial_{z_1} -z_3\partial_{z_1}\wedge \partial_{z_2}
%  \end{align}
\begin{align}\label{eq:complex basis}
  \pi_{\C} &:=z_1\partial_{z_2} \wedge \partial_{z_3} +z_2 \partial_{z_3} \wedge \partial_{z_1} +z_3\partial_{z_1}\wedge \partial_{z_2}
 \end{align}
The real and the imaginary part of $\pi_{\C}$ yield two Poisson structures 
 \begin{align}\label{eq: real identification}
      \pi=\pi_{1}:=4\cdot \Re (\pi_{\C}), \ \ \ \ \pi_{2} =4\cdot \Im(\pi_{\C})
\end{align}
The constant $4$ ensures that the linear Poisson structure associated with the \emph{real} Lie algebra $\spl$ is:
\[(\spl,\pi).\]

We denote the corresponding \emph{singular symplectic foliation} by:
\[(\mathcal{F},\omega_{1}).\]
From general properties of complex Poisson structures (see \cite{LGStXu}), it follows that the leaves of $\mathcal{\F}$ coincide with the adjoint orbits on $\mathfrak{sl}_2(\C)$, and agree also with the leaves of $\pi_2$ and of $\pi_{\C}$. The leaves can be described using the level sets of the basic, complex-valued Casimir function:
% \begin{align}\label{eq:casimir}
%  &f=f_1+f_2\, i :\spl\to \C,\nonumber \\
%  &f(A):= -\det (A)=z_1^2+z_2^2-z_3^2.
% \end{align}
% \begin{align}\label{eq:casimir}
%  &f=f_1+f_2\, i :\spl\to \C,\nonumber \\
%  &f(A):= -\det (A)=-(z_1^2+z_2^2+z_3^2).
% \end{align}
\begin{align}\label{eq:casimir}
 &f=f_1+ i\, f_2 :\spl\to \C,\nonumber \\
 &f(A):= \det (A)=z_1^2+z_2^2+z_3^2.
\end{align}
More precisely, the leaves are the following families of submanifolds:
 \[S_{z}:=f^{-1}(z), \ \ z\in \C \setminus\{ 0\},\]
and the singular cone $S_0:=f^{-1}(0)$ decomposes into two leaves:
\[\{0\} \ \ \ \ \ \textrm{ and }\ \ \ \ \  S^{\text{reg}}_{0}:=f^{-1}(0)\setminus \{0\}. \]

The map $f$ generates all Casimir functions on $\spl$:

\begin{proposition}\label{prop:Casimirs}
The algebra of Casimir functions of $(\spl,\pi)$ is isomorphic to the algebra of smooth functions on $\C$, via the map: 
\begin{equation*}
f^*:C^{\infty}(\C)\diffto \Cas(\mathfrak{sl}_2(\C),\pi),\quad g\mapsto g\circ f.
\end{equation*}
\end{proposition}
\begin{proof}
Clearly, the assignment is well-defined and injective. Surjectivity follows because $f$ restricts to a surjective submersion on the open dense set $\mathfrak{sl}_2(\C)\setminus \{0\}$, whose fibers are precisely the leaves. 
\end{proof}

\begin{remark}
The \textbf{leaf-space} of $\F$, denoted $\spl/\mathcal{F}$, is obtained by identifying points in $\spl$ that belong to the same leaf. The \textbf{regular leaf-space} $(\spl\backslash\{0\})/\mathcal{F}$ has a smooth structure such that the quotient map is a submersion. In fact, $f|_{\mathfrak{sl}_2(\C)\setminus \{0\}}$ descends to a diffeomorphism: 
\[ (\spl\backslash\{0\})/\mathcal{F}\simeq \C.\] 
Therefore, Proposition \ref{prop:Casimirs} implies that the restriction map
\[\Cas(\mathfrak{sl}_2(\C),\pi)\to C^{\infty}\big((\spl\backslash\{0\})/\F\big)\]
is an isomorphism from the algebra of Casimirs to the algebra of smooth functions on the regular leaf-space.
 \end{remark}
 
 
% Denote the singular cone by
%  \[Z:=\{f=0\}\subset \mathfrak{sl}_2(\C)^*.\]


 
 
 
 \subsection{Formal Poisson cohomology of $\mathfrak{sl}_2(\C)$}\label{section: formal poisson}

We compute the formal Poisson cohomology of $(\mathfrak{sl}_2(\C),\pi)$. For this, we introduce the real coordinates $\{x_j,y_j\}_{j=1}^3$ on 
$\mathfrak{sl}_2(\C)$:
 \[ z_j:= x_j+i\cdot y_{j}, \quad \text{ for } j\in \{1,2,3\}.\]
% In this section we compute the formal Poisson cohomology for $(\mathfrak{sl}_2(\C),\pi)$ in Proposition \ref{formal cohomology sl2}. As we are interested in the real structure we introduce on $\mathfrak{sl}_2(\C)$ the coordinates $\{x_j\}_{j=1}^6$ given by
%  \[ z_j:= x_j+i\cdot x_{j+3} \ \ \ \text{ for } j\in \{1,2,3\}.\]
%  To simplify notation we write for the standard vector fields
% \[ \partial_i:=\partial_{x_i}\]
% and similarly for the standard multivector fields and forms
% \[ \partial_{i_1 \dots i_n}:=\wedge_{j=1}^{n}\partial_{x_{i_j}}\ \ \ \ \ \dif x_{i_1 \dots i_n}:=\wedge_{j=1}^n \dif x_{i_j}\]
By Proposition \ref{formal cohomology}, the invariant polynomials on $\mathfrak{sl}_2(\C)$ are generated by the functions $f_{1}$ and $f_{2}$ from $f=f_1+i\cdot f_2$ in \eqref{eq:casimir}. Therefore, in order to determine the formal Poisson cohomology of $(\mathfrak{sl}_2(\C),\pi)$, we need to calculate the Lie algebra cohomology of $\spl$. We obtain the following result.

\begin{proposition}\label{formal cohomology sl2} 
The formal Poisson cohomology groups of $(\mathfrak{sl}_2(\C),\pi)$ at the origin are given by
\[H^k_F(\mathfrak{sl}_2(\C),\pi)=
\begin{cases}
\R[[f_1,f_2]]& \text{ if }k=0\\
\R[[f_1,f_2]]\cdot C_{\mathcal{R}} \oplus \R[[f_1,f_2]]\cdot C_{\mathcal{I}}& \text{ if } k=3\\
\R[[f_1,f_2]]\cdot C_{\mathcal{R}}\wedge C_{\mathcal{I}}& \text{ if } k=6\\
%\R[[f_1,f_2]]\cdot\partial_{x_1}\partial_{x_2}\partial_{x_3}\partial_{y_1}\partial_{y_2}\partial_{y_3}& \text{ if } k=6\\
0& \text{ else}
\end{cases}\]
where $C_{\mathcal{R}}$ and $C_{\mathcal{I}}$ are $\frac{4}{3}$ of the real and imaginary part of the Cartan three-form, respectively. Explicitly:
\begin{align*}
    C_{\mathcal{R}}=&\ \frac{1}{2}( \partial_{x_1}\partial_{x_2}\partial_{x_3}-\partial_{y_1}\partial_{y_2}\partial_{x_3}-\partial_{x_1}\partial_{y_2}\partial_{y_3}-\partial_{y_1}\partial_{x_2}\partial_{y_3})\\
    C_{\mathcal{I}}=&\ \frac{1}{2} ( \partial_{y_1}\partial_{y_2}\partial_{y_3}-\partial_{y_1}\partial_{x_2}\partial_{x_3}-\partial_{x_1}\partial_{y_2}\partial_{x_3}-\partial_{x_1}\partial_{x_2}\partial_{y_3})
\end{align*}
 \end{proposition}
 \begin{proof}
 By Propositions \ref{formal cohomology} we have 
\[H^{\bullet}_F(\mathfrak{sl}_2(\C),\pi)= H^{\bullet}(\spl)\otimes \R[[f_1,f_2]].\]
From standard Lie theory we know that $H^{\bullet}(\mathfrak{sl}_2(\C))$ is isomorphic to a free exterior algebra with two generators in degree three (see \cite{Chev50} or also \cite[Corollary 3.7]{Sol02}). 
%  Note that as a vector space we have
% \[ \spl =\su \oplus \ i\cdot \su = \langle x_1,x_2,x_3\rangle \oplus \langle y_1,y_2,y_3\rangle\]
% where $\langle\cdot \rangle$ denotes the $\R$-span. Using that $(\wedge^{\bullet}\su)^{\su}$ is generated by the element $x_1\wedge x_2 \wedge x_3$ 
The complex-valued Cartan three-form is given by
\begin{align*}
    3\, \partial_{z_1}\partial_{z_2}\partial_{z_3}
\end{align*}
Hence taking $\frac{4}{3}$ of the real and imaginary part yields $C_{\mathcal{R}}$ and $C_{\mathcal{I}}$, respectively. Note that $C_{\mathcal{R}},C_{\mathcal{I}}\in(\wedge^{3}\spl)^{\spl}$ and from \cite[Theorem 19.1]{Chev1948} we know that every element in $H^{\bullet}(\spl)$ has a unique $\spl$-invariant representative. 
% in $(\wedge^{\bullet}\spl)^{\spl}$.
% Both are non-trivial in cohomology which can be seen from
% \begin{align*}
%     C_{\mathcal{R}}\wedge C_{\mathcal{I}}=4\cdot \partial_{x_1}\partial_{x_2}\partial_{x_3}\partial_{y_1}\partial_{y_2}\partial_{y_3}
% \end{align*}
As a result we obtain for the Lie algebra cohomology $H^{\bullet}(\spl)$:
\begin{align*}
         H^0(\spl) &=\R,\\ 
         H^{3}(\spl)&=\R\cdot 
         C_{\mathcal{R}} \oplus \R\cdot C_{\mathcal{I}}, \\
         H^{6}(\spl)&=\R\cdot C_{\mathcal{R}}\wedge C_{\mathcal{I}}
\end{align*}
and $H^{k}(\spl)=0$ in all other degrees.
\end{proof}

\subsection{Poisson cohomology of $\spl$}\label{section: PC statement}

Recall that Poisson cohomology is a module over the space of Casimir functions, which, for $\spl$, is isomorphic to $C^{\infty}(\C)$ (see Proposition \ref{prop:Casimirs}). We will describe the Poisson cohomology groups as modules over this algebra, and we will also describe the induced Schouten Nijenhuis bracket.

The following two vector fields on $\C\setminus \{0\}$ will play an important role:
\begin{align*}
        Y_1:=-y\partial_x+ (|z|+x)\partial_y  \quad \text{ and }\quad     Y_2:= (|z|-x)\partial_x -y\partial_y,
\end{align*}
where we used the coordinate $z=x+i\cdot y$ on $\C$. 
These satisfy, the relations
 \begin{align*}%\label{eq: relation y's}
    [Y_1,Y_2]=Y_2 \qquad \textrm{and} \qquad 
    (|z|-x)\cdot Y_1 = -y\cdot Y_2.
\end{align*}

The mild singularities of these vector fields imply that, when multiplied with flat functions, they became smooth, flat vector fields on $\C$. Motivated by the theorem below, we denote the resulting $C^{\infty}(\C)$-module by:
\begin{equation}\label{eq:flat:module:of:vector:fields}
\out:=\{g_1Y_1+g_2Y_2\, |\, g_1,g_2\in C^{\infty}_0(\C)\} \subset \mathfrak{X}^1_0(\C).
\end{equation}
The bracket relation above shows that $\out$ is a Lie subalgebra of the algebra of flat vector fields. The second relation above shows that we have an isomorphism of $C^{\infty}(\C)$-modules: 
\[
\out\simeq 
\frac{C_0^{\infty}(\C)\oplus C^{\infty}_0(\C)}{\big\{(g_1,g_2)\ |\  yg_1=(|z|-x) g_2\big\}}.
\]
This module will appear more frequently in the paper (see Subsection \ref{subsection: twisted module}).

We are ready now to describe the Poisson cohomology.

\begin{theorem}\label{theorem: PC} The Poisson cohomology groups of $(\spl,\pi)$ are
\begin{itemize}
    \item $H^0(\spl,\pi)\simeq C^{\infty}(\C)$, via the isomorphism:
    \[g\circ f\in H^0(\spl,\pi) \qquad \leftrightarrow \qquad   g\in C^{\infty}(\C);\]
    \item 
$H^1(\spl,\pi)\simeq \out$, as $C^{\infty}(\C)$-modules and as Lie algebras, via the natural action of $H^1(\spl,\pi)$ on Casi\-mirs; i.e.,
\[[X]\in H^1(\spl,\pi)   \qquad \leftrightarrow \qquad Y\in \out\]
if and only if, for all $g\in C^{\infty}(\C)$:
\[\Lie_X(g\circ f)=\Lie_Y(g)\circ f;\]
\item $H^2(\spl,\pi)=0$;
    \item 
$H^3(\spl,\pi)\simeq 
C^{\infty}(\C)\oplus C^{\infty}(\C)/C^{\infty}_0(\C)
$ as $C^{\infty}(\C)$-modules, where to $(g_1,[g_2])\in C^{\infty}(\C)\oplus C^{\infty}(\C)/C^{\infty}_0(\C)$ we associate: 
    \[[g_1\circ f\cdot C_{\mathcal{R}}+g_2\circ f \cdot C_{\mathcal{I}}] \in H^3(\spl,\pi);\]
\item $H^4(\spl,\pi)\simeq H^1(\spl,\pi)$, via the isomorphism: 
\[[X]\in H^1(\spl,\pi)\quad \leftrightarrow \quad [X\wedge C_\mathcal{R}]\in H^4(\spl,\pi);\]
\item $H^5(\spl,\pi)=0$;
\item $H^6(\spl,\pi)\simeq C^{\infty}(\C)/C^{\infty}_0(\C)$, via the isomorphism: 
\[[g\circ f\cdot C_{\mathcal{R}}\wedge C_{\mathcal{I}}]\in H^6(\spl,\pi) \qquad \leftrightarrow \qquad [g]\in C^{\infty}(\C)/C^{\infty}_0(\C).\]
\end{itemize}
\end{theorem}
Note that the wedge product on $H^{\bullet}(\spl,\pi)$ is determined from the descriptions in the theorem. The Schouten bracket is determined by the isomorphism of Lie algebras from $H^1(\spl,\pi)\simeq \out$, the usual Leibniz rule, and the following relations: for any $[X]\in H^1(\spl,\pi)$, 
\[[[X,C_{\mathcal{R}}]]=[[X,C_{\mathcal{I}}]]=0\in H^3(\spl,\pi).\]

The proof of Theorem \ref{theorem: PC} will be completed in Subsection \ref{section: algebra}, where we also prove the above relation.
% \[x+|z|=c\geq 0\]
% \[y^2+2cx-c^2=0,\quad  c\geq 0.\]


==> eigenspaces.tex <==
\section{Some decompositions of smooth functions on $\C$}\label{eigenspaces}

In this section, we will prove Lemma \ref{lemma:pullbacks and invariant functions}. We will use the notation from Subsection \ref{subsection:desing} for the eigenspaces of the pullback along the maps $\sigma=-\mathrm{id}_{\C}$ and $\tau=$ conjugation. As the operators $\sigma^*$ and $\tau^*$ commute they preserve their respective eigenspaces. We use similar notation for their common eigenspaces, for example:
\[C^{\infty}_{\sigma,-\tau}(\C):=\{g\in C^{\infty}(\C)\,|\, g=\sigma^*(g)=-\tau^*(g)\},\]
and similarly for functions flat at the origin.

We have the following decomposition of smooth functions: 
\begin{lemma}\label{lemma:eigenspaces}
Any function $g\in C^{\infty}(\C)$ can be written uniquely as: 
\[ g= g_0 + x\cdot g_x +y\cdot g_y +xy\cdot g_{xy}\]
where $g_0,g_x,g_y,g_{xy}\in C^{\infty}_{\sigma,\tau}(\C)$ and similarly for functions flat at the origin.
\end{lemma}
\begin{proof}
The four functions are constructed by the usual projections onto the common eigenspaces of $\sigma^*$ and $\tau^*$, namely: 
\begin{align*}
g_{0}:=&\frac{1}{4}(\mathrm{id}+\sigma^*)(\mathrm{id}+\tau^*)(g)\\
x\cdot g_{x}:=&\frac{1}{4}(\mathrm{id}-\sigma^*)(\mathrm{id}+\tau^*)(g)\\
y\cdot g_{y}:=&\frac{1}{4}(\mathrm{id}-\sigma^*)(\mathrm{id}-\tau^*)(g)\\
xy\cdot g_{xy}:=&\frac{1}{4}(\mathrm{id}+\sigma^*)(\mathrm{id}-\tau^*)(g).
\end{align*}
That these functions are indeed smooth follows from Hadamard's lemma. For example, in the first case, the function 
\[h:=\frac{1}{4}(\mathrm{id}-\sigma^*)(\mathrm{id}+\tau^*)(g)\]
satisfies $h(0,y)=0$, and therefore, by Hadamard's lemma, $h=xg_x$, with $g_x\in C^{\infty}(\C)$. 
\end{proof}

Flat functions invariant under $\sigma$ and $\tau$ can be described more explicitly: 
\begin{lemma}\label{lemma: lambda casimir}
The map defined by
\begin{equation*}
    \begin{array}{ccc}
        C^{\infty}(\R^2_{\ge 0} ) &\to &C_{\sigma,\tau}^{\infty}(\C), \\
         g &\mapsto & \widetilde{g}(x,y):= g(x^2 ,y^2)  
    \end{array}
\end{equation*}
is an isomorphism of rings, and similarly for functions flat at the origin.
\end{lemma}
\begin{proof}
Clearly, we only need to check that this map is surjective. For this, consider $\widetilde{g}\in C_{\sigma,\tau}^{\infty}(\C)$. We need to show that the function:
\[g:\R^2_{\geq 0}\to \R, \quad g(p,q)=\widetilde{g}(\sqrt{p},\sqrt{q}),\]
which is smooth on $\R^2_{>0}$, is smooth also on $\big(\{0\}\times \R_{\geq 0}\big)\cup \big(\R_{\geq 0}\times\{0\}\big)$. For this it suffices to check that all its partial derivatives extend continuously. Note that, for $p,q>0$, we have that 
\[    \partial_p^i\partial_q^j g(p,q)=
\Big(\frac{\partial_x}{2x}\Big)^{i}\Big(\frac{\partial_y}{2y}\Big)^{j}\widetilde{g}(x,y)\big|_{x=\sqrt{p},y=\sqrt{q}}.\]
Therefore, the proof will be complete once we show that the functions  
\[\Big(\frac{\partial_x}{2x}\Big)^{i}\Big(\frac{\partial_y}{2y}\Big)^{j}\widetilde{g}(x,y)\]
extend smoothly to $\R^2$. First, because $\widetilde{g}$ is invariant under $\sigma^*$ and $\tau^*$, we have that $\partial_xg(0,y)=0$ and $\partial_yg(x,0)=0$. Therefore, by Hadamard's lemma,
\[\frac{\partial_x\widetilde{g}}{2x}, \frac{\partial_y\widetilde{g}}{2y}\in  C^{\infty}(\C).\]
Moreover, note that these functions are also invariant under $\sigma^*$ and $\tau^*$, and so we can iterate this observation, and obtain that, for all $i,j\geq 0$,
\begin{align*}
\Big(\frac{\partial_x}{2x}\Big)^{i}\Big(\frac{\partial_y}{2y}\Big)^{j}\widetilde{g}\in C^{\infty}_{\sigma,\tau}(\C).  
\end{align*}
This concludes the proof. 
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:pullbacks and invariant functions}]
First, we show that the map from (1) is an isomorphism. 
Since $\mathrm{sq}:\C\to \C$ is surjective, the map is clearly injective. For surjectivity, consider first $h\in C^{\infty}_{0,\sigma,\tau}(\C)$. By Lemma \ref{lemma: lambda casimir}, we can write 
\[h(\lambda_1,\lambda_2)=k(2\lambda_1^2,2\lambda_2^2),\]
for some $k\in C^{\infty}_0(\R^2_{\geq 0})$. Define:
\[g:\C\to \R,\quad  g(z)=k(|z|+x,|z|-x), \quad z=x+yi\in \C.\]
Clearly, $g$ is smooth on $\C^{\times}$. Because $k$ is flat at $0$, it is easy to see that all partial derivatives of $g$ extend continuously as $0$ at $z=0$. Therefore $g\in C^{\infty}_0(\C)$. Clearly, $g$ is also $\tau^*$-invariant. Finally, note that
\[g(\lambda^2)=k(2\lambda_1^2,2\lambda_2^2)=h(\lambda).
\]
For a general element $h\in C^{\infty}_{0,\sigma}(\C)$, by Lemma \ref{lemma:eigenspaces}, we can find $h_0,h_1\in C^{\infty}_{0,\sigma,\tau}(\C)$ such that
\[h(\lambda)=h_0(\lambda)+2\lambda_1\lambda_2\cdot h_1(\lambda).\]
By the first part, we can write $h_i(\lambda)=g_i(\lambda^2)$, with $g_i\in C^{\infty}_{0,\sigma,\tau}(\C)$. Thus
\[h(\lambda)=g(\lambda^2),\quad \textrm{with}\quad g\in C^{\infty}_0(\C),\]
where $g(z)=g_1(z)+y\cdot g_2(z)$, for $z=x+iy$. This proves (1).

Next, we show that the map from (2) is surjective. Let $h\in C^{\infty}_{0,-\sigma}(\C)$. By Lemma \ref{lemma:eigenspaces}, we can write:
\[h(\lambda)=-\lambda_1\cdot h_1(\lambda)+\lambda_2\cdot h_2(\lambda),\]
with $h_i\in C^{\infty}_{0,\sigma,\tau}(\C)$. Again by the first part, there are $g_i\in C^{\infty}_{0,\tau}(\C)$ such that $h_i(\lambda)=g_i(\lambda^2)$, and so
\[h(\lambda)=-\lambda_1\cdot g_1(\lambda^2)+\lambda_2\cdot g_2(\lambda^2).\]
This proves surjectivity. 

To show understand the kernel, let $g_i\in C^{\infty}_{0}(\C)$ such that 
\[-\lambda_1\cdot g_1(\lambda^2)+\lambda_2\cdot g_2(\lambda^2)=0.\]
Note that this is equivalent to: 
\[2\lambda_1\lambda_2\cdot g_1(\lambda^2)=2\lambda_2^2\cdot g_2(\lambda^2).\]
If we denote $z=\lambda^2$, then $2\lambda_1\lambda_2=y$ and $2\lambda_2^2=|z|-x$. Thus the above identity is equivalent to
\begin{equation}\label{eq:relation:for:kernel}
y\cdot g_1(z)=(|z|-x)\cdot g_2(z), \quad \forall z\in \C.
\end{equation}
This concludes the proof of (2).

Item (3) follows from Proposition \ref{proposition: twisted module}. 
\end{proof}

% {\color{green}
% \begin{remark}\label{remark: free module}
% By choosing instead of \eqref{eq: second foliated ch identification} the identification
% \begin{equation*}
%     \begin{array}{ccc}
%          E^{\tau}_0\oplus E^{\tau}_0\oplus C^{\infty}_0(\R)&\to&(E^{\tau}_0\oplus E^{\tau}_0)^2/\mathcal{K}  \\
%          (g_1,g_2,h)&\mapsto&((g_1,g_2)(h(\frac{\Lambda_1}{2}),0)) 
%     \end{array}
% \end{equation*}
% one obtains the vector space isomorphism
% \begin{equation*}
%     \begin{array}{cccc}
%          &\Cas_0\times C^{\infty}_0(\R)&\to& H^{2}_{0}(\F)\\
%          &(g,h)&\mapsto &  [g\cdot e_{\varphi}(\tilde{\omega}_1) +h(\frac{\Lambda_1}{2})\circ f\cdot e_{\varphi}(\tilde{\omega}_2)]_{\F}
%     \end{array}
%     \end{equation*}
%     Here $C^{\infty}_0(\R)$ denotes the smooth functions on $\R$ which are flat at the origin. To obtain a module isomorphism we define the map
%     \begin{equation}\label{eq: strange quotient}
%         \begin{array}{cccc}
%              Q:&E^{\tau}_0&\to &E^{\tau}_0  \\
%              &k_1&\mapsto &\frac{ k_1(x,y)-k_1(\frac{\Lambda_1}{2},0)}{\Lambda_2}
%         \end{array}
%     \end{equation}
% \end{remark}
% }
